auto-sktime: Automated Time Series Forecasting

In today's data-driven landscape, time series forecasting is pivotal in decision-making across various sectors. Yet, the proliferation of more diverse time series data, coupled with the expanding landscape of available forecasting methods, poses significant challenges for forecasters. To meet the growing demand for efficient forecasting, we introduce auto-sktime, a novel framework for automated time series forecasting. The proposed framework uses the power of automated machine learning (AutoML) techniques to automate the creation of the entire forecasting pipeline. The framework employs Bayesian optimization, to automatically construct pipelines from statistical, machine learning (ML) and deep neural network (DNN) models. Furthermore, we propose three essential improvements to adapt AutoML to time series data. First, pipeline templates to account for the different supported forecasting models. Second, a novel warm-starting technique to start the optimization from prior optimization runs. Third, we adapt multi-fidelity optimizations to make them applicable to a search space containing statistical, ML and DNN models. Experimental results on 64 diverse real-world time series datasets demonstrate the effectiveness and efficiency of the framework, outperforming traditional methods while requiring minimal human involvement.

==> AISTATS/library.tex <==
@article{Masini2023,
author = {Masini, Ricardo P. and Medeiros, Marcelo C. and Mendes, Eduardo F.},
journal = {Journal of Economic Surveys},
number = {1},
pages = {76--111},
title = {{Machine learning advances for time series forecasting}},
volume = {37},
year = {2023}
}
@article{Rady2021,
abstract = {This paper aims to use the tree-based methods for time series data forecasting and compare between Decision Tree (DT), Random Forest (RF), Gradient Boosted Trees (GBT) and ARIMA model to predict monthly gold prices. The time series data for the monthly gold prices was used during the period from Nov-1989 to Dec-2019, which represents 362 observations. ARIMA, DT, RF, and GBT models were fitted based on 90{\%} of data as training set. Then, their accuracy was compared using the statistical measure RMSE. The results indicated that RF was better than DT, GBT and ARIMA (0,1,1) in predicting future gold prices, based on RMSE= 38.52.},
author = {Rady, EL Houssainy A. and Fawzy, Haitham and Fattah, Amal Mohamed Abdel},
file = {:root/Documents/Mendeley Desktop/Rady, Fawzy, Fattah - 2021 - Time series forecasting using tree based methods.pdf:pdf},
journal = {Journal of Statistics Applications and Probability},
number = {1},
pages = {229--244},
title = {{Time series forecasting using tree based methods}},
volume = {10},
year = {2021}
}
@article{Zhou2020a,
abstract = {Many real-world applications require the prediction of long sequence time-series, such as electricity consumption planning. Long sequence time-series forecasting (LSTF) demands a high prediction capacity of the model, which is the ability to capture precise long-range dependency coupling between output and input efficiently. Recent studies have shown the potential of Transformer to increase the prediction capacity. However, there are several severe issues with Transformer that prevent it from being directly applicable to LSTF, including quadratic time complexity, high memory usage, and inherent limitation of the encoder-decoder architecture. To address these issues, we design an efficient transformer-based model for LSTF, named Informer, with three distinctive characteristics: (i) a {\$}ProbSparse{\$} self-attention mechanism, which achieves {\$}O(L \backslashlog L){\$} in time complexity and memory usage, and has comparable performance on sequences' dependency alignment. (ii) the self-attention distilling highlights dominating attention by halving cascading layer input, and efficiently handles extreme long input sequences. (iii) the generative style decoder, while conceptually simple, predicts the long time-series sequences at one forward operation rather than a step-by-step way, which drastically improves the inference speed of long-sequence predictions. Extensive experiments on four large-scale datasets demonstrate that Informer significantly outperforms existing methods and provides a new solution to the LSTF problem.},
author = {Zhou, Haoyi and Zhang, Shanghang and Peng, Jieqi and Zhang, Shuai and Li, Jianxin and Xiong, Hui and Zhang, Wancai},
file = {:root/Documents/Mendeley Desktop/Zhou et al. - 2020 - Informer Beyond Efficient Transformer for Long Sequence Time-Series Forecasting.pdf:pdf},
journal = {AAI Conference on Artificial Intelligence},
number = {12},
pages = {11106--11115},
title = {{Informer: Beyond Efficient Transformer for Long Sequence Time-Series Forecasting}},
volume = {35},
year = {2020}
}
@article{Smyl2020,
abstract = {This paper presents the winning submission of the M4 forecasting competition. The submission utilizes a dynamic computational graph neural network system that enables a standard exponential smoothing model to be mixed with advanced long short term memory networks into a common framework. The result is a hybrid and hierarchical forecasting method.},
author = {Smyl, Slawek},
file = {:root/Documents/Mendeley Desktop/Smyl - 2020 - A hybrid method of exponential smoothing and recurrent neural networks for time series forecasting.pdf:pdf},
journal = {International Journal of Forecasting},
number = {1},
pages = {75--85},
title = {{A hybrid method of exponential smoothing and recurrent neural networks for time series forecasting}},
volume = {36},
year = {2020}
}
@article{Januschowski2020,
abstract = {The prevalence of approaches based on gradient boosted trees among the top contestants in the M5 competition is potentially the most eye-catching result. Tree-based methods out-shone other solutions, in particular deep learning-based solutions. The winners in both tracks of the M5 competition heavily relied on them. This prevalence is even more remarkable given the dominance of other methods in the literature and the M4 competition. This article tries to explain why tree-based methods were so widely used in the M5 competition. We see possibilities for future improvements of tree-based models and then distill some learnings for other approaches, including but not limited to neural networks.},
author = {Januschowski, Tim and Wang, Yuyang and Torkkola, Kari and Erkkil{\"{a}}, Timo and Hasson, Hilaf and Gasthaus, Jan},
file = {:root/Documents/Mendeley Desktop/Januschowski et al. - 2022 - Forecasting with trees.pdf:pdf},
journal = {International Journal of Forecasting},
keywords = {Deep Learning,Global forecasting models,Gradient Boosted Trees,Probabilistic forecasting,Random forests},
number = {4},
pages = {1473--1481},
title = {{Forecasting with trees}},
volume = {38},
year = {2022}
}
@article{Salinas2020,
author = {Salinas, David and Flunkert, Valentin and Gasthaus, Jan and Januschowski, Tim},
journal = {International Journal of Forecasting},
number = {3},
pages = {1181--1191},
title = {{DeepAR: Probabilistic forecasting with autoregressive recurrent networks}},
volume = {36},
year = {2020}
}
@inproceedings{Vogelsgesang2018,
abstract = {Industrial as well as academic analytics systems are usually evaluated based on well-known standard benchmarks, such as TPC-H or TPC-DS. These benchmarks test various components of the DBMS including the join optimizer, the implementation of the join and aggregation operators, concurrency control and the scheduler. However, these benchmarks fall short of evaluating the "real" challenges imposed by modern BI systems, such as Tableau, that emit machine-generated query workloads. This paper reports a comprehensive study based on a set of more than 60k real-world BI data repositories together with their generated query workload. The machine-generated workload posed by BI tools differs from the "hand-crafted" benchmark queries in multiple ways: Structurally simple relational operator trees often come with extremely complex scalar expressions such that expression evaluation becomes the limiting factor. At the same time, we also encountered much more complex relational operator trees than covered by benchmarks. This long tail in both, operator tree and expression complexity, is not adequately represented in standard benchmarks. We contribute various statistics gathered from the large dataset, e.g., data type distributions, operator frequency, string length distribution and expression complexity. We hope our study gives an impetus to database researchers and benchmark designers alike to address the relevant problems in future projects and to enable better database support for data exploration systems which become more and more important in the Big Data era.},
author = {Vogelsgesang, A. Adrian and Haubenschild, M. Michael and Finis, J. Jan and Kemper, A. Alfons and Leis, V. Viktor and Muehlbauer, T. Tobias and Neumann, T. Thomas and Then, M. Manuel},
booktitle = {Workshop on Testing Database Systems},
file = {:root/Documents/Mendeley Desktop/Vogelsgesang et al. - 2018 - Get real How benchmarks fail to represent the real world.pdf:pdf},
title = {{Get real: How benchmarks fail to represent the real world}},
year = {2018}
}
@article{Bansal2022,
abstract = {Recent advancements in deep learning architecture have increased its utility in real-life applications. Deep learning models require a large amount of data to train the model. In many application domains, there is a limited set of data available for training neural networks as collecting new data is either not feasible or requires more resources such as in marketing, computer vision, and medical science. These models require a large amount of data to avoid the problem of overfitting. One of the data space solutions to the problem of limited data is data augmentation. The purpose of this study focuses on various data augmentation techniques that can be used to further improve the accuracy of a neural network. This saves the cost and time consumption required to collect new data for the training of deep neural networks by augmenting available data. This also regularizes the model and improves its capability of generalization. The need for large datasets in different fields such as computer vision, natural language processing, security, and healthcare is also covered in this survey paper. The goal of this paper is to provide a comprehensive survey of recent advancements in data augmentation techniques and their application in various domains.},
author = {Bansal, Aayushi and Sharma, Rewa and Kathuria, Mamta},
file = {:root/Documents/Mendeley Desktop/Bansal, Sharma, Kathuria - 2022 - A Systematic Review on Data Scarcity Problem in Deep Learning Solution and Applications.pdf:pdf},
journal = {ACM Computing Surveys},
number = {10},
pages = {1--29},
title = {{A Systematic Review on Data Scarcity Problem in Deep Learning: Solution and Applications}},
volume = {54},
year = {2022}
}
@inproceedings{Wistuba2015,
   author = {Martin Wistuba and Nicolas Schilling and Lars Schmidt-Thieme},
   journal = {Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
   pages = {104–119},
   title = {Hyperparameter Search Space Pruning - A New Component for Sequential Model-Based Hyperparameter Optimization},
   year = {2015},
}
@inproceedings{Lindauer2018,
   author = {Marius Lindauer and Frank Hutter},
   booktitle = {AAAI Conference on Artificial Intelligence},
   pages = {1355-1362},
   title = {Warmstarting of Model-based Algorithm Configuration},
   year = {2018},
}
@article{Feurer2018,
   author = {Matthias Feurer and Katharina Eggensperger and Stefan Falkner and Marius Lindauer and Frank Hutter},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Practical Automated Machine Learning for the AutoML Challenge 2018},
   year = {2018},
}
@inproceedings{Rijn2018,
   author = {Jan N. van Rijn and Frank Hutter},
   journal = {International Conference on Knowledge Discovery and Data Mining},
   pages = {2367–2376},
   publisher = {Association for Computing Machinery},
   title = {Hyperparameter Importance Across Datasets},
   year = {2018},
}
@inproceedings{vanRijn2015,
   author = {Jan N. van Rijn and Salisu Mamman Abdulrahman and Pavel Brazdil and Joaquin Vanschoren},
   journal = {International Symposium on Intelligent Data Analysis},
   title = {Fast Algorithm Selection Using Learning Curves},
   year = {2015},
}
@inproceedings{Feurer2015a,
   author = {Matthias Feurer and Jost Tobias Springenberg and Frank Hutter},
   booktitle = {AAAI},
   pages = {1128-1135},
   title = {Initializing Bayesian Hyperparameter Optimization via Meta-Learning},
   year = {2015},
}
@article{DeMiranda2012,
   author = {Péricles B.C. De Miranda and Ricardo B.C. Prudêncio and Andre Carlos P.L.F. De Carvalho and Carlos Soares},
   journal = {International Conference on Computational Science and Its Applications},
   pages = {562-575},
   title = {An Experimental Study of the Combination of Meta-Learning with Particle Swarm Algorithms for SVM Parameter Selection},
   year = {2012},
}
@article{Reif2012,
   author = {Matthias Reif and Faisal Shafait and Andreas Dengel},
   journal = {Machine Learning},
   pages = {357-380},
   title = {Meta-learning for evolutionary parameter optimization of classifier},
   volume = {87},
   year = {2012},
}
@web_page{H2O.ai2018,
   author = {H2O.ai},
   title = {H2O Driverless AI},
   url = {https://www.h2o.ai/products/h2o-driverless-ai/},
   year = {2018},
}
@article{Alia2006,
   author = {Shawkat Alia and Kate A. Smith-Miles},
   issue = {1-3},
   journal = {Neurocomputing},
   pages = {173–186},
   title = {A meta-learning approach to automatic kernel selection for support vector machines},
   volume = {70},
   year = {2006},
}
@web_page{Google2019,
   author = {Google},
   title = {Google Trends},
   url = {https://trends.google.de/trends/explore?date=today 5-y&q=automl},
   year = {2019},
}
@article{Guyon2008,
   author = {Isabelle Guyon and Amir Saffari and Gideon Dror and Gavin Cawley},
   issue = {2-3},
   journal = {Neural Networks},
   pages = {544-550},
   title = {Analysis of the IJCNN 2007 Agnostic Learning vs. Prior Knowledge Challenge},
   volume = {21},
   year = {2008},
}
@article{Escalante2009,
   author = {Hugo Jair Escalante and Manuel Montes and Villaseñor Luis},
   journal = {Iberoamerican Congress on Pattern Recognition},
   pages = {563-570},
   title = {Particle Swarm Model Selection for Authorship Verificatio},
   year = {2009},
}
@inproceedings{Chen2004,
   author = {Peng-Wei Chen and Jung-Ying Wang and Hahn-Ming Lee},
   journal = {IEEE International Joint Conference on Neural Networks},
   title = {Model selection of SVMs using GA approach},
   year = {2004},
}
@article{Samanta2004,
   author = {B. Samanta},
   issue = {3},
   journal = {Mechanical Systems and Signal Processing},
   pages = {625-644},
   title = {Gear fault detection using artificial neural networks and support vector machines with genetic algorithms},
   volume = {18},
   year = {2004},
}
@web_page{Dinsmore2016,
   author = {Thomas Dinsmore},
   title = {Automated Machine Learning: A Short History},
   url = {https://blog.datarobot.com/automated-machine-learning-short-history},
   year = {2016},
}
@article{Liu2016,
   author = {Weibo Liu and Zidong Wang and Xiaohui Liu and Nianyin Zeng and Yurong Liu and Fuad E. Alsaadi},
   journal = {Neurocomputing},
   pages = {11-26},
   title = {A survey of deep neural network architectures and their applications},
   volume = {234},
   year = {2017},
}
@book_section{Olson2016c,
   author = {Randal S. Olson and Jason H. Moore},
   journal = {Genetic Programming Theory and Practice XIV},
   pages = {211-223},
   title = {Identifying and Harnessing the Building Blocks of Machine Learning Pipelines for Sensible Initialization of a Data Science Automation Tool},
   year = {2018},
}
@inproceedings{Langford2008,
   author = {John Langford and Tong Zhang},
   journal = {Advances in Neural Information Processing Systems},
   pages = {817-824},
   title = {The Epoch-Greedy Algorithm for Contextual Multi-armed Bandits},
   year = {2008},
}
@article{Robbins1952,
   author = {Herbert Robbins},
   issue = {5},
   journal = {Bulletin of the American Mathematical Society},
   pages = {527-535},
   title = {Some Aspects of the Sequential Design of Experiments},
   volume = {58},
   year = {1952},
}
@inproceedings{Zoph2016,
   author = {Barret Zoph and Quoc V. Le},
   journal = {International Conference on Learning Representations},
   title = {Neural Architecture Search with Reinforcement Learning},
   year = {2017},
}
@article{Auer1995,
   author = {Peter Auer and Nicolo Cesa-Bianchi and Yoav Freund and Robert E. Schapire},
   journal = {Foundations of Computer Science},
   pages = {322-346},
   title = {Gambling in a Rigged Casino: The Adversarial Multi-Armed Bandit Problem},
   year = {1995},
}
@article{Auer2002,
   author = {Peter Auer and Nicolo Cesa-Bianchi and Paul Fischer},
   issue = {2},
   journal = {Machine Learning},
   pages = {235-256},
   title = {Finite-time Analysis of the Multiarmed Bandit Problem},
   volume = {47},
   year = {2002},
}
@book{Breiman1984,
   author = {Leo Breiman and Jerome Friedman and Charles J. Stone and R.A. Olsen},
   publisher = {Chapman and Hall},
   title = {Classification and Regression Trees},
   year = {1984},
}
@article{Wang2009,
   author = {Zhou Wang and Alan C. Bovik},
   issue = {1},
   journal = {IEEE Signal Processing Magazine},
   pages = {98-117},
   title = {Mean squared error: Love it or leave it? A new look at Signal Fidelity Measures},
   volume = {26},
   year = {2009},
}
@article{Dixon1978,
   author = {L. C. W. Dixon and G. P. Szego},
   journal = {Towards Global Optimisation},
   pages = {1-15},
   title = {The Global Optimization Problem: An Introduction},
   year = {1978},
}
@article{Rosasco2004,
   author = {Lorenzo Rosasco and Ernesto De Vito and Andrea Caponnetto and Michele Piana and Alessandro Verri},
   issue = {5},
   journal = {Neural Computation},
   pages = {1063-1076},
   title = {Are Loss Functions All the Same?},
   volume = {16},
   year = {2004},
}
@article{Pepelyshev2017,
   author = {Andrey Pepelyshev and Anatoly Zhigljavsky and Antanas Žilinskas},
   issue = {1},
   journal = {Journal of Global Optimization},
   pages = {57-71},
   title = {Performance of global random search algorithms for large dimensions},
   volume = {71},
   year = {2017},
}
@article{Laguna2005,
   author = {Manuel Laguna and Rafael Martí},
   issue = {2},
   journal = {Journal of Global Optimization},
   pages = {235-255},
   title = {Experimental Testing of Advanced Scatter Search Designs for Global Optimization of Multimodal Functions},
   volume = {33},
   year = {2005},
}
@inproceedings{Jamieson2016,
   author = {Kevin Jamieson and Ameet Talwalkar},
   journal = {Artificial Intelligence and Statistics},
   pages = {240-248},
   title = {Non-stochastic Best Arm Identification and Hyperparameter Optimization},
   year = {2015},
}
@article{Parzen1961,
   author = {Emanuel Parzen},
   issue = {3},
   journal = {The Annals of Mathematical Statistics},
   pages = {1065-1076},
   title = {On Estimation of a Probability Density Function and Mode},
   volume = {33},
   year = {1961},
}
@inproceedings{Klein2016,
   author = {Aaron Klein and Stefan Falkner and Simon Bartels and Philipp Hennig and Frank Hutter},
   booktitle = {Artificial Intelligence and Statistics},
   pages = {528-536},
   title = {Fast Bayesian Optimization of Machine Learning Hyperparameters on Large Datasets},
   year = {2016},
}
@article{Quanming2018,
   author = {Yao Quanming and Wang Mengshuo and Jair Escalante Hugo and Guyon Isabelle and Hu Yi-Qi and Li Yu-Feng and Tu Wei-Wei and Yang Qiang and Yu Yang},
   journal = {arXiv:1810.13306},
   title = {Taking Human out of Learning Applications: A Survey on Automated Machine Learning},
   year = {2018},
}
@inproceedings{Hutter2009a,
   author = {Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown and Kevin P. Murphy},
   journal = {Conference on Genetic and Evolutionary Computation},
   keywords = {active learning,design,gaussian processes,noisy optimization,parameter tuning,sequential experimental},
   pages = {271-278},
   title = {An Experimental Investigation of Model-Based Parameter Optimisation: SPO and Beyond},
   year = {2009},
}
@article{Pedregosa2011,
   author = {F. Pedregosa and G. Varoquaux and A. Gramfort and V. Michel and B. Thirion and O. Grisel and M. Blondel and P. Prettenhofer and R. Weiss and V. Dubourg and Jake Vanderplas and A. Passos and D. Cournapeau and M. Brucher and M. Perrot and E. Duchesnay},
   journal = {Journal of Machine Learning Research},
   pages = {2825-2830},
   title = {Scikit-learn: Machine Learning in Python},
   volume = {12},
   year = {2011},
}
@article{Dewancker2015,
   author = {Ian Dewancker and Michael McCourt and Scott Clark},
   pages = {2-5},
   title = {Bayesian Optimization Primer},
   year = {2015},
}
@inproceedings{Gelbart2014,
   author = {Michael A. Gelbart and Jasper Snoek and Ryan P. Adams},
   journal = {Conference on Uncertainty in Artificial Intelligence},
   pages = {25-259},
   title = {Bayesian Optimization with Unknown Constraints},
   year = {2014},
}
@thesis{Snoek2013,
   author = {Jasper Snoek},
   title = {Bayesian Optimization and Semiparametric Models with Applications to Assistive Technology},
   year = {2013},
}
@inproceedings{Snoek2014,
   author = {Jasper Snoek and Kevin Swersky and Richard S. Zemel and Ryan P. Adams},
   journal = {International Conference on Machine Learning},
   pages = {1674-1682},
   title = {Input Warping for Bayesian Optimization of Non-stationary Functions},
   year = {2014},
}
@inproceedings{Swersky2013,
   author = {Kevin Swersky and Jasper Snoek and Ryan P. Adams},
   journal = {International Conference on Neural Information Processing Systems},
   pages = {2004-2012},
   title = {Multi-Task Bayesian Optimization},
   year = {2013},
}
@article{Breiman2001,
   author = {Leo Breiman},
   issue = {1},
   journal = {Machine Learning},
   pages = {5-32},
   title = {Random Forests},
   volume = {45},
   year = {2001},
}
@book{Rasmussen2006,
   author = {C. E. Rasmussen and C. K. I. Williams},
   journal = {MIT Press},
   publisher = {The MIT Press},
   title = {Gaussian Processes for Machine Learning},
   year = {2006},
}
@article{Frazier2018,
   author = {Peter I. Frazier},
   journal = {arXiv: 1807.02811},
   title = {A Tutorial on Bayesian Optimization},
   year = {2018},
}
@book_section{Guyon2018,
   author = {Isabelle Guyon and Lisheng Sun-Hosoya and Marc Boullé and Hugo Jair Escalante and Sergio Escalera and Zhengying Liu and Damir Jajetic and Bisakha Ray and Mehreen Saeed and Michele Sebag and Alexander Statnikov and Wei-Wei Tu and Evelyne Viegas},
   journal = {Automatic Machine Learning: Methods, Systems, Challenges},
   publisher = {Springer Verlag},
   title = {Analysis of the AutoML Challenge series 2015-2018},
   year = {2018},
}
@article{Mockus1978,
   author = {Jonas Mockus and Vytautas Tiesis and Antanas Zilinskas},
   journal = {Towards Global Optimisation},
   keywords = {Expected Improvement},
   pages = {117-129},
   title = {The application of Bayesian methods for seeking the extremum},
   volume = {2},
   year = {1978},
}
@article{Anderson1953,
   author = {Richard Loree Anderson},
   issue = {264},
   journal = {Journal of the American Statistical Association},
   pages = {789-798},
   title = {Recent Advances in Finding Best Operating Conditions},
   volume = {48},
   year = {1953},
}
@web_page{Kegl2017,
   author = {Balázs Kégl},
   title = {How to Build a Data Science Pipeline},
   url = {https://www.kdnuggets.com/2017/07/build-data-science-pipeline.html},
   year = {2017},
}
@book{Snyman2005,
   author = {Jan A. Snyman},
   publisher = {Springer},
   title = {Practical Mathematical Optimization: An introduction to basic optimization theory and classical and new gradient-based algorithms},
   year = {2005},
}
@web_page{Zhou2018,
   author = {Linda Zhou},
   title = {How to Build a Better Machine Learning Pipeline},
   url = {https://www.datanami.com/2018/09/05/how-to-build-a-better-machine-learning-pipeline/},
   year = {2018},
}
@inproceedings{Agerri2014,
   author = {Rodrigo Agerri and Josu Bermudez and German Rigau},
   journal = {Language Resources and Evaluation},
   pages = {3823-3828},
   title = {IXA pipeline: Efficient and Ready to Use Multilingual NLP tools},
   year = {2014},
}
@article{Bischl2017,
   author = {Bernd Bischl and Giuseppe Casalicchio and Matthias Feurer and Frank Hutter and Michel Lang and Rafael G. Mantovani and Jan N. van Rijn and Joaquin Vanschoren},
   journal = {arXiv:1708.03731v1},
   title = {OpenML Benchmarking Suites and the OpenML100},
   year = {2017},
}
@article{Vanschoren2014,
   author = {Joaquin Vanschoren and Jan N. van Rijn and Bernd Bischl and Luis Torgo},
   issue = {2},
   journal = {ACM International Conference on Knowledge Discovery and Data Mining},
   pages = {49-60},
   title = {OpenML: networked science in machine learning},
   volume = {15},
   year = {2014},
}
@inproceedings{Chen2016,
   author = {Tianqi Chen and Carlos Guestrin},
   journal = {ACM International Conference on Knowledge Discovery and Data Mining},
   pages = {785-794},
   title = {XGBoost: A Scalable Tree Boosting System Tianqi},
   year = {2016},
}
@web_page{Ayria2018,
   author = {Pourya Ayria},
   title = {A complete Machine Learning PipeLine},
   url = {https://www.kaggle.com/pouryaayria/a-complete-ml-pipeline-tutorial-acu-86},
   year = {2018},
}
@inproceedings{Abadi2016,
   author = {Martin Abadi and Paul Barham and Jianmin Chen and Zhifeng Chen and Andy Davis and Jeffrey Dean and Matthieu Devin and Sanjay Ghemawat and Geoffrey Irving and Michael Isard and Manjunath Kudlur and Josh Levenberg and Rajat Monga and Sherry Moore and Derek G. Murray and Benoit Steiner and Paul Tucker and Vijay Vasudevan and Pete Warden and Martin Wicke and Yuan Yu and Xiaoqiang Zheng},
   journal = {OSDI},
   pages = {265-283},
   title = {TensorFlow: A System for Large-Scale Machine Learning},
   volume = {16},
   year = {2016},
}
@inproceedings{Balles2017,
   author = {Lukas Balles and Maren Mahsereci and Philipp Hennig},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Automating Stochastic Optimization with Gradient Variance Estimates},
   year = {2017},
}
@inproceedings{Efimova2017,
   author = {Valeria Efimova and Andrey Filchenkov and Viacheslav Shalamov},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Fast Automated Selection of Learning Algorithm And its Hyperparameters by Reinforcement Learning},
   year = {2017},
}
@article{Raileanu2004,
   author = {Laura Elena Raileanu and Kilian Stoffel},
   issue = {1},
   journal = {Annals of Mathematics and Artificial Intelligence},
   pages = {77-93},
   title = {Theoretical comparison between the Gini Index and Information Gain criteria},
   volume = {41},
   year = {2004},
}
@inproceedings{Malkomes2017,
   author = {Gustavo Malkomes and Roman Garnett},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Towards Automated Bayesian Optimization},
   year = {2017},
}
@inproceedings{Kandasamy2018,
   author = {Kirthevasan Kandasamy and Akshay Krishnamurthy and Jeff Schneider and Barnabás Póczos},
   journal = {International Conference on Artificial Intelligence and Statistics},
   pages = {133-142},
   title = {Parallelised Bayesian Optimisation via Thompson Sampling Kirthevasan},
   year = {2018},
}
@inproceedings{Do2000,
   author = {Erhard Rahm and Hong Hai Do},
   journal = {IEEE Data Engineering Bulletin},
   title = {Data cleaning: Problems and Current Approaches},
   year = {2000},
}
@inproceedings{Bottou2010,
   author = {Leon Bottou},
   journal = {International Conference on Computational Statistics},
   pages = {177-186},
   title = {Large-Scale Machine Learning with Stochastic Gradient Descent},
   year = {2010},
}
@article{Bengio1994,
   author = {Yoshua Bengio and Patrice Simard and Paolo Frasconi},
   issue = {2},
   journal = {IEEE Transactions on Neural Networks},
   pages = {157-166},
   title = {Learning Long-Term Dependencies with Gradient Descent is Difficult},
   volume = {5},
   year = {1994},
}
@article{Bengio2000,
   author = {Yoshua Bengio},
   issue = {8},
   journal = {Neural Computation},
   pages = {1889-1900},
   title = {Gradient-Based Optimization of Hyperparameters},
   volume = {12},
   year = {2000},
}
@inproceedings{Franceschi2017,
   author = {Luca Franceschi and Michele Donini and Paolo Frasconi and Massimiliano Pontil},
   journal = {International Conference on Machine Learning},
   pages = {1165-1173},
   title = {Forward and Reverse Gradient-Based Hyperparameter Optimization},
   year = {2017},
}
@inproceedings{Maclaurin2015,
   author = {Dougal Maclaurin and David Duvenaud and Ryan P. Adams},
   journal = {International Conference on Machine Learning},
   pages = {2113–2122},
   title = {Gradient-based Hyperparameter Optimization through Reversible Learning},
   year = {2015},
}
@inproceedings{Pedregosa2016,
   author = {Fabian Pedregosa},
   booktitle = {International Conference on Machine Learning},
   pages = {737-746},
   title = {Hyperparameter optimization with approximate gradient},
   year = {2016},
}
@book{Coello2007,
   author = {Carlos A. Coello Coello and Gary B. Lamont and David A. Van Veldhuizen},
   journal = {American Journal of Psychiatry},
   publisher = {Springer},
   title = {Evolutionary Algorithms for Solving Multi-Objective Problems},
   volume = {5},
   year = {2007},
}
@article{Friedman1997a,
   author = {Jerome Friedman},
   journal = {Data Mining and Knowledge Discovery},
   keywords = {bagging,bias,classification,curse-of-dimensionality,naive Bayes,nearest-neighbors,variance},
   pages = {55-77},
   title = {On Bias, Variance, 0/1-Loss, and the Curse-of-Dimensionality},
   volume = {1},
   year = {1997},
}
@book_section{Parsopoulos2016,
   author = {Konstantinos E. Parsopoulos},
   journal = {Handbook of Heuristics},
   pages = {1-47},
   publisher = {Springer International Publishing},
   title = {Particle Swarm Methods},
   year = {2016},
}
@article{Reynolds1987,
   author = {Craig W. Reynolds},
   issue = {4},
   journal = {Computer Graphics},
   pages = {25-34},
   title = {Flocks, Herds, and Schools: A Distributed Behavioral Model},
   volume = {21},
   year = {1987},
}
@inproceedings{Kennedy1995,
   author = {James Kennedy and Russell Eberhart},
   journal = {International Conference on Neural Networks},
   pages = {1942-1948},
   title = {Particle Swarm Optimization},
   year = {1995},
}
@article{McGibbon2016,
   author = {Robert T. McGibbon and Carlos X. Hernández and Matthew P. Harrigan and Steven Kearnes and Mohammad M. Sultan and Stanislaw Jastrzebski and Brooke E. Husic and Vijay S. Pande},
   issue = {5},
   journal = {Journal of Open Source Software},
   pages = {34},
   title = {Osprey: Hyperparameter Optimization for Machine Learning},
   volume = {1},
   year = {2016},
}
@book{Banzhaf1997,
   author = {Wolfgang Banzhaf and Peter Nordin and Robert E. Keller and Frank D. Francone},
   publisher = {Morgan Kaufmann},
   title = {Genetic Programming: An Introduction},
   year = {1997},
}
@web_page{McGushion2019,
   author = {Hunter McGushion},
   title = {HyperparameterHunter},
   url = {https://github.com/HunterMcGushion/hyperparameter_hunter},
   year = {2019},
}
@web_page{Parry2019,
   author = {Preston Parry},
   title = {auto_ml},
   url = {https://github.com/ClimbsRocks/auto_ml},
   year = {2019},
}
@article{Meng2016,
   author = {Xiangrui Meng and Joseph Bradley and Burak Yavuz and Evan Sparks and Shivaram Venkataraman and Davies Liu and Jeremy Freeman and DB Tsai and Manish Amde and Sean Owen and Doris Xin and Reynold Xin and Michael J. Franklin and Reza Zadeh and Matei Zaharia and Ameet Talwalkar},
   issue = {34},
   journal = {Journal of Machine Learning Research},
   pages = {1-7},
   title = {MLlib: Machine Learning in Apache Spark},
   volume = {17},
   year = {2016},
}
@web_page{Baidu2018,
   author = {Baidu},
   title = {EZDL},
   url = {http://ai.baidu.com/ezdl/},
   year = {2018},
}
@article{Buitinck2013,
   author = {Lars Buitinck and Gilles Louppe and Mathieu Blondel and Fabian Pedregosa and Andreas Mueller and Olivier Grisel and Vlad Niculae and Peter Prettenhofer and Alexandre Gramfort and Jaques Grobler and Robert Layton and Jake Vanderplas and Arnaud Joly and Brian Holt and Gaél Varoquaux},
   journal = {European Conference on Machine Learning Workshop: Languages for Data Mining and Machine Learning},
   pages = {1-15},
   title = {API design for machine learning software: experiences from the scikit-learn project},
   year = {2013},
}
@web_page{Clouder2018,
   author = {Alibaba Clouder},
   title = {Shortening Machine Learning Development Cycle with AutoML},
   url = {https://www.alibabacloud.com/blog/shortening-machine-learning-development-cycle-with-automl_594232},
   year = {2018},
}
@article{Dean2008,
   author = {Jeffrey Dean and Sanjay Ghemawat},
   issue = {1},
   journal = {Communications of the ACM},
   pages = {107-113},
   title = {MapReduce: Simplified Data Processing on Large Clusters},
   volume = {51},
   year = {2008},
}
@book{Buyya1999,
   author = {Rajkumar Buyya},
   publisher = {Prentice Hall},
   title = {High Performance Cluster Computing: Architectures and Systems},
   volume = {1},
   year = {1999},
}
@article{Desautels2014,
   author = {Thomas Desautels and Andreas Krause and Joel W. Burdick},
   journal = {Journal of Machine Learning Research},
   pages = {4053-4103},
   title = {Parallelizing Exploration-Exploitation Tradeoffs with Gaussian Process Bandit Optimization},
   volume = {15},
   year = {2014},
}
@inproceedings{Zeng2008,
   author = {Zhi-Qiang Zeng and Hong-Bin Yu and Hua-Rong Xu and Yan-Qi Xie and Ji Gao},
   journal = {International Conference on Intelligent System and Knowledge Engineering},
   pages = {997-1001},
   title = {Fast training Support Vector Machines using parallel sequential minimal optimization},
   year = {2008},
}
@inproceedings{Zinkevich2010,
   author = {Martin Zinkevich and Markus Weimer and Lihong Li and Alex J. Smola},
   journal = {Advances in Neural Information Processing Systems},
   pages = {2595-2603},
   title = {Parallelized Stochastic Gradient Descent},
   volume = {23},
   year = {2010},
}
@incollection{Hutter2018a,
   author = {Frank Hutter and Lars Kotthoff and Joaquin Vanschoren},
   booktitle = {Automatic Machine Learning: Methods, Systems, Challenges},
   pages = {3-38},
   publisher = {Springer},
   title = {Hyperparameter Optimization},
   year = {2018},
}
@article{Nickson2014,
   author = {Thomas Nickson and Michael A. Osborne and Steven Reece and Stephen Roberts},
   journal = {arXiv: 1407.7969},
   title = {Automated Machine Learning on Big Data using Stochastic Algorithm Tuning},
   year = {2014},
}
@article{Hennig2012,
   author = {Philipp Hennig and Christian J. Schuler},
   journal = {Journal of Machine Learning Research},
   pages = {1809-1837},
   title = {Entropy Search for Information-Efficient Global Optimization},
   volume = {13},
   year = {2012},
}
@article{Swersky2014,
   author = {Kevin Swersky and Jasper Snoek and Ryan P. Adams},
   journal = {arXiv:1406.3896},
   title = {Freeze-Thaw Bayesian Optimization},
   year = {2014},
}
@book_section{Bottou2012,
   author = {Leon Bottou},
   journal = {Neural Networks, Tricks of the Trade, Reloaded},
   pages = {430-445},
   publisher = {Springer},
   title = {Stochastic Gradient Descent Tricks},
   year = {2012},
}
@inproceedings{Krizhevsky2012,
   author = {Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton},
   journal = {International Conference on Neural Information Processing Systems},
   pages = {1097-1105},
   title = {ImageNet Classification with Deep Convolutional Neural Networks},
   volume = {1},
   year = {2012},
}
@inproceedings{Malik2011,
   author = {Hassan H. Malik and Vikas S. Bhardwaj},
   journal = {IEEE International Conference on Data Mining},
   pages = {442-449},
   title = {Automatic training data cleaning for text classification},
   year = {2011},
}
@inproceedings{Chu2016,
   author = {Xu Chu and Ihab F Ilyas and Sanjay Krishnan and Jiannan Wang},
   journal = {International Conference on Management of Data},
   pages = {2201-2206},
   title = {Data Cleaning: Overview and Emerging Challenges},
   year = {2016},
}
@inproceedings{Raman2001,
   author = {Vijayshankar Raman and Joseph M. Hellerstein},
   journal = {International Conference on Very Large Data Bases},
   pages = {381-390},
   title = {Potter’s Wheel: An Interactive Data Cleaning System},
   volume = {1},
   year = {2001},
}
@article{Hellerstein2008,
   author = {Joseph M. Hellerstein},
   journal = {United Nations Economic Commission for Europe},
   title = {Quantitative Data Cleaning for Large Databases},
   year = {2008},
}
@inproceedings{Chu2015,
   author = {Xu Chu and John Morcos and Ihab F. Ilyas and Mourad Ouzzani and Paolo Papotti and Nan Tang and Yin Ye},
   journal = {ACM International Conference on Management of Data},
   keywords = {crowdsourcing,data cleaning,data quality,knowledge base},
   pages = {1247-1261},
   title = {KATARA: A Data Cleaning System Powered by Knowledge Bases and Crowdsourcing},
   year = {2015},
}
@thesis{Salvador2017,
   author = {Manuel Martin Salvador},
   institution = {Bournemouth University},
   title = {Automatic and adaptive preprocessing for the development of predictive models},
   year = {2017},
}
@inproceedings{Gil2019,
   author = {Yolanda Gil and James Honaker and Shikhar Gupta and Yibo Ma and Vito D Orazio and Daniel Garijo and Shruti Gadewar and Qifan Yang and Neda Jahanshad},
   journal = {International Conference on Intelligent User Interfaces},
   publisher = {Association for Computing Machinery},
   title = {Towards Human-Guided Machine Learning},
   year = {2019},
}
@inproceedings{Messaoud2011,
   author = {Ines Ben Messaoud and Haikal El Abed and Volker Märgner and Hamid Amiri},
   journal = {Workshop on Historical Document Imaging and Processing},
   pages = {177-183},
   title = {A design of a preprocessing framework for large database of historical documents},
   year = {2011},
}
@inproceedings{Teichmann2010,
   author = {Erich Teichmann and Eren Demir and Thierry Chaussalet},
   journal = {International Symposium on Computer-Based Medical Systems},
   pages = {184-189},
   title = {Data preparation for clinical data mining to identify patients at risk of readmission},
   year = {2010},
}
@inproceedings{Salvador2016,
   author = {Manuel Martin Salvador and Marcin Budka and Bogdan Gabrys},
   journal = {International Conference on Hybrid Artificial Intelligence Systems},
   pages = {27-39},
   title = {Towards automatic composition of multicomponent predictive systems},
   year = {2016},
}
@book{Pyle1999,
   author = {Dorian Pyle},
   journal = {Applied Artificial Intelligence},
   publisher = {Morgan Kaufmann Publishers, Inc.},
   title = {Data Preparation for Data Mining},
   year = {1999},
}
@inproceedings{Nisioti2018,
   author = {Eleni Nisioti and Kyriakos C. Chatzidimitriou and Andreas L. Symeonidis},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Predicting hyperparameters from meta-features in binary classification problems},
   year = {2018},
}
@inproceedings{Smith2017,
   author = {Micah J. Smith and Roy Wedge and Kalyan Veeramachaneni},
   booktitle = {IEEE DSAA},
   pages = {590-600},
   title = {FeatureHub: Towards collaborative data science},
   year = {2017},
}
@article{Zhu2004,
   author = {Xingquan Zhu and Xindong Wu},
   issue = {3},
   journal = {Artificial Intelligence Review},
   keywords = {attribute noise,class noise,machine learning,noise impacts},
   pages = {177-210},
   title = {Class Noise vs. Attribute Noise: A Quantitative Study},
   volume = {22},
   year = {2004},
}
@article{Jeatrakul2010,
   author = {Piyasak Jeatrakul and Kok Wai Wong and Chun Che Fung},
   issue = {3},
   journal = {Journal of Advanced Computational Intelligence and Intelligent Informatics},
   keywords = {Artificial neural network,Classifier,Data cleaning,Data pre-processing},
   pages = {297-302},
   title = {Data Cleaning for Classification Using Misclassification Analysis},
   volume = {14},
   year = {2010},
}
@inproceedings{Jeffery2006,
   author = {Shawn R. Jeffery and Gustavo Alonso and Michael J. Franklin and Wei Hong and Jennifer Widom},
   journal = {International Conference on Pervasive Computing},
   pages = {83-100},
   title = {Declarative Support for Sensor Data Cleaning},
   year = {2006},
}
@web_page{Chan2017,
   author = {Tobe Chan},
   title = {Advisor},
   url = {https://github.com/tobegit3hub/advisor},
   year = {2017},
}
@article{Wolpert1997,
   author = {David H. Wolpert and William G. Macready},
   issue = {1},
   journal = {IEEE Transactions on Evolutionary Computation},
   pages = {67-82},
   title = {No Free Lunch Theorems for Optimization},
   volume = {1},
   year = {1997},
}
@article{Baker2016,
   author = {Bowen Baker and Otkrist Gupta and Nikhil Naik and Ramesh Raskar},
   journal = {arXiv: 1611.02167},
   pages = {1-18},
   title = {Designing Neural Network Architectures using Reinforcement Learning},
   year = {2016},
}
@inproceedings{Litjens2017,
   author = {Geert Litjens and Thijs Kooi and Babak Ehteshami Bejnordi and Arnaud Arindra Adiyoso Setio and Francesco Ciompi and Mohsen Ghafoorian and Jeroen A.W.M. van der Laak and Bram van Ginneken and Clara I. Sánchez},
   journal = {Medical Image Computing and Computer-Assisted Intervention},
   pages = {254--261},
   title = {A Survey on Deep Learning in Medical Image Analysis},
   year = {2013},
}
@article{Browne2012,
   author = {Cameron Browne and Edward Powley and Daniel Whitehouse and Simon Lucas and Senior Member and Peter I Cowling and Philipp Rohlfshagen and Stephen Tavener and Diego Perez and Spyridon Samothrakis and Simon Colton},
   issue = {1},
   journal = {IEEE Transactions on Computational Intelligence and AI in Games},
   pages = {1-49},
   title = {A Survey of Monte Carlo Tree Search Methods},
   volume = {4},
   year = {2012},
}
@article{Silver2017,
   author = {David Silver and Thomas Hubert and Julian Schrittwieser and Ioannis Antonoglou and Matthew Lai and Arthur Guez and Marc Lanctot and Laurent Sifre and Dharshan Kumaran and Thore Graepel and Timothy Lillicrap and Karen Simonyan and Demis Hassabis},
   journal = {arXiv:1712.01815},
   title = {Mastering Chess and Shogi by Self-Play with a General Reinforcement Learning Algorithm},
   year = {2017},
}
@article{Lake2017,
   author = {Brenden M. Lake and Tomer D. Ullman and Joshua B. Tenenbaum and Samuel J. Gershman},
   journal = {Behavioral and Brain Sciences},
   pages = {1-58},
   title = {Building machines that learn and think like people},
   volume = {40},
   year = {2017},
}
@book{Ghallab2004,
   author = {Malik Ghallab and Dana Nau and Paolo Traverso},
   publisher = {Morgan Kaufmann Publishers, Inc.},
   title = {Automated Planmning: Theory & Praxis},
   year = {2004},
}
@inproceedings{Cooper2003a,
   author = {Jason Cooper and Chris Hinde},
   journal = {International Conference on Industrial, Engineering and Other Applications of Applied Intelligent Systems},
   pages = {636-643},
   title = {Improving genetic algorithms’ efficiency using intelligent fitness functions},
   year = {2003},
}
@article{Mohr2018,
   author = {Felix Mohr and Marcel Wever and Eyke Hüllermeier},
   journal = {Machine Learning},
   pages = {1495-1515},
   title = {ML-Plan: Automated machine learning via hierarchical planning},
   volume = {107},
   year = {2018},
}
@inproceedings{Drori2018,
   author = {Iddo Drori and Yamuna Krishnamurthy and Remi Rampin and Raoni de Paula Lourenco and Jorge Piazentin Ono and Kyunghyun Cho and Claudio Silva and Juliana Freire},
   booktitle = {International Conference on Machine Learning AutoML Workshop},
   pages = {1-8},
   title = {AlphaD3M: Machine Learning Pipeline Synthesis},
   year = {2018},
}
@inproceedings{Langevin2018,
   author = {Scott Langevin and David Jonker and Christopher Bethune and Glen Coppersmith and Casey Hilland and Jonathon Morgan and Paul Azunre and Justin Gawrilow},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Distil: A Mixed-Initiative Model Discovery System for Subject Matter Experts},
   year = {2018},
}
@inproceedings{Schoenfeld2018,
   author = {Brandon Schoenfeld and Christophe Giraud-Carrier and Mason Poggemann and Jarom Christensen and Kevin Seppi},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Preprocessor Selection for Machine Learning Pipelines},
   year = {2018},
}
@inproceedings{Khurana2018a,
   author = {Udayan Khurana and Horst Samulowitz and Deepak Turaga},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Ensembles with Automated Feature Engineering},
   year = {2018},
}
@inproceedings{Wever2018,
   author = {Marcel Wever and Felix Mohr and Eyke Hüllermeier},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {ML-Plan for Unlimited-Length Machine Learning Pipelines},
   year = {2018},
}
@article{Doshi-Velez2017,
   author = {Finale Doshi-Velez and Been Kim},
   journal = {arXiv:1702.08608},
   title = {Towards A Rigorous Science of Interpretable Machine Learning},
   year = {2017},
}
@article{Wolpert1992,
   author = {David H. Wolpert},
   issue = {2},
   journal = {Neural Networks},
   pages = {241-259},
   title = {Stacked Generalization},
   volume = {5},
   year = {1992},
}
@article{Pudil1994,
   author = {Pavel Pudil and Jana Novovičová and Josef Kittler},
   issue = {11},
   journal = {Pattern recognition letters},
   pages = {1119-1125},
   title = {Floating search methods in feature selection},
   volume = {15},
   year = {1994},
}
@article{Yang1997,
   author = {Yiming Yang and Jan O. Pedersen},
   journal = {International Conference on Machine Learning},
   pages = {412-420},
   title = {A Comparative Study on Feature Selection in Text Categorization},
   volume = {97},
   year = {1997},
}
@article{Dash1997,
   author = {Manoranjan Dash and Huan Liu},
   journal = {Intelligent Data Analysis},
   pages = {131-156},
   title = {Feature Selection for Classification},
   volume = {1},
   year = {1997},
}
@article{Guyon2003,
   author = {Isabelle Guyon and André Elisseeff},
   journal = {Journal of Machine Learning Research},
   pages = {1157-1182},
   title = {An Introduction to Variable and Feature Selection},
   volume = {3},
   year = {2003},
}
@article{Saeys2007,
   author = {Yvan Saeys and Iñaki Inza and Pedro Larrañaga},
   issue = {19},
   journal = {Bioinformatics},
   pages = {2507-2517},
   title = {A review of feature selection techniques in bioinformatics},
   volume = {23},
   year = {2007},
}
@article{Lam2017,
   author = {Hoang Thanh Lam and Johann-Michael Thiebaut and Mathieu Sinn and Bei Chen and Tiep Mai and Oznur Alkan},
   journal = {arXiv:1706.00327},
   pages = {1-9},
   title = {One button machine for automating feature engineering in relational databases},
   year = {2017},
}
@inproceedings{Wistuba2017,
   author = {Martin Wistuba and Nicolas Schilling and Lars Schmidt-Thieme},
   journal = {SIAM International Conference on Data Mining},
   pages = {741-749},
   title = {Automatic Frankensteining: Creating Complex Ensembles Autonomously},
   year = {2017},
}
@article{Friedman2015,
   author = {Lior Friedman and Shaul Markovitch},
   journal = {Journal of Artificial Intelligence Research},
   pages = {3-17},
   title = {Recursive Feature Generation for Knowledge-based Learning},
   volume = {1},
   year = {2015},
}
@inproceedings{Nargesian2017,
   author = {Fatemeh Nargesian and Horst Samulowitz and Udayan Khurana and Elias B. Khalil and Deepak Turaga},
   journal = {International Joint Conference on Artificial Intelligence},
   pages = {2529-2535},
   title = {Learning Feature Engineering for Classification},
   year = {2017},
}
@inproceedings{Khurana2018,
   author = {Udayan Khurana and Horst Samulowitz and Deepak Turaga},
   journal = {AAAI Conference on Artificial Intelligence},
   pages = {3407-3414},
   title = {Feature Engineering for Predictive Modeling Using Reinforcement Learning},
   year = {2018},
}
@inproceedings{Kaul2017,
   author = {Ambika Kaul and Saket Maheshwary and Vikram Pudi},
   journal = {IEEE International Conference on Data Mining},
   title = {AutoLearn - Automated Feature Generation and Selection},
   year = {2017},
}
@inproceedings{Koch2018,
   author = {Patrick Koch and Oleg Golovidov and Steven Gardner and Brett Wujek and Joshua Griffin and Yan Xu},
   journal = {ACM International Conference on Knowledge Discovery and Data Mining},
   pages = {443-452},
   title = {Autotune: A Derivative-free Optimization Framework for Hyperparameter Tuning},
   year = {2018},
}
@inproceedings{Ozaki2017,
   author = {Yoshihiko Ozaki and Masaki Yano and Masaki Onishi},
   journal = {IPSJ Transactions on Computer Vision and Applications},
   title = {Effective hyperparameter optimization using Nelder-Mead method in deep learning},
   volume = {9},
   year = {2017},
}
@article{Li2016,
   author = {Lisha Li and Kevin G. Jamieson and Giulia DeSalvo and Afshin Rostamizadeh and Ameet Talwalkar},
   journal = {arXiv:1603.06560},
   title = {Efficient Hyperparameter Optimization and Infinitely Many Armed Bandits},
   year = {2016},
}
@web_page{USU2018,
   author = {USU Software AG},
   title = {Katana},
   url = {https://katana.usu.de/},
   year = {2018},
}
@article{Gosset1908,
   author = {Student},
   issue = {1},
   journal = {Biometrika},
   pages = {1-25},
   title = {The Probable Error of a Mean},
   volume = {6},
   year = {1908},
}
@article{Rizzo2016,
   author = {Maria L. Rizzo and Gábor J. Székely},
   issue = {1},
   journal = {Wiley Interdisciplinary Reviews: Computational Statistics},
   keywords = {DISCO,Distance correlation,Goodness-of-fit,Independence,Multivariate},
   pages = {27-38},
   title = {Energy distance},
   volume = {8},
   year = {2016},
}
@article{Alaeddini2011,
   abstract = {Despite their fame and capability in detecting out-of-control conditions, control charts are not effective tools for fault diagnosis. There are other techniques in the literature mainly based on process information and control charts patterns to help control charts for root cause analysis. However these methods are limited in practice due to their dependency on the expertise of practitioners. In this study, we develop a network for capturing the cause and effect relationship among chart patterns, process information and possible root causes/assignable causes. This network is then trained under the framework of Bayesian networks and a suggested data structure using process information and chart patterns. The proposed method provides a real time identification of single and multiple assignable causes of failures as well as false alarms while improving itself performance by learning from mistakes. It also has an acceptable performance on missing data. This is demonstrated by comparing the performance of the proposed method with methods like neural nets and K-Nearest Neighbor under extensive simulation studies. © 2011 Elsevier Ltd. All rights reserved.},
   author = {Adel Alaeddini and Ibrahim Dogan},
   issue = {9},
   journal = {Expert Systems with Applications},
   keywords = {Bayesian network,Control chart patterns,Root cause analysis (RCA),Statistical process control (SPC)},
   pages = {11230-11243},
   publisher = {Elsevier Ltd},
   title = {Using Bayesian networks for root cause analysis in statistical process control},
   volume = {38},
   year = {2011},
}
@book{Rice1995,
   author = {John Rice},
   publisher = {Duxbury Press},
   title = {Mathematical Statistics and Data Analysis},
   year = {1995},
}
@book_section{Houck1995,
   author = {K. Houck and S. Calo and A. Finkel},
   journal = {Integrated Network Management IV},
   pages = {226-237},
   publisher = {Springer US},
   title = {Towards a Practical Alarm Correlation System},
   year = {1995},
}
@article{Cowley2014,
   author = {Benjamin Cowley and Giuseppe Vinci},
   journal = {Statistics Journal Club},
   pages = {1-23},
   title = {Summary and discussion of: “Brownian Distance Covariance”},
   year = {2014},
}
@article{Phillips2007,
   abstract = {We describe a variation of the iterative closest point (ICP) algorithm for aligning two point sets under a set of transformations. Our algorithm is superior to previous algorithms because (1) in determining the optimal alignment, it identifies and di...},
   author = {Jeff M. Phillips and Ran Liu and Carlo Tomasi},
   issue = {3dim},
   journal = {International Conference on 3-D Digital Imaging and Modeling},
   pages = {427-434},
   title = {Outlier robust ICP for minimizing fractional RMSD},
   year = {2007},
}
@book{Dasgupta2006,
   author = {Sanjoy Dasgupta and Christos H. Papadimitriou and Umesh V. Vazirani},
   journal = {Algorithms},
   pages = {254-255},
   publisher = {McGraw-Hill},
   title = {Algorithms},
   year = {2006},
}
@book_section{Benesty2009,
   author = {Jacob Benesty and Jingdong Chen and Yiteng Huang and Israel Cohen},
   journal = {Noise Reduction in Speech Processing},
   pages = {1 - 4},
   publisher = {Springer Berlin Heidelberg},
   title = {Pearson Correlation Coefficient},
   year = {2009},
}
@article{Benferhat2008,
   abstract = {Alert correlation is a very useful mechanism to reduce the high volume of reported alerts and to detect complex and coordinated attacks. Existing approaches either require a large amount of expert knowledge or use simple similarity measures that prevent detecting complex attacks. They also suffer from high computational issues due, for instance, to a high number of possible scenarios. In this paper, we propose a Naive Bayes approach to alert correlation. Our modeling only needs a small part of expert knowledge. It takes advantage of available historical data, and provides efficient algorithms for detecting and predicting most plausible scenarios. Our approach is illustrated using the well known DARPA 2000 data set.},
   author = {Salem Benferhat and Tayeb Kenaza and Aicha Mokhtari},
   journal = {International Computer Software and Applications Conference},
   keywords = {Alert correlation,Attack prediction,Intrusion detection,Naive bayes},
   pages = {704-709},
   title = {A Naive Bayes approach for detecting coordinated attacks},
   year = {2008},
}
@article{Spielman2004,
   abstract = {We introduce the smoothed analysis of algorithms, which continuously in- terpolates between the worst-case and average-case analyses of algorithms. In smoothed analysis, we measure the maximum over inputs of the expected performance of an algorithm under small random perturbations of that in- put. We measure this performance in terms of both the input size and the magnitude of the perturbations. We show that the simplex algorithm has smoothed complexity polynomial in the input size and the standard deviation of Gaussian perturbations.},
   author = {D. Spielman and S. Teng},
   issue = {3},
   journal = {Journal of the Association for Computing Machinery},
   pages = {385-463},
   title = {Smoothed Analysis of Algorithms: Why the Simplex Algorithm Usually Takes Polynomial Time},
   volume = {51},
   year = {2004},
}
@article{Rao1981,
   author = {J. N. K. Rao and A. J. Scott},
   issue = {374},
   journal = {Journal of the American Statistical Association},
   keywords = {completely monotone,correlation function,geostatistics,kriging,positive definite,separable,spatiotemporal},
   pages = {221-230},
   title = {The Analysis of Categorical Data From Complex Sample Surveys: Chi-Squared Tests for Goodness of Fit and Independence in Two-Way Tables},
   volume = {76},
   year = {1981},
}
@book{Reichmann1961,
   author = {W. J. Reichmann},
   publisher = {Oxford University Press},
   title = {Use And Abuse of Statistics},
   year = {1961},
}
@article{Pomerleau2015,
   author = {François Pomerleau and Francis Colas and Roland Siegwart},
   issue = {1},
   journal = {Foundations and Trends in Robotics},
   pages = {1-104},
   title = {A Review of Point Cloud Registration Algorithms for Mobile Robotics},
   volume = {4},
   year = {2015},
}
@article{Nelder1965,
   abstract = {A method is descipted for minimization of a function of n variables, which depends on the comparison of function values at the (n+1) vertices of the general simplex, followed by the replacement of the vertex with the highest value by another point. The simplex adapts itself to the local landscape, and contracts on the final minimum. The method is shown to be effective and computationally compact. A procedure is given for the estimation of the hessian matrix on the neighbourhood of the minimum, needed in statistical estimation problems.},
   author = {J. A. Nelder and R. Mead},
   journal = {Computer Journal},
   pages = {308-313},
   title = {A simplex method for function minimization},
   volume = {7},
   year = {1965},
}
@web_page{Glira2016,
   author = {Philipp Glira},
   title = {Iterative Closest Point (ICP)},
   url = {https://www.youtube.com/watch?v=uzOCS_gdZuM},
   year = {2016},
}
@article{Jakobson1993,
   author = {Gabriel Jakobson and Mark D. Weissman},
   issue = {6},
   journal = {IEEE Network: The Magazine of Global Internetworking},
   pages = {52-59},
   title = {Alarm Correlation},
   volume = {7},
   year = {1993},
}
@book{Brigham1974,
   author = {Elbert Oran Brigham},
   city = {Englewood Cliffs, New Jersey},
   isbn = {O-13-301496-X},
   pages = {7},
   publisher = {Prentice-Hall, Inc},
   title = {The Fast Fourier Transform},
   year = {1974},
}
@article{Hassin1994,
   author = {Refael Hassin and Shlomi Rubinstein},
   issue = {3},
   journal = {Information Processing Letters},
   pages = {133-140},
   title = {Approximations for the maximum acyclic subgraph problem},
   volume = {51},
   year = {1994},
}
@thesis{Margaritis2003,
   abstract = {In this thesis I address the important problem of the determination of the structure of directed statistical models, with the widely used class of Bayesian network models as a concrete vehicle of my ideas. The structure of a Bayesian network represents a set of conditional independence relations that hold in the domain. Learning the structure of the Bayesian network model that represents a domain can reveal insights into its underlying causal structure. Moreover, it can also be used for prediction of quantities that are difficult, expensive, or unethical to measure— such as the probability of lung cancer for example—based on other quantities that are easier to obtain. The contributions of this thesis include (a) an algorithm for determining the structure of a Bayesian network model from statistical independence statements; (b) a statistical independence test for continuous variables; and finally (c) a practical application of structure learning to a decision support problem, where a model learned from the database—most importantly its structure—is used in lieu of the database to yield fast approximate answers to count queries, surpassing in certain aspects other state-of-the-art approaches to the same problem.},
   author = {Dimitris Margaritis},
   issue = {May},
   institution = {Carnegie Mellon University},
   keywords = {Bayesian network structure learning,Bayesian networks,DataCube approximation,Markov blanket,causal discovery,continuous variable independence test,database count queries.},
   title = {Learning Bayesian Network Model Structure from Data},
   year = {2003},
}
@article{Dragomir2003,
   author = {Sever Dragomir},
   issue = {3},
   journal = {Journal of Inequalities in Pure and Applied Mathematics},
   pages = {1-142},
   title = {A survey on Cauchy-Bunyakovsky-Schwarz type discrete inequalities.},
   volume = {4},
   year = {2003},
}
@article{White2009,
   abstract = {Methods to monitor spatial patterns of disease in populations are of interest in public health practice. The M statistic uses interpoint distances between cases to detect abnormalities in the spatial patterns of diseases. This statistic compares the observed distribution of interpoint distances with that which is expected when no unusual spatial patterns exist. We show the relationship of M to Pearson's Chi Square statistic, Xn2. Both statistics require the discretization of continuous data into bins and then are formed by creating a quadratic form, scaled by an appropriate variance covariance matrix. We seek to choose the number and type of these bins for the M statistic so as to maximize the power to detect spatial anomalies. By showing the relationship between M to Xn2, we argue for the extension of the theory that has been developed for the selection of the number and type of bins for Xn2 to M. We further show that spatial data provides a unique insight into the problem through examples with simulated data and spatial data from a health care provider. In the spatial setting, these indicate that the optimal number of bins depends on the size of the cluster. For large clusters, a smaller number of bins appears to be preferable, however for small clusters having many bins increases the power. Further, results indicate that the number of bins does not appear to vary with m, the number of spatial locations. We discuss the implications of this result for further work. ?? 2009 Elsevier B.V. All rights reserved.},
   author = {Laura Forsberg White and Marco Bonetti and Marcello Pagano},
   issue = {10},
   journal = {Computational Statistics and Data Analysis},
   keywords = {dependent data,distances,pearson,s chi square statistic,spatial statistics,surveillance},
   pages = {3640-3649},
   title = {The choice of the number of bins for the M statistic},
   volume = {53},
   year = {2009},
}
@article{Niculescu2004,
   author = {Constantin P. Niculescu and Lars-Erik Persson},
   title = {Convex Functions and Their Applications: A Contemporary Approach},
   year = {2004},
}
@article{DeMaesschalck20001,
   abstract = {The theory of many multivariate chemometrical methods is based on the measurement of distances. The Mahalanobis distance (MD), in the original and principal component (PC) space, will be examined and interpreted in relation with the Euclidean distance (ED). Techniques based on the \{MD\} and applied in different fields of chemometrics such as in multivariate calibration, pattern recognition and process control are explained and discussed.},
   author = {R. De. Maesschalck and D. L. Massart},
   issue = {1},
   journal = {Chemometrics and Intelligent Laboratory Systems},
   keywords = {euclidean distance,mahalanobis distance,principal components},
   pages = {1-18},
   title = {The Mahalanobis distance},
   volume = {50},
   year = {2000},
}
@inproceedings{Rusu2009,
   abstract = {In our recent work [1], [2], we proposed Point Feature Histograms (PFH) as robust multi-dimensional features which describe the local geometry around a point p for 3D point cloud datasets. In this paper, we modify their mathematical expressions and perform a rigorous analysis on their robustness and complexity for the problem of 3D registration for overlapping point cloud views. More concretely, we present several optimizations that reduce their computation times drastically by either caching previously computed values or by revising their theoretical formulations. The latter results in a new type of local features, called Fast Point Feature Histograms (FPFH), which retain most of the discriminative power of the PFH. Moreover, we propose an algorithm for the online computation of FPFH features for realtime applications. To validate our results we demonstrate their efficiency for 3D registration and propose a new sample consensus based method for bringing two datasets into the convergence basin of a local non-linear optimizer: SAC-IA (SAmple Consensus Initial Alignment).},
   author = {Radu Bogdan Rusu and Nico Blodow and Michael Beetz},
   journal = {IEEE International Conference on Robotics and Automation},
   pages = {3212-3217},
   title = {Fast Point Feature Histograms (FPFH) for 3D registration},
   year = {2009},
}
@article{Do2008,
   author = {Chuong B Do and Serafim Batzoglou},
   issue = {8},
   journal = {Nature Biotechnology},
   pages = {897-899},
   title = {What is the expectation maximization algorithm?},
   volume = {26},
   year = {2008},
}
@article{Mannila1997,
   abstract = {Sequences of events describing the behavior and actions of users or systems can be collected in several domains. An episode is a collection of events that occur relatively close to each other in a given partial order. We consider the problem of discovering frequently occurring episodes in a sequence. Once such episodes are known, one can produce rules for describing or predicting the behavior of the sequence. We give efficient algorithms for the discovery of all frequent episodes from a given class of episodes, and present detailed experimental results. The methods are in use in telecommunication alarm management.},
   author = {Heikki Mannila and Hannu Toivonen and A. Inkeri Verkamo},
   issue = {3},
   journal = {Data Mining and Knowledge Discovery},
   keywords = {event sequences,frequent episodes,sequence analysis},
   pages = {259-289},
   title = {Discovery of Frequent Episodes in Event Sequences},
   volume = {1},
   year = {1997},
}
@article{Dempster1977,
   author = {A.P. Dempster and N.M. Laird and Donald B. Rubin},
   issue = {1},
   journal = {Journal of the Royal Statistical Society},
   pages = {1-38},
   title = {Maximum Likelihood from Incomplete Data via the EM Algorithm},
   volume = {39},
   year = {1977},
}
@article{Cobb2006,
   author = {Barry R. Cobb and Prakash P. Shenoy},
   issue = {1-2},
   journal = {International Journal of Approximate Reasoning},
   pages = {21-36},
   title = {Operations for inference in continuous Bayesian networks with linear deterministic variables},
   volume = {42},
   year = {2006},
}
@article{Tang2012,
   abstract = {Time lag is a key feature of hidden temporal dependencies within sequential data. In many real-world applications, time lag plays an essential role in interpreting the cause of discovered temporal dependencies. Traditional temporal mining methods either use a predefined time window to analyze the item sequence, or employ statistical techniques to simply derive the time dependencies among items. Such paradigms cannot effectively handle varied data with special properties, e.g., the interleaved temporal dependencies. In this paper, we study the problem of finding lag intervals for temporal dependency analysis. We first investigate the correlations between the temporal dependencies and other temporal patterns, and then propose a generalized framework to resolve the problem. By utilizing the sorted table in representing time lags among items, the proposed algorithm achieves an elegant balance between the time cost and the space cost. Extensive empirical evaluation on both synthetic and real data sets demonstrates the efficiency and effectiveness of our proposed algorithm in finding the temporal dependencies with lag intervals in sequential data.},
   author = {Liang Tang and Tao Li and Larisa Shwartz},
   journal = {ACM International Conference on Knowledge Discovery and Data Mining},
   keywords = {temporal dependency,time lag},
   pages = {633},
   title = {Discovering lag intervals for temporal dependencies},
   year = {2012},
}
@article{Benferhat,
   author = {Salem Benferhat and Tayeb Kenaza},
   journal = {IEEE International Computer Software and Applications},
   title = {Causality and intervention for alarm correlation : A Naive Bayes approach for detecting coordinated attacks},
   year = {2008},
}
@article{Stewart2003,
   author = {Charles V. Stewart and Chia-Ling Tsai and Badrinath Roysam},
   issue = {11},
   journal = {IEEE Transactions on Medical Imaging},
   keywords = {Algorithms,Automated,Computer-Assisted,Computer-Assisted: methods,Fluorescein Angiography,Fluorescein Angiography: methods,Humans,Image Enhancement,Image Enhancement: methods,Image Interpretation,Pattern Recognition,Reproducibility of Results,Retina,Retina: anatomy & histology,Retinal Diseases,Retinal Diseases: diagnosis,Retinal Vessels,Retinal Vessels: anatomy & histology,Sensitivity and Specificity,Subtraction Technique},
   pages = {1379-1394},
   title = {The dual-bootstrap iterative closest point algorithm with application to retinal image registration.},
   volume = {22},
   year = {2003},
}
@article{Marvasti2013,
   author = {Mazda A. Marvasti and Arnak V. Poghosyan and Ashot N. Harutyunyan and Naira M. Grigoryan},
   issue = {JUNE},
   journal = {VMWARE TECHNICAL JOURNAL},
   pages = {35-45},
   title = {An Anomaly Event Correlation Engine : Identifying Root Causes , Bottlenecks , and Black Swans in IT Environments},
   volume = {2},
   year = {2013},
}
@article{Ezra2008,
   author = {Esther Ezra and Micha Sharir and Alon Efrat},
   issue = {1},
   journal = {Computational Geometry},
   pages = {77-93},
   title = {On the performance of the ICP algorithm},
   volume = {41},
   year = {2008},
}
@article{Pradhan2007,
   abstract = {We describe an Early Warning System (EWS) which enables the root-cause-analysis for initiating quality improvements in the manufacturing shop floor and process-engineering departments, at product OEMs as well as their tiered suppliers. The EWS combines the use of custom-designed domain ontology of manufacturing processes and failure related knowledge, innovative application of domain knowledge in the form of probability constraints and a novel two-step constrained optimization approach to causal network construction. Probabilistic reasoning is the main vehicle for inference from the causal network. This inference engine provides the capability to do a root-cause-analysis in manufacturing scenarios, and is thus a powerful weapon for an automotive EWS. This technique is widely applicable and can be used in various contexts in the broader manufacturing industry as well.},
   author = {S. Pradhan and R. Singh and K. Kachru and S. Narasimhamurthy},
   journal = {nternational Conference on Computational Intelligence and Security},
   pages = {10-14\r1082},
   title = {A Bayesian network based approach for root-cause-analysis in manufacturing process},
   year = {2007},
}
@generic{So2008,
   abstract = {While Bessel's correction for the sample variance is well known and quoted abundantly in statistics' texts, a detailed treatment of why the correction is needed at all, does not appear to be prominently mentioned, other than a cursory statement to the effect that the estimator is biased without the correction. In this article, we present a mathematical treatment of the 'uncorrected' sample variance and explain why it is a biased estimator of the true variance of a population. This will be of interest to readers who are studying or have studied statistics but whom cannot find the real reason for Bessel's correction. The reader is assumed to have some prior knowledge of statistics and probability, particularly in relation to random variables and the mathematical expectation operator.},
   author = {Stephen So},
   keywords = {Bessel's correction,Index terms,biased estimator,sample variance},
   pages = {1-4},
   title = {Why is the sample variance a biased estimator?},
   year = {2008},
}
@inproceedings{Gopal2000,
   author = {Rajeev Gopal},
   journal = {Network Operations and Management Symposium},
   keywords = {and recovery,fault detection,fault management,isolation,modeling},
   pages = {729-742},
   publisher = {IEEE},
   title = {Layered model for supporting fault isolation and recovery},
   year = {2000},
}
@inproceedings{Bouandas2007,
   author = {Khellaf Bouandas and Aomar Osmani},
   journal = {IEEE Symposium on Computational Intelligence and Data Mining},
   pages = {610-615},
   title = {Mining Association Rules in Temporal Sequences},
   year = {2007},
}
@inproceedings{Chetverikov2002,
   abstract = {The problem of geometric alignment of two roughly preregistered, partially overlapping, rigid, noisy 3D point sets is considered. A new natural and simple, robustified extension of the popular Iterative Closest Point (ICP) algorithm (Besl and McKay, 1992) is presented, called the Trimmed ICP (TrICP). The new algorithm is based on the consistent use of the least trimmed squares (LTS) approach in all phases of the operation. Convergence is proved and an efficient implementation is discussed. TrICP is fast, applicable to overlaps under 50%, robust to erroneous measurements and shape defects, and has easy-to-set parameters. ICP is a special case of TrICP when the overlap parameter is 100%. Results of testing the new algorithm are shown.},
   author = {D. Chetverikov and D. Svirko and D. Stepanov and P. Krsek},
   journal = {International Conference on Pattern Recognition},
   pages = {545-548},
   publisher = {IEEE},
   title = {The Trimmed Iterative Closest Point algorithm},
   volume = {3},
   year = {2002},
}
@book{Russell2010,
   author = {Stuart J. Russell and Peter Norvig},
   edition = {3},
   pages = {524-528},
   publisher = {Pearson Education},
   title = {Artificial Intelligence: A Modern Approach},
   year = {2010},
}
@article{Bowman1984,
   author = {Adrian W. Bowman},
   issue = {2},
   journal = {Biometrika},
   pages = {353-360},
   title = {An alternative method of cross-validation for the smoothing of density estimates},
   volume = {71},
   year = {1984},
}
@article{Murty1987,
   abstract = {In continuous variable, smooth, nonconvex nonlinear programming, we analyze the complexity of checking whether (a) a given feasible solution is not a local minimum, and (b) the objective function is not bounded below on the set of feasible solutions. We construct a special class of indefinite quadratic programs, with simple constraints and integer data, and show that checking (a) or (b) on this class is NP-complete. As a corollary, we show that checking whether a given integer square matrix is not copositive, is NP-complete.},
   author = {Katta G. Murty and Santosh N. Kabadi},
   issue = {2},
   journal = {Mathematical Programming},
   keywords = {NP-complete,Nonconvex nonlinear programming,copositive matrices,global minimum,local minimum},
   pages = {117-129},
   title = {Some NP-complete problems in quadratic and nonlinear programming},
   volume = {39},
   year = {1987},
}
@book{Papadimitriou1994,
   author = {Christos H. Papadimitriou},
   journal = {Computational Complexity},
   pages = {76-78},
   publisher = {Addison Wesley Longman},
   title = {Computational Complexity},
   year = {1994},
}
@inproceedings{Zhou2015,
   author = {Wubai Zhou and Tao Li and Larisa Shwartz and Genady Ya Grabarnik},
   journal = {International Conference on Network and Service Management},
   pages = {15-21},
   publisher = {IEEE},
   title = {Recommending Ticket Resolution using Feature Adaptation},
   year = {2015},
}
@article{Marvasti2013a,
   abstract = {Data-agnostic management of today's virtualized and cloud IT infrastructures motivates statistical inference from unstructured or semi-structured data. We introduce a universal approach to the determination of statistically relevant patterns in unstructured data, and then showcase its application to log data of a Virtual Center (VMware's virtualization management software). The premise of this study is that the unstructured data can be converted into events, where an event is defined by time, source, and a series of attributes. Every event can have any number of attributes but all must have a time stamp and optionally a source of origination (be it a server, a location, a business process, etc.) The statistical relevance of the data can then be made clear via determining the joint and prior probabilities of events using a discrete probability computation. From this we construct a Directed Virtual Graph with nodes representing events and the branches representing the conditional probabilities between two events. Employing information-theoretic measures the graphs are reduced to a subset of relevant nodes and connections. Moreover, the information contained in the unstructured data set is extracted from these graphs by detecting particular patterns of interest.},
   author = {Mazda a. Marvasti and Arnak V. Poghosyan and Ashot N. Harutyunyan and Naira M. Grigoryan},
   journal = {Integrated Network Management},
   keywords = {Fault management,directed graph,event correlation,pattern detection,unstructured data},
   pages = {1048-1053},
   title = {Pattern detection in unstructured data: An experience for a virtualized IT infrastructure},
   year = {2013},
}
@article{Cooper1990,
   abstract = {Bayesian belief networks provide a natural, efficient method for representing probabilistic dependen- cies among a set of variables. For these reasons, numerous researchers are exploring the use of belief networks as a knowledge representation m artificial intelligence. Algorithms have been developed previously for efficient probabilistic inference using special classes of belief networks. More general classes of belief networks, however, have eluded efforts to develop efficient inference algorithms. We show that probabilistic inference using belief networks is NP-hard. Therefore, it seems unlikely that an exact algorithm can be developed to perform probabilistic inference efficiently over all classes of belief networks. This result suggests that research should be directed away from the search for a general, efficient probabilistic inference algorithm, and toward the design of efficient special-case, average-case, and approximation algorithms.},
   author = {Gregory F. Cooper},
   issue = {2-3},
   journal = {Artificial Intelligence},
   pages = {393-405},
   title = {The Computational Complexity of Probabilistic Inference Using Bayesian Belief Networks (Research Note)},
   volume = {42},
   year = {1990},
}
@article{Yao1998,
   author = {Qiwei Yao and Howell Tong},
   issue = {2},
   journal = {Journal of Statistical Planning and Inference},
   pages = {387-415},
   title = {Cross-Validatory Bandwidth Selections For Regression Estimation Based on Dependent Data},
   volume = {68},
   year = {1998},
}
@article{Fischler1981,
   author = {Martin A. Fischler and Robert C. Bolles},
   issue = {6},
   journal = {Communications of the ACM},
   keywords = {automated cartography,camera calibration,image matching,location determination,model fitting,scene analysis},
   pages = {381-395},
   title = {Random Sample Consensus: A Paradigm for Model Fitting with Applications to Image Analysis and Automated Cartography},
   volume = {24},
   year = {1981},
}
@article{Munkres1957,
   author = {James Munkres},
   journal = {Society for Industrial and Applied Mathematics},
   pages = {32-38},
   title = {Algorithms for the Assignment and Transportation Problem},
   volume = {5},
   year = {1957},
}
@article{Shannon1951,
   author = {C. E. Shannon},
   issue = {1},
   journal = {Bell System Technical Journal},
   pages = {50-64},
   title = {Prediction and Entropy of Printed English},
   volume = {30},
   year = {1951},
}
@article{Harutyunyan2014,
   abstract = {We examine the determination of abnormality of streamed data using the statistical structure of the meta-data associated with it. The vital need for such a subject within a heterogeneous log based environment in real-time comes from the fact that most cloud based applications will use text-based logging as a means of reporting application behavior. The sheer volume of such logs makes retrospective analysis infeasible due to large processing and storage requirements. Our approach is based on conversion of the original data stream into meta-data (graph) and revealing the dominating (normal) statistical patterns within it. Real-time analysis of the stream compared with the meta-data model determines the degree of anomaly of the current data. The resulting graph also reveals the fundamental structure (“behavioral footprint”) of the data beyond the sources (physical or virtual devices) and processes.},
   author = {Ashot N. Harutyunyan and Arnak V. Poghosyan and Naira M. Grigoryan and Mazda A. Marvasti},
   issue = {May},
   journal = {IEEE/IFIP Network Operations and Management Symposium: Management in a Software Defined World},
   keywords = {Cloud and virtualization management,anomaly and change detection,big data,events stream,log analysis,normalcy structure},
   title = {Abnormality analysis of streamed log data},
   year = {2014},
}
@article{Fu2011,
   abstract = {If f is a function of n variables that is locally L1 approximable by a sequence of smooth functions satisfying local L1 bounds on the determinants of the minors of the Hessian, then f admits a second order Taylor expansion almost everywhere. This extends a classical theorem of A.D. Alexandrov, covering the special case in which f is locally convex. ?? 2011 Elsevier Inc.},
   author = {J. Fu},
   issue = {4},
   journal = {Advances in Mathematics},
   keywords = {Second derivatives,Weak derivatives},
   pages = {2258-2267},
   title = {An extension of Alexandrov's theorem on second derivatives of convex functions},
   volume = {228},
   year = {2011},
}
@web_page{ThePennsylvaniaStateUniversity2017,
   author = {The Pennsylvania State University},
   title = {Hypothesis Testing},
   url = {https://onlinecourses.science.psu.edu/statprogram/node/138},
   year = {2017},
}
@book{Scott1992,
   author = {David W. Scott},
   city = {New York},
   publisher = {Wiley-Interscience},
   title = {Multivariate Density Estimation : Theory, Practice, and Visualization},
   year = {1992},
}
@inproceedings{Kettschau2002,
   author = {H.-J. Kettschau and S. Bruck and P. Schefczik},
   journal = {Network Operations and Management Symposium},
   keywords = {alarm correlation,fault management,operation and maintenance centcr,radio access nclwork},
   pages = {903-905},
   publisher = {IEEE},
   title = {LUCAS - an Expert System for Intelligent Fault Management and Alarm Correlation},
   year = {2002},
}
@article{Szekely2009,
   abstract = {Distance correlation is a new class of multivariate dependence coefficients applicable to random vectors of arbitrary and not necessarily equal dimension. Distance covariance and distance correlation are analogous to product-moment covariance and correlation, but generalize and extend these classical bivariate measures of dependence. Distance correlation characterizes independence: it is zero if and only if the random vectors are independent. The notion of covariance with respect to a stochastic process is introduced, and it is shown that population distance covariance coincides with the covariance with respect to Brownian motion; thus, both can be called Brownian distance covariance. In the bivariate case, Brownian covariance is the natural extension of product-moment covariance, as we obtain Pearson product-moment covariance by replacing the Brownian motion in the definition with identity. The corresponding statistic has an elegantly simple computing formula. Advantages of applying Brownian covariance and correlation vs the classical Pearson covariance and correlation are discussed and illustrated.},
   author = {Gábor J. Székely and Maria L. Rizzo},
   issue = {4},
   journal = {The Annals of Applied Statistics},
   keywords = {Brownian covariance,Dcor,Distance correlation,Independence,Multivariate},
   pages = {1236-1265},
   title = {Brownian distance covariance},
   volume = {3},
   year = {2009},
}
@book{Cover2005,
   abstract = {Following a brief introduction and overview, early chapters cover the basic algebraic relationships of entropy, relative entropy and mutual information, AEP, entropy rates of stochastics processes and data compression, duality of data compression and the growth rate of wealth. Later chapters explore Kolmogorov complexity, channel capacity, differential entropy, the capacity of the fundamental Gaussian channel, the relationship between information theory and statistics, rate distortion and network information theories. The final two chapters examine the stock market and inequalities in information theory. In many cases the authors actually describe the properties of the solutions before the presented problems.},
   author = {Thomas M. Cover and Joy A. Thomas},
   journal = {Elements of Information Theory},
   pages = {13-14, 243-248},
   publisher = {John Wiley & Sons, Inc.},
   title = {Elements of Information Theory},
   year = {2006},
}
@article{Fuqiang2015,
   author = {Chen Fuqiang},
   keywords = {icle},
   title = {An Improved Expectation Maximization Algorithm},
   volume = {1},
   year = {2015},
}
@article{Besl1992,
   abstract = {The authors describe a general-purpose, representation-independent method for the accurate and computationally efficient registration of 3-D shapes including free-form curves and surfaces. The method handles the full six degrees of freedom and is based on the iterative closest point (ICP) algorithm, which requires only a procedure to find the closest point on a geometric entity to a given point. The ICP algorithm always converges monotonically to the nearest local minimum of a mean-square distance metric, and the rate of convergence is rapid during the first few iterations. Therefore, given an adequate set of initial rotations and translations for a particular class of objects with a certain level of 'shape complexity', one can globally minimize the mean-square distance metric over all six degrees of freedom by testing each initial registration. One important application of this method is to register sensed data from unfixtured rigid objects with an ideal geometric model, prior to shape inspection. Experimental results show the capabilities of the registration algorithm on point sets, curves, and surfaces.},
   author = {Paul J. Besl and Neil D. McKay},
   issue = {2},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   keywords = {3D shape registration,computational geometry,convergence,convergence of numerical methods,geometric entity,geometric model,iterative closest point,iterative methods,mean-square distance metric,optimisation,pattern recognition,picture processing,point set registration},
   pages = {239-256},
   title = {A Method for Registration of 3-D Shapes},
   volume = {14},
   year = {1992},
}
@article{MurrayRosenblatt1956,
   author = {Murray Rosenblatt},
   issue = {3},
   journal = {The Annals of Mathematical Statistics},
   pages = {832-837},
   title = {Remarks on Some Nonparametric Estimates of a Density Function},
   volume = {27},
   year = {1956},
}
@book{Lehmann2008,
   author = {Erich Leo Lehmann and Joseph P. Romano},
   edition = {3},
   pages = {63-65, 81-83},
   publisher = {Springer New York},
   title = {Testing Statistical Hypotheses},
   year = {2008},
}
@inproceedings{Katz2017,
   author = {Gilad Katz and Eui Chul Richard Shin and Dawn Song},
   journal = {IEEE International Conference on Data Mining},
   pages = {979-984},
   title = {ExploreKit: Automatic feature generation and selection},
   year = {2017},
}
@inproceedings{DeSa2017,
   author = {Alex G. C. de Sá and Walter José G. S. Pinto and Luiz Otávio V. B. Oliveira and Gisele L. Pappa},
   booktitle = {European Conference on Genetic Programming},
   pages = {246-261},
   title = {RECIPE: A Grammar-Based Framework for Automatically Evolving Classification Pipelines},
   volume = {10196},
   year = {2017},
}
@inproceedings{Guyon2016,
   author = {Isabelle Guyon and Imad Chaabane and Hugo Jair Escalante and Sergio Escalera and Damir Jajetic and James Robert Lloyd and Núria Maciá and Bisakha Ray and Lukasz Romaszko and Michéle Sebag and Alexander Statnikov and Sébastien Treguer and Evelyne Viegas},
   journal = {International Conference on Machine Learning AutoML Workshop},
   pages = {21-30},
   title = {A brief Review of the ChaLearn AutoML Challenge: Any-time Any-dataset Learning without Human Intervention},
   year = {2016},
}
@article{Anderson2017,
   author = {Alec W. Anderson},
   title = {Deep Mining : Scaling Bayesian Auto-tuning of Data Science Pipelines by},
   year = {2017},
}
@article{Guyon2015,
   author = {Isabelle Guyon and Kristin Bennett and Gavin Cawley and Hugo Jair Escalante and Sergio Escalera and Tin Kam Ho and Núria Maciá and Bisakha Ray and Mehreen Saeed and Alexander Statnikov and Evelyne Viegas},
   journal = {International Joint Conference on Neural Networks},
   pages = {1-8},
   title = {Design of the 2015 ChaLearn AutoML Challenge},
   year = {2015},
}
@inproceedings{Chen2018,
   author = {Boyuan Chen and Harvey Wu and Warren Mo and Ishanu Chattopadhyay and Hod Lipson},
   journal = {Genetic and Evolutionary Computation Conference},
   pages = {402–409},
   publisher = {Association for Computing Machinery},
   title = {Autostacker: A Compositional Evolutionary Learning System},
   year = {2018},
}
@article{Hutter2009,
   author = {Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown and Thomas Stützle},
   journal = {Journal of Artificial Intelligence Research},
   pages = {267-306},
   title = {ParamILS: An Automatic Algorithm Configuration Framework},
   volume = {36},
   year = {2009},
}
@book_section{Birattari2010,
   author = {Mauro Birattari and Zhi Yuan and Thomas Stützle and Prasanna Balaprakash},
   journal = {Experimental Methods for the Analysis of Optimization Algorithms},
   pages = {311-336},
   publisher = {Springer Berlin Heidelberg},
   title = {Experimental Methods for the Analysis of Optimization Algorithms},
   year = {2010},
}
@article{Kotthoff2016,
   author = {Lars Kotthoff and Chris Thornton and Holger H. Hoos and Frank Hutter and Kevin Leyton-Brown},
   journal = {Journal of Machine Learning Research},
   pages = {1-5},
   title = {Auto-WEKA 2.0: Automatic model selection and hyperparameter optimization in WEKA},
   volume = {17},
   year = {2016},
}
@inproceedings{Thornton2013,
   author = {Chris Thornton and Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown},
   booktitle = {ACM International Conference on Knowledge Discovery and Data Mining},
   pages = {847-855},
   title = {Auto-WEKA: Combined Selection and Hyperparameter Optimization of Classification Algorithms},
   year = {2013},
}
@inproceedings{Swearingen2017,
   author = {Thomas Swearingen and Will Drevo and Bennett Cyphers and Alfredo Cuesta-Infante and Arun Ross and Kalyan Veeramachaneni},
   journal = {IEEE International Conference on Big Data},
   pages = {151-162},
   title = {ATM: A distributed, collaborative, scalable system for automated machine learning},
   year = {2017},
}
@inproceedings{Kanter2015,
   author = {James Max Kanter and Kalyan Veeramachaneni},
   journal = {IEEE International Conference on Data Science and Advanced Analytics},
   pages = {1-10},
   title = {Deep Feature Synthesis: Towards Automating Data Science Endeavors},
   year = {2015},
}
@inproceedings{Hutter2011,
   author = {Frank Hutter and Holger H Hoos and Kevin Leyton-Brown},
   booktitle = {LION},
   pages = {507-523},
   title = {Sequential Model-Based Optimization for General Algorithm Configuration},
   year = {2011},
}
@inproceedings{Olson2016a,
   author = {Randal S. Olson and Nathan Bartley and Ryan J. Urbanowicz and Jason H. Moore},
   journal = {Genetic and Evolutionary Computation Conference},
   pages = {485-492},
   title = {Evaluation of a Tree-based Pipeline Optimization Tool for Automating Data Science},
   year = {2016},
}
@inproceedings{Feurer2015,
   author = {Matthias Feurer and Aaron Klein and Katharina Eggensperger and Jost Tobias Springenber and Manuel Blum and Frank Hutter},
   booktitle = {NeurIPS},
   pages = {2755-2763},
   title = {Efficient and Robust Automated Machine Learning},
   year = {2015},
}
@inproceedings{Olson2016,
   author = {Randal S. Olson and Jason H. Moore},
   booktitle = {International Conference on Machine Learning AutoML Workshop},
   pages = {66-74},
   publisher = {Springer International Publishing},
   title = {TPOT: A Tree-based Pipeline Optimization Tool for Automating Machine Learning},
   year = {2016},
}
@inproceedings{Olson2016b,
   author = {Randal S. Olson and Ryan J. Urbanowicz and Peter C. Andrews and Nicole A. Lavender and La Creis Kidd and Jason H. Moore},
   journal = {Applications of Evolutionary Computation},
   pages = {123-137},
   publisher = {Springer International Publishing},
   title = {Automating biomedical data science through tree-based pipeline optimization},
   year = {2016},
}
@article{Vmware2014,
   author = {Ashot N Harutyunyan Vmware and Arnak Poghosyan and National Academy and Naira Grigoryan Vmware},
   issue = {May 2016},
   keywords = {data categorization,dynamic thresholding,monitoring,normalcy determination,parametric and non-parametric statistics,statistical process control,time series data},
   title = {Statistical Normalcy Determination based on Data Categorization},
   year = {2014},
}
@article{Friedman1997,
   author = {Nir Friedman and Dan Geiger and Moises Goldszmit},
   issue = {2},
   journal = {Machine Learning},
   pages = {131-163},
   title = {Bayesian Network Classifiers},
   volume = {29},
   year = {1997},
}
@book{Lehmann2014,
   author = {E.L. Lehmann and Joseph P. Romano},
   issue = {1},
   journal = {Igarss},
   keywords = {Bott},
   pages = {1-5},
   publisher = {Springer New York},
   title = {Testing Statistical Hypotheses},
   year = {2014},
}
@article{Blomer2013,
   author = {J. Blömer and K. Bujna},
   journal = {arXiv: 1312.5946},
   title = {Simple Methods for Initializing the EM Algorithm for Gaussian Mixture Models},
   year = {2013},
}
@inproceedings{Zeng2015,
   author = {Chunqiu Zeng and Liang Tang and Tao Li and Larisa Shwartz and Genady Ya Grabarnik},
   journal = {International Conference on Network and Service Management},
   pages = {19-27},
   title = {Mining temporal lag from fluctuating events for correlation and root cause analysis},
   year = {2015},
}
@inproceedings{Arora2002,
   abstract = {Proving integrality gaps for linear relaxations of NP optimization problems is a difficult task and usually undertaken on a case-by-case basis. We initiate a more systematic approach. We prove an integrality gap of 2-o(1) for three families of linear relaxations for vertex cover, and our methods seem relevant to other problems as well.},
   author = {Sanjeev Arora and Béla Bollobás and László Lovász},
   journal = {IEEE Symposium on Foundations of Computer Science},
   pages = {313-322},
   title = {Proving Integrality Gaps without Knowing the Linear Program},
   year = {2002},
}
@inproceedings{Li2004,
   author = {T. Li},
   journal = {IEEE International Conference on Data Mining},
   pages = {451-454},
   title = {Mining Temporal Patterns Without Predefined Time Windows},
   year = {2004},
}
@article{Bouillard2013,
   abstract = {Abstract: Nowadays telecommunication systems are growing more and more complex, generating huge amount of alarms that cannot be effectively managed by human operators. The problematic is to detect in real-time significant combinations of alarms that describe an issue. In this article, we present a powerful heuristic algorithm that constructs alarm patterns dependency graphs. More precisely, it is able to highlight patterns extracted from an alarm flow learning process with a small footprint on network management system performance. This algorithm is first relevant to real-time issues detection by effectively delivering their concise alarm patterns. And secondly it allows the proactive analysis of network health by retrieving the general trends of a network. We challenge our algorithm to an optical network alarms data set of an existing operator. We find immediately similar results to the experts analysis performed for this operator by Alcatel-Lucent Customer Services.},
   author = {Anne Bouillard and Aurore Junier and Benoit Ronot},
   pages = {17},
   title = {Alarms Correlation in Telecommunication Networks},
   year = {2013},
}
@article{Babaud1986,
   author = {Jean Babaud and Andrew P. Witkin and Michel Baudin and Richard O. Duda},
   issue = {1},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   pages = {26-33},
   title = {Uniqueness of the Gaussian Kernel for Scale-Space Filtering},
   volume = {PAMI-8},
   year = {1986},
}
@article{Raykar2006,
   author = {Vikas Chandrakant Raykar and Ramani Duraiswami},
   journal = {Technical Reports from UMIACS},
   pages = {522-526},
   title = {Very fast optimal bandwidth selection for univariate kernel density estimation},
   year = {2006},
}
@article{MolineroVelasco2012,
   author = {Javier Molinero Velasco},
   issue = {2},
   journal = {Artificial Intelligence Research},
   pages = {75-85},
   title = {A Bayesian Network approach to diagnosing the root cause of failure from Trouble Tickets},
   volume = {1},
   year = {2012},
}
@web_page{Garcia2010,
   abstract = {This is a three-section tutorial on correlation coefficients. Section one discusses the proper way of computing r values. Section two describes statistical applications. Section three discusses recent research on the problem of correlation coefficients as biased estimators.},
   author = {E. Garcia},
   pages = {1},
   title = {A Tutorial on Correlation Coefficients},
   url = {https://pdfs.semanticscholar.org/c3e1/095209d3f72ff66e07b8f3b152fab099edea.pdf},
   year = {2010},
}
@article{Efron2013,
   author = {Bradley Efron},
   issue = {6137},
   journal = {Science},
   pages = {1177-1178},
   title = {Bayes' Theorem in the 21st Century},
   volume = {340},
   year = {2013},
}
@article{Solis1981,
   author = {Francisco J. Solis and Roger J.-B. Wets},
   issue = {1},
   journal = {Mathematics of Operations Research},
   pages = {19-30},
   title = {Minimization By Random Search Techniques},
   volume = {6},
   year = {1981},
}
@article{Hesterman2010,
   author = {Jacob Y. Hesterman and Luca Caucci and Matthew A. Kupinski and Harrison H. Barrett and Lars R. Furenlid},
   issue = {3},
   journal = {IEEE Transactions on Nuclear Science},
   pages = {1077-1084},
   title = {Maximum-Likelihood Estimation With a Contracting-Grid Search Algorithm},
   volume = {57},
   year = {2010},
}
@article{LaValle2004,
   author = {Steven M. LaValle and Michael S. Branicky and Stephen R. Lindemann},
   journal = {The International Journal of Robotics Research},
   keywords = {algorithms,carlo,discrepancy,motion planning,path planning,probabilistic roadmaps,quasi-monte,robotics research,sampling-based motion planning,the international journal of},
   pages = {673-692},
   title = {On the Relationship Between Classical Grid Search and Probabilistic Roadmaps},
   volume = {23},
   year = {2004},
}
@report{Hsu2003,
   author = {Chih-Wei Hsu and Chih-Chung Chang and Chih-Jen Lin},
   institution = {Department of Computer Science, National Taiwan University},
   title = {A Practical Guide to Support Vector Classification},
   year = {2003},
}
@inproceedings{Snoek2012,
   author = {Jasper Snoek and Hugo Larochelle and Ryan P. Adams},
   journal = {Advances in Neural Information Processing Systems},
   pages = {2951-2959},
   title = {Practical Bayesian Optimization of Machine Learning Algorithms},
   year = {2012},
}
@thesis{Wang2016,
   author = {Ziyu Wang},
   institution = {University of Oxford},
   title = {Practical and Theoretical Advances in Bayesian Optimization},
   year = {2016},
}
@article{Dewancker2016,
   author = {Ian Dewancker and Michael McCourt and Scott Clark},
   journal = {arXiv: 1612.04858},
   title = {Bayesian Optimization for Machine Learning A Practical Guidebook},
   year = {2016},
}
@article{Brochu2010,
   author = {Eric Brochu and Vlad M. Cora and Nando de Freitas},
   journal = {arXiv:1012.2599},
   title = {A Tutorial on Bayesian Optimization of Expensive Cost Functions, with Application to Active User Modeling and Hierarchical Reinforcement Learning},
   year = {2010},
}
@book_section{,
   title = {Bayesian Optimization},
}
@article{BergstraJames2012,
   author = {James Bergstra and Yoshua Bengio},
   journal = {Journal of Machine Learning Research},
   pages = {281-305},
   title = {Random Search for Hyper-Parameter Optimization},
   volume = {13},
   year = {2012},
}
@inproceedings{Komer2014,
   author = {Brent Komer and James Bergstra and Chris Eliasmith},
   booktitle = {International Conference on Machine Learning AutoML Workshop},
   pages = {2825-2830},
   title = {Hyperopt-Sklearn: Automatic Hyperparameter Configuration for Scikit-Learn},
   year = {2014},
}
@inproceedings{Golovin2017,
   author = {Daniel Golovin and Benjamin Solnik and Subhodeep Moitra and Greg Kochanski and John Karro and D. Sculley},
   journal = {International Conference on Knowledge Discovery and Data Mining},
   keywords = {Automated Stopping,Bayesian Optimization,Black-Box Optimization,Gaussian Processes,Hyperparameters,Transfer Learning},
   pages = {1487-1495},
   publisher = {Association for Computing Machinery},
   title = {Google Vizier: A Service for Black-Box Optimization},
   year = {2017},
}
@inproceedings{Hutter2014,
   author = {Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown},
   journal = {International Conference on Machine Learning},
   pages = {754-762},
   title = {An Efficient Approach for Assessing Hyperparameter Importance},
   year = {2014},
}
@inproceedings{Springenberg2016,
   author = {Jost Tobias Springenberg and Aaron Klein and Stefan Falkner and Frank Hutter},
   journal = {Advances in Neural Information Processing Systems},
   pages = {4134-4142},
   title = {Bayesian Optimization with Robust Bayesian Neural Networks},
   year = {2016},
}
@inproceedings{Klein2017,
   author = {Aaron Klein and Stefan Falkner and Numair Mansur and Frank Hutter},
   journal = {NIPS Bayesian Optimization Workshop},
   title = {RoBO: A Flexible and Robust Bayesian Optimization Framework in Python},
   year = {2017},
}
@inproceedings{Cao2018,
   author = {Zhen Cao and Vasily Tarasov and Sachin Tiwari and Erez Zadok},
   journal = {USENIX Annual Technical Conference},
   pages = {893-907},
   title = {Towards Better Understanding of Black-box Auto-Tuning: A Comparative Analysis for Storage Systems},
   year = {2018},
}
@article{Eggensperger2017,
   author = {Katharina Eggensperger and Marius Thomas Lindauer and Holger H. Hoos and Frank Hutter and Kevin Leyton-Brown},
   journal = {Machine Learning},
   pages = {15-41},
   title = {Efficient Benchmarking of Algorithm Configuration Procedures via Model-Based Surrogates},
   volume = {107},
   year = {2018},
}
@inproceedings{Dewancker2016a,
   author = {Ian Dewancker and Michael McCourt and Scott Clark and Patrick Hayes and Alexandra Johnson and George Ke},
   issue = {64},
   journal = {International Conference on Machine Learning AutoML Workshop},
   pages = {11-20},
   title = {A Strategy for Ranking Optimization Methods using Multiple Criteria},
   year = {2016},
}
@inproceedings{Eggensperger2013,
   author = {Katharina Eggensperger and Matthias Feurer and Frank Hutter and James Bergstra and Jasper Snoek and Holger Hoos and Kevin Leyton-Brown},
   journal = {NIPS Workshop on Bayesian Optimization in Theory and Practice},
   note = {https://automl.github.io/HPOlib2/stable/<br/><br/>https://www.ml4aad.org/automl/hpolib/},
   title = {Towards an Empirical Foundation for Assessing Bayesian Optimization of Hyperparameters},
   year = {2013},
}
@inproceedings{Bergstra2014,
   author = {James Bergstra and Brent Komer and Chris Eliasmith and David Warde-Farley},
   journal = {International Conference on Machine LearningAutoML Workshop},
   keywords = {algorithm,evaluation},
   note = {http://compneuro.uwaterloo.ca/publications/bergstra2014.html#bergstra2014cite},
   title = {Preliminary Evaluation of Hyperopt Algorithms on HPOLib},
   year = {2014},
}
@article{Huber2018,
   abstract = {Many technical systems like manufacturing plants or software applications generate large event sequences. Knowing the temporal relationship between events is important for gaining insights into the status and behavior of the system. This paper proposes a novel approach for identifying the time lag between different event types. This identification task is formulated as a binary integer optimization problem that can be solved efficiently and close to optimality by means of a linear programming approximation. The performance of the proposed approach is demonstrated on synthetic and real-world event sequences.},
   author = {Marco F. Huber and Marc-André Zöller and Marcus Baum},
   doi = {https://doi.org/10.1016/j.automatica.2018.08.025},
   journal = {Automatica},
   keywords = {Assignment problem,Event sequences,Linear programming,Optimization,Root cause analysis,Time lag},
   pages = {14-19},
   publisher = {Elsevier Ltd},
   title = {Linear programming based time lag identification in event sequences},
   volume = {98},
   year = {2018},
}
@article{Yogatama2014,
   author = {Dani Yogatama and Gideon Mann},
   journal = {International Conference on Artificial Intelligence and Statistics},
   pages = {1077-1085},
   title = {Efficient Transfer Learning Method for Automatic Hyperparameter Tuning},
   volume = {33},
   year = {2014},
}
@inproceedings{Eggensperger2015,
   author = {Katharina Eggensperger and Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown},
   journal = {AAAI Conference on Artificial Intelligence},
   keywords = {Heuristic Search and Optimization Track},
   pages = {1114-1120},
   title = {Efficient Benchmarking of Hyperparameter Optimizers via Surrogates},
   year = {2015},
}
@article{Claesen2014,
   author = {Marc Claesen and Jaak Simm and Dusan Popovic and Yves Moreau and Bart De Moor},
   journal = {arXiv: 1412.1114},
   note = {http://homes.esat.kuleuven.be/~claesenm/optunity/},
   title = {Easy Hyperparameter Search Using Optunity},
   year = {2014},
}
@inproceedings{Zoller2017,
   author = {Marc-André Zöller and Marcus Baum and Marco F. Huber},
   doi = {https://doi.org/10.1109/INDIN.2017.8104876},
   issue = {July},
   journal = {IEEE International Conference on Industrial Informatics},
   title = {Framework for Mining Event Correlations and Time Lags in Large Event Sequences},
   year = {2017},
}
@inproceedings{Falkner2018,
   author = {Stefan Falkner and Aaron Klein and Frank Hutter},
   booktitle = {ICML},
   pages = {1437-1446},
   title = {BOHB: Robust and Efficient Hyperparameter Optimization at Scale},
   year = {2018},
}
@article{Li2018,
   author = {Lisha Li and Kevin G. Jamieson and Giulia DeSalvo and Afshin Rostamizadeh and Ameet Talwalkar},
   journal = {JMLR},
   keywords = {deep learning,hyperparameter optimization,infinite-armed bandits,model selection,online,optimization},
   title = {Hyperband: A Novel Bandit-Based Approach to Hyperparameter Optimization},
   volume = {18},
   year = {2018},
}
@thesis{Gustafson2018,
   author = {Laura Gustafson},
   institution = {Massachusetts Institute of Technology},
   pages = {1-100},
   title = {Bayesian Tuning and Bandits : An Extensible, Open Source Library for AutoML},
   year = {2018},
}
@inproceedings{Bergstra2011,
   author = {James Bergstra and Rémi Bardenet and Yoshua Bengio and Balázs Kégl},
   journal = {Advances in Neural Information Processing Systems},
   pages = {2546-2554},
   publisher = {Curran Associates, Inc.},
   title = {Algorithms for Hyper-Parameter Optimization},
   year = {2011},
}
@inproceedings{Bergstra2013,
   author = {James Bergstra and Dan Yamins and David D. Cox},
   journal = {Python in Science Conference},
   note = {http://hyperopt.github.io/hyperopt/},
   pages = {13-20},
   title = {Hyperopt: A python library for optimizing the hyperparameters of machine learning algorithms},
   year = {2013},
}
@inproceedings{Khurana2016,
   author = {Udayan Khurana and Deepak Turaga and Horst Samulowitz and Srinivasan Parthasrathy},
   journal = {IEEE International Conference on Data Mining},
   pages = {1304-1307},
   title = {Cognito: Automated Feature Engineering for Supervised Learning},
   year = {2016},
}
@web_page{RapidMiner2018,
   author = {RapidMiner},
   title = {Introducing RapidMiner Auto Model},
   url = {https://rapidminer.com/resource/automated-machine-learning/},
   year = {2018},
}
@article{Molga2005,
   author = {Marcin Molga and Czesław Smutnicki},
   journal = {Test functions for optimization needs},
   title = {Test functions for optimization needs},
   year = {2005},
}
@inproceedings{Brandt2010,
   author = {Felix Brandt and Felix Fischer and Paul Harrenstein},
   journal = {International Symposium on Algorithmic Game Theory},
   pages = {102-113},
   title = {On the Rate of Convergence of Fictitious Play},
   year = {2010},
}
@book{Das2018,
   author = {Sibanjan Das and Umit Mert Cakmak},
   isbn = {9781788629898},
   publisher = {Packt Publishing},
   title = {Hands-On Automated Machine Learning},
   year = {2018},
}
@inproceedings{Dores2018,
   author = {Silvia Cristina Nunes das Dôres and Carlos Soares and Duncan Ruiz},
   journal = {Brazilian Conference on Intelligent Systems},
   title = {Bandit-Based Automated Machine Learning},
   year = {2018},
}
@book{Poli2008,
   author = {Riccardo Poli and William B. Langdon and Nicholas Freitag McPhee and John R. Koza},
   publisher = {Lulu.com},
   title = {A Field Guide to Genetic Programing},
   year = {2008},
}
@web_page{Press2016,
   author = {Gil Press},
   title = {Data Scientists Spend Most of Their Time Cleaning Data},
   url = {https://whatsthebigdata.com/2016/05/01/data-scientists-spend-most-of-their-time-cleaning-data/},
   year = {2016},
}
@article{Auer2002a,
   author = {Peter Auer},
   journal = {Journal of Machine Learning Research},
   pages = {397-422},
   title = {Using Confidence Bounds for Exploitation-Exploration Trade-offs},
   volume = {3},
   year = {2002},
}
@book{Rubinstein2008,
   author = {Reuven Y. Rubinstein and Dirk P. Kroese},
   publisher = {Wiley},
   title = {Simulation and the Monte Carlo Method},
   year = {2008},
}
@inproceedings{Geiger2012,
   author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
   journal = {Conference on Computer Vision and Pattern Recognition},
   title = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
   year = {2012},
}
@inproceedings{Wistuba2015a,
   author = {Martin Wistuba and Nicolas Schilling and Lars Schmidt-Thieme},
   journal = {IEEE International Conference on Data Science and Advanced Analytics},
   title = {Learning Hyperparameter Optimization Initializations},
   year = {2015},
}
@inproceedings{Weisz2018a,
   author = {Gellert Weisz and Andras Gyorgy and Csaba Szepesvari},
   journal = {International Conference on Machine Learning AutoML Workshop},
   pages = {5257-5265},
   title = {LeapsAndBounds: A Method for Approximately Optimal Algorithm Configuration},
   year = {2018},
}
@inproceedings{Lacoste2014,
   author = {Alexandre Lacoste and Hugo Larochelle and Mario Marchand and François Laviolette},
   journal = {Uncertainty In Artificial Intelligence},
   pages = {440-448},
   title = {Sequential Model-Based Ensemble Optimization},
   year = {2014},
}
@article{Weisz2018,
   author = {Gellért Weisz and András György and Csaba Szepesvári},
   title = {CapsAndRuns: An Improved Method for Approximately Optimal Algorithm Configuratio},
   year = {2018},
}
@inproceedings{Hoffman2014,
   author = {Matthew W Hoffman and Bobak Shahriari and Nando de Freitas},
   journal = {Artificial Intelligence and Statistics},
   pages = {365-374},
   title = {On correlation and budget constraints in model-based bandit optimization with application to automatic machine learning},
   year = {2014},
}
@inproceedings{Sparks2015,
   author = {Evan R. Sparks and Ameet Talwalkar and Daniel Haas and Michael J. Franklin and Michael I. Jordan and Tim Kraska},
   journal = {ACM Symposium on Cloud Computing},
   pages = {368-380},
   title = {Automating model search for large scale machine learning},
   year = {2015},
}
@inproceedings{Feurer2018a,
   author = {Matthias Feurer and Frank Hutter},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Towards Further Automation in AutoML},
   year = {2018},
}
@article{Luo2016,
   author = {Gang Luo},
   issue = {1},
   journal = {Network Modeling Analysis in Health Informatics and Bioinformatics},
   pages = {1-15},
   title = {A Review of Automatic Selection Methods for Machine Learning Algorithms and Hyper- parameter Values},
   volume = {5},
   year = {2016},
}
@inproceedings{Tuggener2019,
   author = {Lukas Tuggener and Mohammadreza Amirian and Katharina Rombach and Stefan Lörwald and Anastasia Varlet and Christian Westermann and Thilo Stadelmann},
   journal = {Swiss Conference on Data Science},
   pages = {31-36},
   title = {Automated Machine Learning in Practice: State of the Art and Recent Results},
   year = {2019},
}
@book{Hutter2018,
   author = {Frank Hutter and Lars Kotthoff and Joaquin Vanschoren},
   pages = {219},
   publisher = {Springer},
   title = {Automated Machine Learning: Methods, Systems, Challenges},
   year = {2018},
}
@article{He2019,
   author = {Xin He and Kaiyong Zhao and Xiaowen Chu},
   journal = {Knowledge-Based Systems},
   title = {AutoML: A Survey of the State-of-the-Art},
   volume = {212},
   year = {2021},
}
@article{Elshawi2019,
   author = {Radwa Elshawi and Mohamed Maher and Sherif Sakr},
   journal = {arXiv:1906.02287},
   title = {Automated Machine Learning: State-of-The-Art and Open Challenges},
   year = {2019},
}
@inproceedings{Rakotoarison2019,
   author = {Herilalaina Rakotoarison and Marc Schoenauer and Michèle Sebag},
   journal = {International Joint Conference on Artificial Intelligence},
   pages = {3296-3303},
   title = {Automated Machine Learning with Monte-Carlo Tree Search},
   year = {2019},
}
@inproceedings{Kocsis2006,
   author = {Levente Kocsis and Csaba Szepesvári},
   journal = {European Conference on Machine Learning},
   pages = {282-293},
   title = {Bandit based Monte-Carlo Planning},
   year = {2006},
}
@book{Koza1992,
   author = {John R. Koza},
   isbn = {0-262-11170-5},
   publisher = {MIT Press},
   title = {Genetic Programming: On the Programming of Computers by Means of Natural Selection},
   year = {1992},
}
@inproceedings{Gijsbers2019,
   author = {Pieter Gijsbers and Erin LeDell and Janek Thomas and Sébastien Poirier and Bernd Bischl and Joaquin Vanschoren},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {An Open Source AutoML Benchmark},
   year = {2019},
}
@article{Guyon2010,
   author = {Isabelle Guyon and Amir Saffari and Gideon Dror and Gavin Cawley},
   journal = {Journal of Machine Learning Research},
   pages = {61-87},
   title = {Model selection: Beyond the bayesian/frequentist divide},
   volume = {11},
   year = {2010},
}
@report{Munos2014,
   author = {Rémi Munos},
   institution = {hal-00747575},
   title = {From Bandits to Monte-Carlo Tree Search: The Optimistic Principle Applied to Optimization and Planning},
   year = {2014},
}
@article{Krishnan2019,
   author = {Sanjay Krishnan and Eugene Wu},
   journal = {arXiv:1904.11827},
   title = {AlphaClean: Automatic Generation of Data Cleaning Pipelines},
   year = {2019},
}
@inproceedings{Krishnan2016,
   author = {Sanjay Krishnan and Jiannan Wang and Eugene Wu and Michael J. Franklin and Ken Goldberg},
   journal = {Proceedings of the VLDB Endowment},
   pages = {948-959},
   title = {ActiveClean: Interactive Data Cleaning For Statistical Modeling},
   volume = {12},
   year = {2016},
}
@inproceedings{Khayyaty2015,
   author = {Zuhair Khayyaty and Ihab F. Ilyasz and Alekh Jindal and Samuel Madden and Mourad Ouzzani and Paolo Papotti and Jorge Arnulfo Quiané-Ruiz and Nan Tang and Si Yin},
   journal = {ACM International Conference on Management of Data},
   pages = {1215-1230},
   title = {BigDansing: A System for Big Data Cleansing},
   year = {2015},
}
@inproceedings{Rekatsinas2017,
   author = {Theodoros Rekatsinas and Xu Chuy and Ihab F. Ilyasy and Christopher Ré},
   journal = {VLDB Endowment},
   pages = {1190-1201},
   title = {HoloClean: Holistic Data Repairs with Probabilistic Inference},
   year = {2017},
}
@article{Krishnan2015,
   author = {Sanjay Krishnan and Jiannan Wang and Michael J. Franklin and Ken Goldberg and Tim Kraska and Tova Milo and Eugene Wu},
   issue = {3},
   journal = {IEEE Data Engineering Bulletin},
   pages = {59-75},
   title = {SampleClean: Fast and Reliable Analytics on Dirty Data},
   volume = {38},
   year = {2015},
}
@inproceedings{Gaudel2010,
   author = {Romaric Gaudel and Michèle Sebag},
   journal = {International Conference on Machine Learning},
   pages = {359-366},
   title = {Feature Selection as a One-Player Game},
   year = {2010},
}
@article{Meinshausen2010,
   author = {Nicolai Meinshausen and Peter Bühlmann},
   issue = {4},
   journal = {Journal of the Royal Statistical Society},
   pages = {417-473},
   title = {Stability selection},
   volume = {72},
   year = {2010},
}
@article{Motoda2002,
   author = {Hiroshi Motoda and Huan Liu},
   journal = {Communication of Institute of Information and Computing Machinery},
   pages = {67-72},
   title = {Feature Selection, Extraction and Construction},
   volume = {5},
   year = {2002},
}
@article{Smith2005,
   author = {Matthew G. Smith and Larry Bull},
   issue = {3},
   journal = {Genetic Programming and Evolvable Machines},
   pages = {265-281},
   title = {Genetic Programming with a Genetic Algorithm for Feature Construction and Selection},
   volume = {6},
   year = {2005},
}
@article{Tran2016,
   author = {Binh Tran and Bing Xue and Mengjie Zhang},
   journal = {Memetic Computing},
   pages = {3-15},
   publisher = {Springer Berlin Heidelberg},
   title = {Genetic programming for feature construction and selection in classification on high-dimensional data},
   volume = {8},
   year = {2016},
}
@inproceedings{Vafaie1992,
   author = {Haleh Vafaie and Kenneth De Jong},
   journal = {International Conference on Tools with Artificial Intelligence},
   pages = {200-203},
   title = {Genetic Algorithms as a Tool for Feature Selection in Machine Learning},
   year = {1992},
}
@inproceedings{Eduardo2016,
   author = {Simão Eduardo and Charles Sutton},
   journal = {Neural Information Processing Systems},
   title = {Data Cleaning using Probabilistic Models of Integrity Constraints},
   year = {2016},
}
@inproceedings{Galhardas2000,
   author = {Helena Galhardas and Daniela Florescu and Dennis Shasha and Eric Simon},
   journal = {International Conference on Management of Data},
   pages = {590-596},
   title = {AJAX:An Extensible Data Cleaning Tool},
   year = {2000},
}
@article{Markovitch2002,
   author = {Shaul Markovitch and Dan Rosenstein},
   issue = {1},
   journal = {Machine Learning},
   pages = {59-98},
   title = {Feature generation using general constructor functions},
   volume = {49},
   year = {2002},
}
@inproceedings{Margaritis2009,
   author = {Dimitris Margaritis},
   journal = {Neural Information Processing Systems},
   pages = {1240-1248},
   title = {Toward Provably Correct Feature Selection in Arbitrary Domains},
   year = {2009},
}
@inproceedings{Fan2010,
   author = {Wei Fan and Erheng Zhong and Jing Peng and Olivier Verscheure and Kun Zhang and Jiangtao Ren and Rong Yan and Qiang Yang},
   journal = {International Conference on Data Mining},
   pages = {629-640},
   title = {Generalized and Heuristic-Free Feature Construction for Improved Accuracy},
   year = {2010},
}
@article{Dor2012,
   author = {Ofer Dor and Yoram Reich},
   journal = {Information Sciences},
   pages = {176-190},
   publisher = {Elsevier Inc.},
   title = {Strengthening learning algorithms by feature discovery},
   volume = {189},
   year = {2012},
}
@article{Fernandez-Godino2016,
   author = {M. Giselle Fernández-Godino and Chanyoung Park and Nam-Ho Kim and Raphael T. Haftka},
   journal = {arXiv:1609.07196},
   title = {Review of multi-fidelity models},
   year = {2016},
}
@article{Sohn1999,
   author = {So Young Sohn},
   issue = {11},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   pages = {1137-1144},
   title = {Meta analysis of classification algorithms for pattern recognition},
   volume = {21},
   year = {1999},
}
@article{Balaji2018,
   author = {Adithya Balaji and Alexander Allen},
   journal = {arXiv:1808.06492},
   title = {Benchmarking Automatic Machine Learning Frameworks},
   year = {2018},
}
@article{Maron1993,
   author = {Oded Maron and Aw Moore},
   journal = {Advances in Neural Information Processing Systems},
   pages = {59-66},
   title = {Hoeffding Races: Accelerating Model Selection Search for Classification and Function Approximation},
   year = {1993},
}
@article{Gomes2012,
   author = {Taciana A.F. Gomes and Ricardo B.C. Prudĉncio and Carlos Soares and André L.D. Rossi and André Carvalho},
   issue = {1},
   journal = {Neurocomputing},
   pages = {3-13},
   title = {Combining Meta-Learning and Search Techniques to Select Parameters for Support Vector Machines},
   volume = {75},
   year = {2012},
}
@article{Klein2017a,
   author = {Aaron Klein and Stefan Falkner and Jost Tobias Springenberg and Frank Hutter},
   journal = {International Conference on Learning Representations},
   pages = {1-16},
   title = {Learning Curve Prediction With Bayesian Neural Networks},
   year = {2017},
}
@inproceedings{Gama2000,
   author = {Joao Gama and Pavel Brazdil},
   journal = {Portuguese Conference on Artificial Intelligence},
   title = {Characterization of Classification Algorithms},
   year = {2000},
}
@article{Domhan2015,
   author = {Tobias Domhan and Jost Tobias Springenberg and Frank Hutter},
   journal = {International Joint Conference on Artificial Intelligence},
   pages = {3460-3468},
   title = {Speeding up Automatic Hyperparameter Optimization of Deep Neural Networks by Extrapolation of Learning Curves},
   year = {2015},
}
@article{Kononenko1994,
   author = {Igor Kononenko},
   journal = {European Conference on Machine Learning},
   title = {Estimating attributes: Analysis and extensions of RELIEF},
   year = {1994},
}
@article{Sondhi2009,
   author = {Parikshit Sondhi},
   journal = {Sifaka. Cs. Uiuc. Edu},
   pages = {70-71},
   title = {Feature Construction Methods: A Survey},
   volume = {69},
   year = {2009},
}
@article{Gower1985,
   author = {John Clifford Gower},
   journal = {Linear Algebra and its Applications},
   pages = {81-97},
   title = {Properties of Euclidean and Non-Euclidean Distance Matrices},
   volume = {67},
   year = {1985},
}
@article{Bischl2019,
   author = {Bernd Bischl and Giuseppe Casalicchio and Matthias Feurer and Frank Hutter and Michel Lang and Rafael G. Mantovani and Jan N. van Rijn and Joaquin Vanschoren},
   journal = {arXiv:1708.03731v2},
   title = {OpenML Benchmarking Suites},
   year = {2019},
}
@article{Rousseeuw1987,
   author = {Peter J. Rousseeuw},
   journal = {Journal of Computational and Applied Mathematics},
   keywords = {Graphical display,classification,cluster analysis,clustering validity},
   pages = {53-65},
   title = {Silhouettes: A graphical aid to the interpretation and validation of cluster analysis},
   volume = {20},
   year = {1987},
}
@web_page{H2O.ai2019,
   author = {H2O.ai},
   title = {H2O AutoML},
   url = {http://docs.h2o.ai/h2o/latest-stable/h2o-docs/automl.html},
   year = {2019},
}
@article{Gower1971,
   author = {John Clifford Gower},
   issue = {4},
   journal = {Biometrics},
   pages = {857-871},
   title = {A General Coefficient of Similarity and Some of Its Properties},
   volume = {27},
   year = {1971},
}
@article{Fukunaga1975,
   author = {Keinosuke Fukunaga and Larry D. Hostetler},
   issue = {1},
   journal = {IEEE Transactions on Information Theory},
   pages = {32-40},
   title = {The estimation of the gradient of a density function, with applications in pattern recognition},
   volume = {21},
   year = {1975},
}
@article{Levenshtein1966,
   author = {Vladimir I. Levenshtein},
   issue = {8},
   journal = {Soviet physics doklady},
   pages = {707-710},
   title = {Binary codes capable of correcting deletions, insertions, and reversals},
   volume = {10},
   year = {1966},
}
@article{Ratcliff1988,
   author = {John W. Ratcliff and David E. Metzener},
   issue = {7},
   journal = {Dr Dobbs Journal},
   pages = {46-72},
   title = {Pattern Matching: The Gestalt Approach},
   volume = {13},
   year = {1988},
}
@article{Belotti2013,
   author = {Pietro Belotti and Christian Kirches and Sven Leyffer and Jeff Linderoth and James Luedtke and Ashutosh Mahajan},
   journal = {Acta Numerica},
   pages = {1-131},
   title = {Mixed-integer nonlinear optimization},
   volume = {22},
   year = {2013},
}
@web_page{MicrosoftCorporation2017,
   author = {Microsoft Corporation},
   title = {Team Data Science Process},
   url = {https://docs.microsoft.com/en-us/azure/machine-learning/team-data-science-process/overview},
   year = {2017},
}
@article{Shearer2000,
   author = {Colin Shearer},
   issue = {4},
   journal = {Journal of Data Warehousing},
   pages = {13-22},
   title = {The CRISP-DM model: the new blueprint for data mining},
   volume = {5},
   year = {2000},
}
@web_page{Press2016a,
   author = {Gil Press},
   title = {Cleaning Big Data: Most Time-Consuming, Least Enjoyable Data Science Task, Survey Says},
   url = {https://www.forbes.com/sites/gilpress/2016/03/23/data-preparation-most-time-consuming-least-enjoyable-data-science-task-survey-says/#7dd352e16f63},
   year = {2016},
}
@article{Sun2019,
   abstract = {Machine learning pipeline potentially consists of several stages of operations like data preprocessing, feature engineering and machine learning model training. Each operation has a set of hyper-parameters, which can become irrelevant for the pipeline when the operation is not selected. This gives rise to a hierarchical conditional hyper-parameter space. To optimize this mixed continuous and discrete conditional hierarchical hyper-parameter space, we propose an efficient pipeline search and configuration algorithm which combines the power of Reinforcement Learning and Bayesian Optimization. Empirical results show that our method performs favorably compared to state of the art methods like Auto-sklearn , TPOT, Tree Parzen Window, and Random Search.},
   author = {Xudong Sun and Jiali Lin and Bernd Bischl},
   issue = {August},
   title = {ReinBo: Machine Learning pipeline search and configuration with Bayesian Optimization embedded Reinforcement Learning},
   url = {http://arxiv.org/abs/1904.05381},
   year = {2019},
}
@article{Bilalli2018,
   author = {Besim Bilalli and Alberto Abelló and Tomàs Aluja-Banet and Robert Wrembel},
   journal = {Computer Standards and Interfaces},
   pages = {101-109},
   title = {Intelligent Assistance for Data Pre-processing Besim},
   volume = {57},
   year = {2018},
}
@inproceedings{Fusi2018a,
   author = {Nicolo Fusi and Rishit Sheth and Melih Elibol},
   journal = {Advances in Neural Information Processing Systems},
   pages = {3348-3357},
   title = {Probabilistic Matrix Factorization for Automated Machine Learning},
   year = {2018},
}
@inproceedings{Kietz2012a,
   author = {Jörg Uwe Kietz and Floarea Serban and Abraham Bernstein and Simon Fischer},
   journal = {Planning to Learn Workshop at ECAI},
   title = {Designing KDD-Workflows via HTN-Planning for Intelligent Discovery Assistance},
   year = {2012},
}
@article{Strang2018a,
   author = {Benjamin Strang and Peter van der Putten and Jan N. van Rijn and Frank Hutter},
   doi = {10.1007/978-3-030-01768-2_25},
   isbn = {9783030017675},
   issn = {16113349},
   journal = {Advances in Intelligent Data Analysis},
   keywords = {Benchmarking,Linear classifiers,Meta-Learning},
   title = {Don’t Rule Out Simple Models Prematurely: a Large Scale Benchmark Comparing Linear and Non-linear Classifiers in OpenML},
   year = {2018},
}
@article{Yu2003a,
   abstract = {Feature selection, as a preprocessing step to machine learning, is effective in reducing dimensionality, removing irrelevant data, increasing learning accuracy, and improving result comprehensibility. However, the recent increase of dimensionality of data poses a severe challenge to many existing feature selection methods with respect to efficiency and effectiveness. In this work, we introduce a novel concept, predominant correlation, and propose a fast filter method which can identify relevant features as well as redundancy among relevant features without pairwise correlation analysis. The efficiency and effectiveness of our method is demonstrated through extensive comparisons with other methods using real-world data of high dimensionality.},
   author = {Lei Yu and Huan Liu},
   journal = {International Conference on Machine Learning},
   pages = {856-863},
   title = {Feature Selection for High-Dimensional Data: A Fast Correlation-Based Filter Solution Lei},
   volume = {2},
   year = {2003},
}
@article{Sun2013a,
   author = {Quan Sun and Bernhard Pfahringer},
   issue = {1},
   journal = {Machine Learning},
   keywords = {Algorithm ranking,Ensemble learning,Meta-learning,Ranking trees},
   pages = {141-161},
   title = {Pairwise meta-rules for better meta-learning-based algorithm ranking},
   volume = {93},
   year = {2013},
}
@article{Kalousis2014,
   author = {Phong Nguyen and Melanie Hilario and Alexandros Kalousis},
   journal = {Journal of Artificial Intelligence Research},
   pages = {605-644},
   title = {Using Meta-mining to Support Data Mining Workflow Planning and Optimization},
   volume = {51},
   year = {2014},
}
@article{Coulom2006,
   author = {Rémi Coulom},
   journal = {5th International Conference on Computer and Games},
   title = {Efficient Selectivity and Backup Operators in Monte-Carlo Tree Search},
   year = {2006},
}
@article{Zoller2021,
   author = {Marc-André Zöller and Marco F. Huber},
   doi = {https://doi.org/10.1613/jair.1.11854},
   journal = {Journal of Artificial Intelligence Research},
   pages = {409-472},
   title = {Benchmark and Survey of Automated Machine Learning Frameworks},
   volume = {70},
   year = {2021},
}
@inproceedings{Auger2013,
   author = {David Auger and Adrien Couetoux and Olivier Teytaud},
   journal = {Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
   pages = {194-209},
   title = {Continuous Upper Confidence Trees with Polynomial Exploration – Consistency},
   year = {2013},
}
@article{Kandasamy2015,
   author = {Kirthevasan Kandasamy and Jeff Schneider and Barnabás Póczos},
   journal = {International Conference on Machine Learning},
   pages = {295-304},
   title = {High Dimensional Bayesian Optimisation and Bandits via Additive Models},
   year = {2015},
}
@inproceedings{Drori2019,
   author = {Iddo Drori and Yamuna Krishnamurthy and Raoni de Paula Lourenco and Remi Rampin and Cho Kyunghyun and Claudio Silva and Juliana Freire},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Automatic Machine Learning by Pipeline Synthesis using Model-Based Reinforcement Learning and a Grammar},
   year = {2019},
}
@inproceedings{Nguyen2020,
   author = {Tien-Dung Nguyen and Tomasz Maszczyk and Katarzyna Musial and Marc-André Zöller and Bogdan Gabrys},
   doi = {https://doi.org/10.1007/978-3-030-44584-3_28},
   journal = {International Symposium on Intelligent Data Analysis},
   pages = {352-365},
   title = {AVATAR - Machine Learning Pipeline Evaluation Using Surrogate Model},
   year = {2020},
}
@book_section{Goodfellow2016,
   author = {Ian Goodfellow and Yoshua Bengio and Aaron Courville},
   journal = {Deep Learning},
   publisher = {MIT Press},
   title = {Representation Learning},
   year = {2016},
}
@report{GoogleLLC2019,
   author = {Google LLC},
   institution = {Google LLC},
   title = {AI Explanations Whitepaper},
   year = {2019},
}
@inproceedings{Zhang2016,
   author = {Yuyu Zhang and Mohammad Taha Bahadori and Hang Su and Jimeng Sun},
   journal = {ACM International Conference on Knowledge Discovery and Data Mining},
   keywords = {Automated hyperparameter tuning,Bayesian optimization,Data analytic pipeline,Health analytics},
   pages = {2065–2074},
   title = {FLASH: Fast Bayesian Optimization for Data Analytic Pipelines},
   year = {2016},
}
@article{Alaa2018,
   author = {Ahmed M. Alaa and Mihaela Van Der Schaar},
   journal = {International Conference on Machine Learning},
   pages = {139-148},
   title = {AutoPrognosis: Automated Clinical Prognostic Modeling via Bayesian Optimization with Structured Kernel Learning},
   volume = {1},
   year = {2018},
}
@inproceedings{Salvador2017a,
   author = {Manuel Martin Salvador and Marcin Budka and Bogdan Gabrys},
   journal = {Industrial Simulation Conference},
   pages = {17-23},
   title = {Modelling multi-component predictive systems as petri nets},
   year = {2017},
}
@inproceedings{Das2020,
   author = {Piali Das and Valerio Perrone and Nikita Ivkin and Tanya Bansal and Zohar Karnin and Huibin Shen and Iaroslav Shcherbatyi and Yotam Elor and Wilton Wu and Aida Zolic and Thibaut Lienart and Alex Tang and Amr Ahmed and Jean Baptiste Faddoul and Rodolphe Jenatton and Fela Winkelmolen and Philip Gautier and Leo Dirac and Andre Perunicic and Miroslav Miladinovic and Giovanni Zappella and Cedric Archambeau and Matthias Seeger and Bhaskar Dutt and Laurence Rouesnel},
   journal = {Data Management for End-to-End Machine Learning},
   pages = {1–7},
   publisher = {Association for Computing Machinery},
   title = {Amazon SageMaker Autopilot: A White Box AutoML Solution at Scale},
   year = {2020},
}
@thesis{Petri1962,
   author = {Carl Adam Petri},
   institution = {Universität Hamburg},
   title = {Kommunikation mit Automaten},
   year = {1962},
}
@inproceedings{Levesque2017,
   author = {Julien Charles Levesque and Audrey Durand and Christian Gagne and Robert Sabourin},
   journal = {International Joint Conference on Neural Networks},
   pages = {286–293},
   title = {Bayesian Optimization for Conditional Hyperparameter Spaces},
   year = {2017},
}
@inproceedings{Momma2002,
   author = {Michinari Momma and Kristin P. Bennett},
   journal = {SIAM International Conference on Data Mining},
   pages = {261–274},
   title = {A Pattern Search Method for Model Selection of Support Vector Regression},
   year = {2002},
}
@inproceedings{Kohavi1995,
   author = {Ron Kohavi and George H. John},
   journal = {International Conference on Machine Learning},
   pages = {304-312},
   title = {Automatic Parameter Selection by Minimizing Estimated Error},
   year = {1995},
}
@article{Chapelle2002,
   author = {Olivier Chapelle and Vladimir Vapnik and Olivier Bousquet and Sayan Mukherjee},
   journal = {Machine Learning},
   pages = {131-159},
   title = {Choosing Multiple Parameters for Support Vector Machines},
   volume = {46},
   year = {2002},
}
@article{Rakotomamonjy2003,
   author = {Alain Rakotomamonjy},
   journal = {Journal of Machine Learning Research},
   pages = {1357-1370},
   title = {Variable selection using SVM-based criteria},
   volume = {3},
   year = {2003},
}
@article{Huberman1997,
   author = {Bernardo A. Huberman and Rajan M. Lukose and Tad Hogg},
   issue = {5296},
   journal = {Science},
   pages = {51-54},
   title = {An Economics Approach to Hard Computational Problems},
   volume = {275},
   year = {1997},
}
@article{Tuv2009,
   author = {Eugene Tuv and Alexander Borisov and George Runger and Kari Torkkola},
   issn = {15324435},
   journal = {Journal of Machine Learning Research},
   pages = {1341-1366},
   title = {Feature Selection with Ensembles, Artificial Variables, and Redundancy Elimination},
   volume = {10},
   year = {2009},
}
@inproceedings{Mejia-Lavalle2006,
   author = {Manuel Mejía-Lavalle and Enrique Sucar and Gustavo Arroyo},
   journal = {International Workshop on Feature Selection for Data Mining},
   pages = {131-135},
   title = {Feature Selection With A Perceptron Neural Net},
   year = {2006},
}
@article{Shahriari2016,
   author = {Bobak Shahriari and Kevin Swersky and Ziyu Wang and Ryan P. Adams and Nando de Freitas},
   issue = {1},
   journal = {Proceedings of the IEEE},
   pages = {148 - 175},
   title = {Taking the Human Out of the Loop: A Review of Bayesian Optimization},
   volume = {104},
   year = {2016},
}
@article{Guyon2002,
   author = {Isabelle Guyon and Jason Weston and Stephen Barnhill},
   isbn = {3540881913},
   issn = {03029743},
   journal = {Machine Learning},
   pages = {389-422},
   title = {Gene Selection for Cancer Classification using Support Vector Machines},
   volume = {46},
   year = {2002},
}
@inproceedings{Li2020,
   author = {Liam Li and Kevin Jamieson and Afshin Rostamizadeh and Ekaterina Gonina and Moritz Hardt and Benjamin Recht and Ameet Talwalkar},
   journal = {Machine Learning and Systems},
   title = {A System for Massively Parallel Hyperparameter Tuning},
   year = {2020},
}
@book_section{Fabris2019,
   author = {Fabio Fabris and Alex A. Freitas},
   journal = {Machine Learning, Optimization, and Data Science},
   pages = {508-520},
   publisher = {Springer International Publishing},
   title = {Analysing the Overfit of the auto-sklearn Automated Machine Learning Tool},
   volume = {11943},
   year = {2019},
}
@inproceedings{Post2016,
   author = {Martijn J. Post and Peter van der Putten and Jan N. van Rijn},
   journal = {Advances in Intelligent Data Analysis XV},
   pages = {158–170},
   title = {Does Feature Selection Improve Classification? A Large Scale Experiment in OpenML},
   year = {2016},
}
@article{Bilalli2017,
   author = {Besim Bilalli and Alberto Abelló and Tomàs Aluja-Banet},
   issue = {4},
   journal = {International Journal of Applied Mathematics and Computer Science},
   pages = {697-712},
   title = {On the Predictive Power of Meta-Features in OpenML},
   volume = {27},
   year = {2017},
}
@book_section{Ginsbourger2010,
   author = {David Ginsbourger and Rodolphe Le Riche and Laurent Carraro},
   journal = {Computational Intelligence in Expensive Optimization Problems},
   pages = {131-162},
   publisher = {Springer Berlin Heidelberg},
   title = {Kriging Is Well-Suited to Parallelize Optimization},
   year = {2010},
}
@inproceedings{Hutter2012,
   author = {Frank Hutter and Holger H. Hoos and Kevin Leyton-Brown},
   journal = {International Conference on Learning and Intelligent Optimization},
   title = {Parallel algorithm configuration},
   volume = {7219},
   year = {2012},
}
@inproceedings{Gil2018,
   author = {Yolanda Gil and Ke-Thia Yao and Varun Ratnakar and Daniel Garijo and Greg Ver Steeg and Pedro Szekely and Rob Brekelmans and Mayank Kejriwal and Fanghao Luo and I-Hui Huang},
   journal = {International Conference on Machine Learning AutoML Workshop},
   keywords = {automating machine learning,automl,pipelines,planning,workflows},
   pages = {1-8},
   title = {P4ML: A Phased Performance-Based Pipeline Planner for Automated Machine Learning},
   year = {2018},
}
@book_section{Perrone2019,
   author = {Valerio Perrone and Huibin Shen and Matthias Seeger and Cedric Archambeau and Rodolphe Jenatton},
   journal = {Advances in Neural Information Processing Systems 32},
   pages = {12771--12781},
   publisher = {Curran Associates, Inc.},
   title = {Learning search spaces for Bayesian optimization: Another view of hyperparameter transfer learning},
   year = {2019},
}
@article{Probst2019,
   author = {Philipp Probst and Anne-Laure Boulesteix and Bernd Bischl},
   issue = {53},
   journal = {Journal of Machine Learning Research},
   pages = {1-32},
   title = {Tunability: Importance of Hyperparameters of Machine Learning Algorithms},
   volume = {20},
   year = {2019},
}
@inproceedings{Garrido-Merchan2018,
   author = {Eduardo C. Garrido-Merchán and Daniel Hernández-Lobato},
   journal = {International Conference on Machine Learning AutoML Workshop},
   pages = {1-18},
   title = {Dealing with Integer-valued Variables in Bayesian Optimization with Gaussian Processes},
   year = {2018},
}
@incollection{Vanschoren2019,
   author = {Joaquin Vanschoren},
   booktitle = {Automatic Machine Learning: Methods, Systems, Challenges},
   pages = {35-61},
   publisher = {Springer},
   title = {Meta-Learning},
   year = {2019},
}
@web_page{Ginsbourger2010a,
   author = {David Ginsbourger and Janis Janusevskis and Rodolphe Le Riche},
   title = {Dealing with asynchronicity in parallel Gaussian process based global optimization},
   url = {https://hal.archives-ouvertes.fr/hal-00507632},
   year = {2010},
}
@article{Bengio2013,
   author = {Yoshua Bengio and Aaron Courville and Pascal Vincent},
   issue = {8},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   pages = {1798-1828},
   title = {Representation Learning: A Review and New Perspectives},
   volume = {35},
   year = {2013},
}
@article{Opitz1999,
   author = {David Opitz and Richard Maclin},
   journal = {Journal of Artificial Intelligence Research},
   pages = {169-198},
   title = {Popular Ensemble Methods: An Empirical Study},
   volume = {11},
   year = {1999},
}
@article{Polikar2006,
   author = {Robi Polikar},
   issue = {3},
   journal = {IEEE Circuits and Systems Magazine},
   keywords = {Classifier combination,Classifier diversity,Classifier fusion,Classifier selection,Data fusion,Incremental learning,Multiple classifier systems},
   pages = {21-45},
   publisher = {IEEE},
   title = {Ensemble Based Systems in Decision Making},
   volume = {6},
   year = {2006},
}
@article{Rokach2010,
   author = {Lior Rokach},
   issue = {1-2},
   journal = {Artificial Intelligence Review},
   keywords = {Boosting,Classification,Ensemble of classifiers,Supervised learning},
   pages = {1-39},
   title = {Ensemble-based classifiers},
   volume = {33},
   year = {2010},
}
@inproceedings{Anthony2017,
   author = {Thomas Anthony and Zheng Tian and David Barber},
   journal = {Advances in Neural Information Processing Systems},
   pages = {5360-5370},
   title = {Thinking Fast and Slow with Deep Learning and Tree Search},
   year = {2017},
}
@inproceedings{Caruana2004,
   author = {Rich Caruana and Alexandru Niculescu-Mizil and Geoff Crew and Alex Ksikes},
   booktitle = {ICML},
   pages = {18},
   title = {Ensemble Selection from Libraries of Models},
   year = {2004},
}
@article{Wang2021,
   abstract = {Data science and machine learning (DS/ML) are at the heart of the recent advancements of many Artificial Intelligence (AI) applications. There is an active research thread in AI, \autoai, that aims to develop systems for automating end-to-end the DS/ML Lifecycle. However, do DS and ML workers really want to automate their DS/ML workflow? To answer this question, we first synthesize a human-centered AutoML framework with 6 User Role/Personas, 10 Stages and 43 Sub-Tasks, 5 Levels of Automation, and 5 Types of Explanation, through reviewing research literature and marketing reports. Secondly, we use the framework to guide the design of an online survey study with 217 DS/ML workers who had varying degrees of experience, and different user roles "matching" to our 6 roles/personas. We found that different user personas participated in distinct stages of the lifecycle -- but not all stages. Their desired levels of automation and types of explanation for AutoML also varied significantly depending on the DS/ML stage and the user persona. Based on the survey results, we argue there is no rationale from user needs for complete automation of the end-to-end DS/ML lifecycle. We propose new next steps for user-controlled DS/ML automation.},
   author = {Dakuo Wang and Q. Vera Liao and Yunfeng Zhang and Udayan Khurana and Horst Samulowitz and Soya Park and Michael Muller and Lisa Amini},
   journal = {arXiv: 2101.03970},
   pages = {1-31},
   title = {How Much Automation Does a Data Scientist Want?},
   year = {2021},
}
@inproceedings{Gil2019a,
   author = {Yolanda Gil and James Honaker and Vito D Orazio and Daniel Garijo and Neda Jahanshad},
   journal = {International Conference on Intelligent User Interfaces},
   pages = {614-624},
   title = {Towards Human-Guided Machine Learning},
   year = {2019},
}
@article{Pillay2018,
   author = {Nelishia Pillay and Rong Qu and Dipti Srinivasan and Barbara Hammer and Kenneth Sorensen},
   issue = {2},
   journal = {IEEE Computational Intelligence Magazine},
   pages = {16-17},
   title = {Automated Design of Machine Learning and Search Algorithms [Guest Editorial]},
   volume = {13},
   year = {2018},
}
@article{Escalante2020,
   author = {Hugo Jair Escalante},
   journal = {arXiv:2008.0851},
   pages = {1-17},
   title = {Automated Machine Learning - a brief review at the end of the early years},
   year = {2020},
}
@thesis{Giannis2020,
   author = {Poulakis Giannis},
   institution = {University of Piraeus},
   title = {Unsupervised AutoML: A Study on Automated Machine Learning in the Context of Clustering},
   year = {2020},
}
@inproceedings{Escalante2020,
   author = {Hugo Jair Escalante and Wei Wei Tu and Isabelle Guyon and Daniel L. Silver and Evelyne Viegas and Yuqiang Chen and Wenyuan Dai and Qiang Yang},
   journal = {The NeurIPS '18 Competition},
   keywords = {Automatic machine learning,Challenge organization,Concept drift,Life long learning},
   pages = {209-229},
   title = {AutoML @ NeurIPS 2018 challenge: Design and results},
   year = {2020},
}
@inproceedings{Tornede2020,
   author = {Tanja Tornede and Alexander Torned and Marcel Wever and Felix Mohr and Eyke Hüllermeier},
   journal = {IoT Streams 2020},
   pages = {106–118},
   title = {AutoML for Predictive Maintenance: One Tool to RUL Them All},
   year = {2020},
}
@inproceedings{Madrid2019,
   author = {Jorge G. Madrid and Hugo Jair Escalante and Eduardo F. Morales and Wei Wei Tu and Yang Yu and Lisheng Sun-Hosoya and Isabelle Guyon and Michele Sebag},
   journal = {International Conference on Machine Learning AutoML Workshop},
   keywords = {AutoML,AutoSKLearn,Concept Drift,Life Long Machine Learning},
   pages = {1-14},
   title = {Towards AutoML in the presence of Drift: First results},
   year = {2018},
}
@thesis{Tschechlov2019,
   author = {Dennis Tschechlov},
   institution = {University of Stuttgart},
   pages = {92},
   title = {Analysis and Transfer of AutoMLConcepts for Clustering Algorithms},
   year = {2019},
}
@article{Shi2020,
   author = {Xiupeng Shi and Yiik Diew Wong and Chen Chai and Michael Zhi-Feng Li},
   journal = {IEEE Transactions on Intelligent Transportation Systems},
   pages = {1-10},
   title = {An Automated Machine Learning (AutoML) Method of Risk Prediction for Decision-Making of Autonomous Vehicles},
   year = {2020},
}
@book_section{Wilson2020,
   author = {Jobin Wilson and Amit Kumar Meher and Bivin Vinodkumar Bindu and Santanu Chaudhury and Brejesh Lall and Manoj Sharma and Vishakha Pareek},
   doi = {10.1007/978-3-030-29135-8_13},
   isbn = {9783030291358},
   journal = {The NeurIPS '18 Competition},
   pages = {317-335},
   title = {Automatically Optimized Gradient Boosting Trees for Classifying Large Volume High Cardinality Data Streams Under Concept Drift},
   year = {2020},
}
@inproceedings{Halvari2020,
   author = {Tuomas Halvari and Jukka K. Nurminen and Tommi Mikkonen},
   journal = {Agents and Robots for reliable Engineered Autonomy},
   pages = {103-116},
   title = {Testing the Robustness of AutoML Systems},
   year = {2020},
}
@inproceedings{Li2019,
   author = {Yu-Feng Li and Hai Wang and Tong Wei and Wei-wei Tu},
   journal = {AAAI Conference on Artificial Intelligence},
   title = {Towards Automated Semi-Supervised Learning},
   year = {2019},
}
@article{Faust2019,
   abstract = {Many continuous control tasks have easily formulated objectives, yet using them directly as a reward in reinforcement learning (RL) leads to suboptimal policies. Therefore, many classical control tasks guide RL training using complex rewards, which require tedious hand-tuning. We automate the reward search with AutoRL, an evolutionary layer over standard RL that treats reward tuning as hyperparameter optimization and trains a population of RL agents to find a reward that maximizes the task objective. AutoRL, evaluated on four Mujoco continuous control tasks over two RL algorithms, shows improvements over baselines, with the the biggest uplift for more complex tasks. The video can be found at: https://youtu.be/svdaOFfQyC8.},
   author = {Aleksandra Faust and Anthony Francis and Dar Mehta},
   issn = {23318422},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Evolving rewards to automate reinforcement learning},
   year = {2019},
}
@inproceedings{Li2019a,
   author = {Michael Y Li and Ryan P Adams},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {Explainability Constraints for Bayesian Optimization},
   year = {2019},
}
@inproceedings{Xiong2019,
   author = {Zheng Xiong},
   journal = {International Conference on Machine Learning AutoML Workshop},
   pages = {1-11},
   title = {Auto-Lifelong : An AutoML System for Lifelong Machine Learning},
   year = {2019},
}
@inproceedings{Xanthopoulos2020,
   author = {Iordanis Xanthopoulos and Ioannis Tsamardinos and Vassilis Christophides and Eric Simon and Alejandro Salinger},
   journal = {Workshop Processdings of the EDBT/ICDT},
   title = {Putting the Human Back in the AutoML Loop},
   year = {2020},
}
@inproceedings{Crisan2021,
   author = {Anamaria Crisan and Brittany Fiore-Gartland},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-15},
   publisher = {Association for Computing Machinery},
   title = {Fits and Starts: Enterprise Use of AutoML and the Role of Humans in the Loop},
   year = {2021},
}
@article{Burkart2021,
   author = {Nadia Burkart and Marco F. Huber},
   journal = {Journal of Artificial Intelligence Research},
   pages = {245-317},
   title = {A Survey on the Explainability of Supervised Machine Learning},
   volume = {70},
   year = {2021},
}
@article{Xin2021,
   author = {Doris Xin and Eva Yiwei Wu and Doris Jung-Lin Lee and Niloufar Salehi and Aditya Parameswaran},
   journal = {arXiv: 2101.04834},
   title = {Whither AutoML? Understanding the Role of Automation in Machine Learning Workflows},
   year = {2021},
}
@inproceedings{Patron2020,
   author = {Gabriel Patron and Diego Leon and Edwin Lopez and German Hernandez},
   journal = {Applied Computer Sciences in Engineering},
   pages = {16-23},
   publisher = {Springer International Publishing},
   title = {An Interpretable Automated Machine Learning Credit Risk Model},
   year = {2020},
}
@article{Tsiakmaki2020,
   author = {Maria Tsiakmaki and Georgios Kostopoulos and Sotiris Kotsiantis and Omiros Ragos},
   issue = {90},
   journal = {Applied Sciences},
   pages = {1-27},
   title = {Implementing AutoML in Educational Data Mining for Prediction Tasks},
   volume = {10},
   year = {2020},
}
@article{Lee2019,
   author = {Doris Jung-Lin Lee and Stephen Macke and Doris Xin and Angela Lee and Silu Huang and Aditya Parameswaran},
   issue = {2},
   journal = {IEEE Data Engineering Bulletin},
   pages = {59-70},
   title = {A Human-in-the-loop Perspective on AutoML: Milestones and the Road Ahead},
   volume = {42},
   year = {2019},
}
@article{Pfisterer2019,
   author = {Florian Pfisterer and Janek Thomas and Bernd Bischl},
   issue = {2019-01},
   journal = {Statistical Computing},
   pages = {18-19},
   title = {Towards Human-Centered AutoML},
   year = {2019},
}
@article{Cambronero2020,
   author = {José P. Cambronero and Jürgen Cito and Martin C. Rinard},
   journal = {ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
   pages = {763-774},
   title = {AMS: Generating AutoML Search Spaces from Weak Specifications},
   year = {2020},
}
@inproceedings{Weidele2020,
   author = {Daniel Karl I. Weidele and Justin D. Weisz and Erick Oduor and Michael Muller and Josh Andres and Alexander Gray and Dakuo Wang},
   journal = {International Conference on Intelligent User Interfaces},
   pages = {308-312},
   publisher = {Association for Computing Machinery},
   title = {AutoAIViz: Opening the Blackbox of Automated Artificial Intelligence with Conditional Parallel Coordinates},
   year = {2020},
}
@inproceedings{Elkholy2019,
   author = {Alexander Elkholy and Fangkai Yang and Steven Gustafson},
   journal = {International Conference on Autonomous Agents and MultiAgent Systems},
   pages = {1937–1939},
   title = {Interpretable Automated Machine Learning in Maana Knowledge Platform},
   year = {2019},
}
@inproceedings{Freitas2019,
   author = {Alex A. Freitas},
   journal = {Machine Learning and Knowledge Extraction},
   pages = {48-66},
   publisher = {Springer International Publishing},
   title = {Automated Machine Learning for Studying the Trade-Off Between Predictive Accuracy and Interpretability},
   year = {2019},
}
@inproceedings{Hong2020,
   author = {Sungsoo Ray Hong and Jessica Hullman and Enrico Bertini},
   doi = {10.1145/3392878},
   issn = {25730142},
   issue = {CSCW1},
   journal = {Human-Computer Interaction},
   pages = {1-26},
   title = {Human Factors in Model Interpretability: Industry Practices, Challenges, and Needs},
   volume = {4},
   year = {2020},
}
@article{Ahmad2018,
   author = {Muhammad Aurangzeb Ahmad and Carly Eckert and Ankur Teredesai},
   issue = {1},
   journal = {IEEE Intelligent Informatics Bulletin},
   pages = {1-7},
   title = {Interpretable Machine Learning in Healthcare},
   volume = {19},
   year = {2018},
}
@inproceedings{Drozdal2020,
   author = {Jaimie Drozdal and Justin Weisz and Dakuo Wang and Gaurav Dass and Bingsheng Yao and Changruo Zhao and Michael Muller and Lin Ju and Hui Su},
   journal = {International Conference on Intelligent User Interfaces},
   pages = {297–307},
   publisher = {Association for Computing Machinery},
   title = {Trust in AutoML: Exploring Information Needs for Establishing Trust in Automated Machine Learning Systems},
   year = {2020},
}
@inproceedings{Wang2019,
   author = {Qianwen Wang and Yao Ming and Zhihua Jin and Qiaomu Shen and Dongyu Liu and Micah J. Smith and Kalyan Veeramachaneni and Huamin Qu},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-12},
   publisher = {Association for Computing Machinery},
   title = {ATMSeer: Increasing Transparency and Controllability in Automated Machine Learning},
   year = {2019},
}
@inproceedings{Mitchell2019,
   author = {Margaret Mitchell and Simone Wu and Andrew Zaldivar and Parker Barnes and Lucy Vasserman and Ben Hutchinson and Elena Spitzer and Inioluwa Deborah Raji and Timnit Gebru},
   journal = {Conference on Fairness, Accountability, and Transparency},
   pages = {220–229},
   title = {Model Cards for Model Reporting},
   year = {2019},
}
@article{Arnold2019,
   author = {M. Arnold and R. K. E. Bellamy and M. Hind and S. Houde and S. Mehta and A. Mojsilović and R. Nair and K. N. Ramamurthy and A. Olteanu and D. Piorkowski and D. Reimer and J. Richards and J. Tsay and K. R. Varshney},
   journal = {IBM Journal of Research and Development},
   pages = {1-11},
   title = {FactSheets : Increasing Trust in AI Services through Supplier ’ s Declarations of Conformity},
   volume = {63},
   year = {2019},
}
@article{Park2021,
   author = {Heungseok Park and Yoonsoo Nam and Ji-hoon Kim and Jaegul Choo},
   issue = {2},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   pages = {1407-1416},
   title = {HyperTendril: Visual Analytics for User-Driven Hyperparameter Optimization of Deep Neural Networks},
   volume = {27},
   year = {2021},
}
@inproceedings{Park2019,
   author = {Heungseok Park and Jinwoong Kim and Minkyu Kim and Ji-hoon Kim and Jaegul Choo and Jung-woo Ha and Nako Sung},
   journal = {SysML Conference},
   title = {VisualHyperTuner: Visual Analytics for User-Driven Hyperparameter Tuning of Deep Neural Networks},
   year = {2019},
}
@book_section{Kovalerchuk2021,
   author = {Boris Kovalerchuk and Muhammad Aurangzeb Ahmad and Ankur Teredesai},
   journal = {Interpretable Artificial Intelligence: A Perspective of Granular Computing},
   pages = {217-267},
   title = {Survey of Explainable Machine Learning with Visual and Granular Methods beyond Quasi-explanations},
   year = {2021},
}
@article{Ono2021,
   author = {Jorge Piazentin Ono and Sonia Castelo and Roque Lopez and Enrico Bertini and Juliana Freire and Claudio Silva},
   issue = {2},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   keywords = {Automatic Machine Learning,Model Evaluation,Pipeline Visualization},
   pages = {390-400},
   title = {PipelineProfiler: A Visual Analytics Tool for the Exploration of AutoML Pipelines},
   volume = {27},
   year = {2021},
}
@inproceedings{Wang2021a,
   author = {Dakuo Wang and Josh Andres and Justin Weisz and Erick Oduor and Casey Dugan},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-12},
   publisher = {Association for Computing Machinery},
   title = {AutoDS: Towards Human-Centered Automation of Data Science},
   year = {2021},
}
@inproceedings{Wang2020,
   author = {Dakuo Wang and Parikshit Ram and Daniel Karl I. Weidele and Sijia Liu and Michael Muller and Justin D. Weisz and Abel Valente and Arunima Chaudhary and Dustin Torres and Horst Samulowitz and Lisa Amini},
   journal = {International Conference on Intelligent User Interfaces},
   pages = {77-78},
   publisher = {Association for Computing Machinery},
   title = {AutoAI: Automating the End-to-End AI Lifecycle with Humans-in-the-Loop},
   year = {2020},
}
@inproceedings{Cobbe2021,
   author = {Jennifer Cobbe and Michelle Seng Ah Lee and Jatinder Singh},
   journal = {Conference on Fairness, Accountability, and Transparency},
   title = {Reviewable Automated Decision-Making: A Framework for Accountable Algorithmic Systems},
   year = {2021},
}
@article{Chatzimparmpas2020,
   author = {A. Chatzimparmpas and R. M. Martins and I. Jusufi and K. Kucher and F. Rossi and A. Kerren},
   issue = {3},
   journal = {Computer Graphics Forum},
   pages = {713-756},
   title = {The State of the Art in Enhancing Trust in Machine Learning Models with the Use of Visualizations},
   volume = {39},
   year = {2020},
}
@inproceedings{Sun2020,
   author = {Dong Sun and Zezheng Feng and Yuanzhe Chen and Yong Wang and Jia Zeng and Mingxuan Yuan and Ting-Chuen Pong and Huamin Qu},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-13},
   publisher = {Association for Computing Machinery},
   title = {DFSeer: A Visual Analytics Approach to Facilitate Model Selection for Demand Forecasting},
   year = {2020},
}
@inproceedings{Yang2018,
   author = {Qian Yang and Jina Suh and Nan-Chen Chen and Gonzalo Ramos},
   journal = {Designing Interactive Systems Conference},
   pages = {573-584},
   title = {Grounding Interactive Machine Learning Tool Design in How Non-Experts Actually Build Models},
   year = {2018},
}
@inproceedings{Ribeiro2016,
   author = {Marco Tulio Ribeiro and Sameer Singh and Carlos Guestrin},
   journal = {International Conference on Knowledge Discovery and Data Mining},
   pages = {1135-1144},
   title = {“Why Should I Trust You?” Explaining the Predictions of Any Classifier},
   year = {2016},
}
@article{Wang2019a,
   author = {Dakuo Wang and Justin D. Weisz and Michael Muller and Parikshit Ram and Werner Geyer and Casey Dugan and Yla Tausczik and Horst Samulowitz and Alexander Gray},
   issue = {CSCW},
   journal = {Human-Computer Interaction},
   pages = {1-24},
   title = {Human-AI Collaboration in Data Science: Exploring Data Scientists' Perceptions of Automated AI},
   volume = {3},
   year = {2019},
}
@inproceedings{Zoller2021a,
   author = {Marc-André Zöller and Tien-Dung Nguyen and Marco F. Huber},
   doi = {https://doi.org/10.1007/978-3-030-74251-5_9},
   journal = {International Symposium on Intelligent Data Analysis},
   pages = {103-115},
   title = {Incremental Search Space Construction for Machine Learning Pipeline Synthesis},
   year = {2021},
}
@inproceedings{Liao2020,
   author = {Q. Vera Liao and Daniel Gruen and Sarah Miller},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-15},
   publisher = {Association for Computing Machinery},
   title = {Questioning the AI: Informing Design Practices for Explainable AI User Experiences},
   year = {2020},
}
@inproceedings{Zhang2020,
   author = {Yunfeng Zhang and Q. Vera Liao and Rachel K.E. Bellamy},
   journal = {Conference on Fairness, Accountability, and Transparency},
   pages = {295–305},
   title = {Effect of Confidence and Explanation on Accuracy and Trust Calibration in AI-Assisted Decision Making},
   year = {2020},
}
@inproceedings{Lage2018,
   author = {Isaac Lage and Andrew Slavin Ross and Been Kim and Samuel J. Gershman and Finale Doshi-Velez},
   journal = {International Conference on Neural Information Processing Systems},
   pages = {10180–10189},
   title = {Human-in-the-Loop Interpretability Prior},
   year = {2018},
}
@inproceedings{Honeycutt2020,
   author = {Donald R. Honeycutt and Mahsan Nourani and Eric D. Ragan},
   journal = {AAAI Conference on Human Computation and Crowdsourcing},
   pages = {63-72},
   title = {Soliciting human-in-the-loop user feedback for interactive machine learning reduces user trust and impressions of model accuracy},
   year = {2020},
}
@article{Chatzimparmpas2020a,
   author = {Angelos Chatzimparmpas and Rafael M. Martins and Ilir Jusufi and Andreas Kerren},
   issue = {3},
   journal = {Information Visualization},
   pages = {207-233},
   title = {A survey of surveys on the use of visualization for interpreting machine learning models},
   volume = {19},
   year = {2020},
}
@article{Afrabandpey2020,
   author = {Homayun Afrabandpey and Tomi Peltola and Juho Piironen and Aki Vehtari and Samuel Kaski},
   issue = {9-10},
   journal = {Machine Learning},
   pages = {1855-1876},
   title = {A decision-theoretic approach for model interpretability in Bayesian framework},
   volume = {109},
   year = {2020},
}
@inproceedings{Poursabzi-Sangdeh2021,
   author = {Forough Poursabzi-Sangdeh and Dan Goldstein and Jake Hofman and Jennifer Wortman Vaughan and Hanna Wallach},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-67},
   publisher = {Association for Computing Machinery},
   title = {Manipulating and Measuring Model Interpretability},
   year = {2021},
}
@inproceedings{Ledell2020,
   author = {E Ledell and S Poirier},
   journal = {International Conference on Machine Learning AutoML Workshop},
   title = {H2O AutoML: Scalable Automatic Machine Learning},
   year = {2020},
}
@article{Arya2019,
   author = {Vijay Arya and Rachel K. E. Bellamy and Pin-Yu Chen and Amit Dhurandhar and Michael Hind and Samuel C. Hoffman and Stephanie Houde and Q. Vera Liao and Ronny Luss and Aleksandra Mojsilović and Sami Mourad and Pablo Pedemonte and Ramya Raghavendra and John Richards and Prasanna Sattigeri and Karthikeyan Shanmugam and Moninder Singh and Kush R. Varshney and Dennis Wei and Yunfeng Zhang},
   journal = {arXiv: 1909.03012},
   title = {One Explanation Does Not Fit All: A Toolkit and Taxonomy of AI Explainability Techniques},
   year = {2019},
}
@inproceedings{Biedenkapp2019,
   author = {André Biedenkapp and Joshua Marben and Marius Lindauer and Frank Hutter},
   journal = {International Conference on Learning and Intelligent Optimization},
   pages = {115-130},
   title = {CAVE: configuration assessment, visualization and evaluation},
   year = {2018},
}
@inproceedings{Juozapaitis2019,
   author = {Zoe Juozapaitis and Anurag Koul and Alan Fern and Martin Erwig and Finale Doshi-velez},
   journal = {IJCAI/ECAI Workshop on Explainable Artificial Intelligence},
   title = {Explainable Reinforcement Learning via Reward Decomposition},
   year = {2019},
}
@inproceedings{Li2018a,
   author = {Tianyi Li and Gregorio Convertino and Wenbo Wang and Haley Most and Tristan Zajonc and Yi-Hsun Tsai},
   journal = {Machine Learning from User Interactions for Visualization and Analytics Workshop},
   title = {HyperTuner: Visual Analytics for Hyperparameter Tuning by Professionals},
   year = {2018},
}
@article{Hoffman2018,
   author = {Robert R. Hoffman and Shane T. Mueller and Gary Klein and Jordan Litman},
   journal = {arXiv: 1812.04608},
   pages = {1-50},
   title = {Metrics for Explainable AI: Challenges and Prospects},
   year = {2018},
}
@inproceedings{Liaw2018,
   author = {Richard Liaw and Eric Liang and Robert Nishihara and Philipp Moritz and Joseph E Gonzalez and Ion Stoica},
   journal = {arXiv: 1807.05118},
   pages = {1-8},
   title = {Tune: A Research Platform for Distributed Model Selection and Training},
   year = {2018},
}
@inproceedings{Weidele2019,
   abstract = {Parallel Coordinates [11],[12] are a popular data visualization technique for multivariate data. Dating back to as early as 1880 [8] PC are nearly as old as John Snow's famous cholera outbreak map [18] of 1855, which is frequently regarded as a historic landmark for modern data visualization. Numerous extensions have been proposed to address integrity, scalability and readability. We make a new case to employ PC on conditional data, where additional dimensions are only unfolded if certain criteria are met in an observation. Compared to standard PC which operate on a flat set of dimensions the ontology of our input to Conditional Parallel Coordinates is of hierarchical nature. We therefore briefly review related work around hierarchical PC using aggregation or nesting techniques. Our contribution is a visualization to seamlessly adapt PC for conditional data under preservation of intuitive interaction patterns to select or highlight polylines. We conclude with intuitions on how to operate CPC on two data sets: an AutoML hyperparameter search log, and session results from a conversational agent.},
   author = {Daniel Karl I. Weidele},
   journal = {IEEE Visualization Conference},
   keywords = {Human-centered computing,Visualization,Visualization design and evaluation methods,Visualization techniques},
   pages = {221-225},
   publisher = {IEEE},
   title = {Conditional Parallel Coordinates},
   year = {2019},
}
@inproceedings{Akiba2019,
   author = {Takuya Akiba and Shotaro Sano and Toshihiko Yanase and Takeru Ohta and Masanori Koyama},
   isbn = {9781450362016},
   journal = {International Conference on Knowledge Discovery and Data Mining},
   keywords = {acm reference format,bayesian op-,black-box optimization,hyperparameter optimization,machine learning system,timization},
   pages = {2623-2631},
   publisher = {Association for Computing Machinery},
   title = {Optuna : A Next-generation Hyperparameter Optimization Framework},
   year = {2019},
}
@article{Liu2019,
   author = {Jiayi Liu and Samarth Tripathi and Unmseh Kurup and Mohak Shah},
   journal = {arXiv: 1911.02522},
   pages = {1-10},
   title = {Auptimizer - an Extensible, Open-Source Framework for Hyperparameter Tuning Jiayi},
   year = {2019},
}
@web_page{Dua2017,
   author = {Dheeru Dua and Casey Graff},
   title = {UCI Machine Learning Repository},
   url = {http://archive.ics.uci.edu/ml},
   year = {2017},
}
@web_page{Fedesoriano2021,
   author = {Fedesoriano},
   title = {Stroke Prediction Dataset},
   url = {https://www.kaggle.com/fedesoriano/stroke-prediction-dataset},
   year = {2021},
}
@inproceedings{Wang2021b,
   author = {Chi Wang and Qingyun Wu and Markus Weimer and Erkang Zhu},
   journal = {Machine Learning and Systems},
   pages = {434-447},
   title = {FLAML: A Fast and Lightweight AutoML Library},
   year = {2021},
}
@inproceedings{Muller2019,
   abstract = {With the rise of big data, there has been an increasing need for practitioners in this space and an increasing opportunity for researchers to understand their workflows and design new tools to improve it. Data science is often described as data-driven, comprising unambiguous data and proceeding through regularized steps of analysis. However, this view focuses more on abstract processes, pipelines, and workflows, and less on how data science workers engage with the data. In this paper, we build on the work of other CSCW and HCI researchers in describing the ways that scientists, scholars, engineers, and others work with their data, through analyses of interviews with 21 data science professionals. We set five approaches to data along a dimension of interventions: Data as given; as captured; as curated; as designed; and as created. Data science workers develop an intuitive sense of their data and processes, and actively shape their data. We propose new ways to apply these interventions analytically, to make sense of the complex activities around data practices.},
   author = {Michael Muller and Ingrid Lange and Dakuo Wang and David Piorkowski and Jason Tsay and Q. Vera Liao and Casey Dugan and Thomas Erickson},
   journal = {Conference on Human Factors in Computing Systems},
   keywords = {Data capture,Data creation,Data curation,Data design,Data discovery,Data science,Grounded theory,Work-practices},
   pages = {1-14},
   publisher = {Association for Computing Machinery},
   title = {How Data Science Workers Work with Data: Discovery, Capture, Curation, Design, Creation},
   year = {2019},
}
@web_page{DataRobot2021,
   author = {DataRobot},
   title = {AI Cloud},
   url = {https://www.datarobot.com/platform/},
   year = {2021},
}
@article{Brooke1996,
   author = {John Brooke},
   issue = {194},
   journal = {Usability Evaluation In Industry},
   pages = {4-7},
   title = {SUS: A 'Quick and Dirty' Usability Scale},
   volume = {189},
   year = {1996},
}
@inproceedings{Grappiolo2019,
   author = {Corrado Grappiolo and Emile Van Gerwen and Jack Verhoosel and Lou Somers},
   journal = {Conference on Human Information Interaction and Retrieval},
   pages = {355-359},
   publisher = {Association for Computing Machinery},
   title = {The Semantic Snake Charmer Search Engine: A Tool to Facilitate Data Science in High-tech Industry Domains},
   year = {2019},
}
@article{Karaca2021,
   author = {Koray Karaca},
   issue = {4},
   journal = {European Journal for Philosophy of Science},
   keywords = {Inductive risk,Machine learning,Social values,Underdetermination of model construction},
   pages = {1-27},
   publisher = {Springer Netherlands},
   title = {Values and Inductive Risk in Machine Learning Modelling: The Case of Binary Classification Models},
   volume = {11},
   year = {2021},
}
@web_page{Recharts2015,
   author = {Recharts Group},
   title = {Recharts - A Composable Charting Library Built on React Components},
   url = {https://recharts.org/},
   year = {2015},
}
@web_page{React2013,
   author = {Meta Platforms Inc.},
   title = {React - A JavaScript library for building user interfaces},
   url = {https://reactjs.org/},
   year = {2013},
}
@article{Bostock2011,
   author = {Michael Bostock and Vadim Ogievetsky and Jeffrey Heer},
   issue = {12},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   pages = {2301-2309},
   title = {D3: Data-Driven Documents},
   volume = {17},
   year = {2011},
}
@inproceedings{McKinney2010,
   abstract = {In this paper we are concerned with the practical issues of working with data sets common to finance, statistics, and other related fields. pandas is a new library which aims to facilitate working with these data sets and to provide a set of fundamental building blocks for implementing statistical models. We will discuss specific design issues encountered in the course of developing pandas with relevant examples and some comparisons with the R language. We conclude by discussing possible future directions for statistical computing and data analysis using Python.},
   author = {Wes McKinney},
   journal = {Python in Science Conference},
   pages = {56-61},
   title = {Data Structures for Statistical Computing in Python},
   year = {2010},
}
@article{VanDerWalt2011,
   author = {Stéfan Van Der Walt and S. Chris Colbert and Gaël Varoquaux},
   issue = {2},
   journal = {Computing in Science and Engineering},
   keywords = {NumPy,Python,numerical computations,programming libraries,scientific programming},
   pages = {22-30},
   title = {The NumPy Array: A structure for Efficient Numerical Computation},
   volume = {13},
   year = {2011},
}
@web_page{GoogleTrends2022,
   author = {Google LLC},
   title = {Google Search Trends},
   url = {https://trends.google.com/trends/explore?date=today 5-y&q=automl,machine learning},
   year = {2022},
}
@inproceedings{Doran2017,
   author = {Derek Doran and Sarah Schulz and Tarek R. Besold},
   journal = {Workshop on Comprehensibility and Explanation in AI and ML},
   pages = {1-8},
   title = {What Does Explainable AI Really Mean? A New Conceptualization of Perspectives},
   year = {2017},
}
@article{Yang2020,
   abstract = {Data scientists seeking a good supervised learning model on a dataset have many choices to make: they must preprocess the data, select features, possibly reduce the dimension, select an estimation algorithm, and choose hyperparameters for each of these pipeline components. With new pipeline components comes a combinatorial explosion in the number of choices In this work, we design a new AutoML system TensorOboe to address this challenge: an automated system to design a supervised learning pipeline. TensorOboe uses low rank tensor decomposition as a surrogate model for efficient pipeline search. We also develop a new greedy experiment design protocol to gather information about a new dataset efficiently. Experiments on large corpora of real-world classification problems demonstrate the effectiveness of our approach.},
   author = {Chengrun Yang and Jicong Fan and Ziyang Wu and Madeleine Udell},
   journal = {Proceedings of the ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
   keywords = {AutoML,experiment design,greedy algorithms,meta-learning,pipeline search,submodular optimization,tensor decomposition},
   pages = {1446-1456},
   title = {AutoML Pipeline Selection: Efficiently Navigating the Combinatorial Space},
   year = {2020},
}
@article{Vehtari2012,
   abstract = {To date, several methods exist in the statistical literature for model assessment, which purport themselves specifically as Bayesian predictive methods. The decision theoretic assumptions on which these methods are based are not always clearly stated in the original articles, however. The aim of this survey is to provide a unified review of Bayesian predictive model assessment and selection methods, and of methods closely related to them. We review the various assumptions that are made in this context and discuss the connections between different approaches, with an emphasis on how each method approximates the expected utility of using a Bayesian model for the purpose of predicting future data. © 2013 The author, under a Creative Commons Attribution License.},
   author = {Aki Vehtari and Janne Ojanen},
   doi = {10.1214/12-ss102},
   issn = {19357516},
   issue = {1},
   journal = {Statistics Surveys},
   keywords = {Bayesian,Cross-validation,Decision theory,Expected utility,Information criteria,Model assessment,Model selection,Predictive},
   pages = {142-228},
   title = {A survey of Bayesian predictive methods for model assessment, selection and comparison},
   volume = {6},
   year = {2012},
}
@article{Friedman2001,
   author = {Jerome Friedman},
   issue = {5},
   journal = {The Annals of Statistics},
   pages = {1189-1232},
   title = {Greedy Function Approximation : A Gradient Boosting Machine},
   volume = {29},
   year = {2001},
}
@article{Goldstein2015,
   author = {Alex Goldstein and Adam Kapelner and Justin Bleich and Emil Pitkin},
   issue = {1},
   journal = {Journal of Computational and Graphical Statistics},
   keywords = {Exploratory data analysis,Graphical method,Model visualization},
   pages = {44-65},
   title = {Peeking Inside the Black Box: Visualizing Statistical Learning With Plots of Individual Conditional Expectation},
   volume = {24},
   year = {2015},
}
@book{Molnar2019,
   author = {Christoph Molnar},
   title = {Interpretable machine learning. A Guide for Making Black Box Models Explainable},
   year = {2019},
}
@article{Hinterreiter2021,
   abstract = {In problem-solving, a path towards a solutions can be viewed as a sequence of decisions. The decisions, made by humans or computers, describe a trajectory through a high-dimensional representation space of the problem. By means of dimensionality reduction, these trajectories can be visualized in lower-dimensional space. Such embedded trajectories have previously been applied to a wide variety of data, but analysis has focused almost exclusively on the self-similarity of single trajectories. In contrast, we describe patterns emerging from drawing many trajectories—for different initial conditions, end states, and solution strategies—in the same embedding space. We argue that general statements about the problem-solving tasks and solving strategies can be made by interpreting these patterns. We explore and characterize such patterns in trajectories resulting from human and machine-made decisions in a variety of application domains: logic puzzles (Rubik’s cube), strategy games (chess), and optimization problems (neural network training). We also discuss the importance of suitably chosen representation spaces and similarity metrics for the embedding.},
   author = {Andreas Hinterreiter and Christian Steinparz and Moritz SchÖfl and Holger Stitz and Marc Streit},
   doi = {10.1145/3387165},
   issn = {2160-6455},
   issue = {3-4},
   journal = {ACM Transactions on Interactive Intelligent Systems},
   pages = {1-29},
   title = {Projection Path Explorer: Exploring Visual Patterns in Projected Decision-making Paths},
   volume = {11},
   year = {2021},
}
@article{Liu2017,
   author = {Shixia Liu and Xiting Wang and Mengchen Liu and Jun Zhu},
   issue = {1},
   journal = {Visual Informatics},
   keywords = {Diagnosis,Interactive model analysis,Interactive visualization,Machine learning,Refinement,Understanding},
   pages = {48-56},
   title = {Towards Better Analysis of Machine Learning Models: A Visual Analytics Perspective},
   volume = {1},
   year = {2017},
}
@article{Spinner2019,
   author = {Thilo Spinner and Udo Schlegel and Hanna Schäfer and Mennatallah El-Assady},
   issue = {1},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   keywords = {Deep Learning,Explainability,Explainable AI,Interactive Machine Learning,Interpretability,Visual Analytics},
   pages = {1064-1074},
   title = {explAIner: A Visual Analytics Framework for Interactive and Explainable Machine Learning},
   volume = {26},
   year = {2019},
}
@inproceedings{Santos2019,
   author = {Aecio Santos and Sonia Castelo and Cristian Felix and Jorge Piazentin Ono and Bowen Yu and Sungsoo Hong and Claudio T. Silva and Enrico Bertini and Juliana Freire},
   journal = {Workshop on Human-In-the-Loop Data Analytics},
   keywords = {Automatic machine learning,Data analytics,Data visualization},
   pages = {1-7},
   publisher = {Association for Computing Machinery},
   title = {Visus: An Interactive System for Automatic Machine Learning Model Building and Curation},
   year = {2019},
}
@inproceedings{Amershi2015,
   author = {Saleema Amershi and Max Chickering and Steven M. Drucker and Bongshin Lee and Patrice Simard and Jina Suh},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {337-346},
   publisher = {Association for Computing Machinery},
   title = {ModelTracker: Redesigning Performance Analysis Tools for Machine Learning},
   year = {2015},
}
@article{Ren2017,
   author = {Donghao Ren and Saleema Amershi and Bongshin Lee and Jina Suh and Jason D. Williams},
   issue = {1},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   keywords = {Performance analysis,classification,usable machine learning},
   pages = {61-70},
   title = {Squares: Supporting Interactive Performance Analysis for Multiclass Classifiers},
   volume = {23},
   year = {2017},
}
@article{Cashman2019,
   author = {Dylan Cashman and Shah Rukh Humayoun and Florian Heimerl and Kendall Park and Subhajit Das and John Thompson and Bahador Saket and Abigail Mosca and John Stasko and Alex Endert and Michael Gleicher and Remco Chang},
   issue = {3},
   journal = {Computer Graphics Forum},
   keywords = {Computing methodologies → Model development and an,Human-centered computing → Visual analytics,Mathematics of computing → Exploratory data analys},
   pages = {185-199},
   title = {A User-based Visual Analytics Workflow for Exploratory Model Analysis},
   volume = {38},
   year = {2019},
}
@article{Lu2017,
   author = {Yafeng Lu and Rolando Garcia and Brett Hansen and Michael Gleicher and Ross Maciejewski},
   issue = {3},
   journal = {Computer Graphics Forum},
   pages = {539-562},
   title = {The State-of-the-Art in Predictive Visual Analytics},
   volume = {36},
   year = {2017},
}
@inproceedings{Heyen2020,
   abstract = {We propose ClaVis, a visual analytics system for comparative analysis of classification models. ClaVis allows users to visually compare the performance and behavior of tens to hundreds of classifiers trained with different hyperparameter configurations. Our approach is plugin-based and classifier-agnostic and allows users to add their own datasets and classifier implementations. It provides multiple visualizations, including a multivariate ranking, a similarity map, a scatterplot that reveals correlations between parameters and scores, and a training history chart. We demonstrate the effectivity of our approach in multiple case studies for training classification models in the domain of natural language processing.},
   author = {Frank Heyen and Tanja Munz and Michael Neumann and Daniel Ortega and Ngoc Thang Vu and Daniel Weiskopf and Michael Sedlmair},
   journal = {Conference on Advanced Visual Interfaces},
   keywords = {Visualization,classifier comparison,machine learning,visual analytics},
   pages = {1-9},
   publisher = {Association for Computing Machinery},
   title = {ClaVis: An Interactive Visual Comparison System for Classifiers},
   year = {2020},
}
@inproceedings{Gleicher2020,
   author = {Michael Gleicher and Aditya Barve and Xinyi Yu and Florian Heimerl},
   journal = {Computer Graphics Forum},
   keywords = {CCS Concepts,Information visualization,Visual analytics,• Human-centered computing → Visualization},
   pages = {181-193},
   publisher = {Association for Computing Machinery},
   title = {Boxer: Interactive Comparison of Classifier Results},
   year = {2020},
}
@inproceedings{Yin2019,
   abstract = {We address a relatively under-explored aspect of human–computer interaction: people’s abilities to understand the relationship between a machine learning model’s stated performance on held-out data and its expected performance post deployment. We conduct large-scale, randomized human-subject experiments to examine whether laypeople’s trust in a model, measured in terms of both the frequency with which they revise their predictions to match those of the model and their self-reported levels of trust in the model, varies depending on the model’s stated accuracy on held-out data and on its observed accuracy in practice. We find that people’s trust in a model is affected by both its stated accuracy and its observed accuracy, and that the effect of stated accuracy can change depending on the observed accuracy. Our work relates to recent research on interpretable machine learning, but moves beyond the typical focus on model internals, exploring a different component of the machine learning pipeline.},
   author = {Ming Yin and Jennifer Wortman Vaughan and Hanna Wallach},
   journal = {Conference on Human Factors in Computing Systems},
   keywords = {Human-subject experiments,Machine learning,Trust},
   pages = {1-12},
   title = {Understanding the effect of accuracy on trust in machine learning models},
   year = {2019},
}
@article{Lee2004,
   author = {John D. Lee and Katrina A. See},
   issue = {1},
   journal = {Human Factors},
   pages = {50-80},
   title = {Trust in Automation: Designing for Appropriate Reliance},
   volume = {46},
   year = {2004},
}
@article{Siau2018,
   author = {Keng Siau and Weiyu Wang},
   issue = {2},
   journal = {Cutter Business Technology Journal},
   pages = {47-53},
   title = {Building Trust in Artificial Intelligence, Machine Learning, and Robotics},
   volume = {31},
   year = {2018},
}
@article{Batch2018,
   author = {Andrea Batch and Niklas Elmqvist},
   issue = {1},
   journal = {IEEE Transactions on Visualization and Computer Graphics},
   keywords = {Data science,contextual inquiry,semi-structured interviews,visual analytics,visualization},
   pages = {278-287},
   publisher = {IEEE},
   title = {The Interactive Visualization Gap in Initial Exploratory Data Analysis},
   volume = {24},
   year = {2018},
}
@article{Waskom2021,
   author = {Michael L. Waskom},
   issue = {60},
   journal = {Journal of Open Source Software},
   pages = {3021-3025},
   title = {Seaborn: Statistical Data Visualization},
   volume = {6},
   year = {2021},
}
@book{Chen2007,
   author = {Chun-Houh Chen and Wolfgang Karl Härdle and Antonz Unwin},
   title = {Handbook of Data Visualization},
   year = {2007},
}
@article{Perer2008,
   abstract = {Although both statistical methods and visualizations have been used by network analysts, exploratory data analysis remains a challenge. We propose that a tight integration of these technologies in an interactive exploratory tool could dramatically speed insight development. To test the power of this integrated approach, we created a novel social network analysis tool, SocialAction, and conducted four long-term case studies with domain experts, each working on unique data sets with unique problems. The structured replicated case studies show that the integrated approach in SocialAction led to significant discoveries by a political analyst, a bibliometrician, a healthcare consultant, and a counter-terrorism researcher. demonstrate that the tight Our contributions integration of statistics and visualizations improves exploratory data analysis, and that our evaluation methodology for long-term case studies captures the research strategies of data analysts.},
   author = {Adam Perer and Ben Shneiderman},
   doi = {10.1145/1357054.1357101},
   isbn = {9781605580111},
   pages = {265},
   title = {Integrating Statistics and Visualization: Case Studies of Gaining Clarity during Exploratory Data Analysis},
   year = {2008},
}
@article{Adadi2018,
   author = {Amina Adadi and Mohammed Berrada},
   journal = {IEEE Access},
   keywords = {Explainable artificial intelligence,black-box models,interpretable machine learning},
   pages = {52138-52160},
   publisher = {IEEE},
   title = {Peeking Inside the Black-Box: A Survey on Explainable Artificial Intelligence (XAI)},
   volume = {6},
   year = {2018},
}
@inproceedings{Rule2018,
   author = {Adam Rule and Aurélien Tabard and James D. Hollan},
   journal = {Conference on Human Factors in Computing Systems},
   pages = {1-12},
   publisher = {Association for Computing Machinery},
   title = {Exploration and Explanation in Computational Notebooks},
   year = {2018},
}
@web_page{JupyterLab2022,
   author = {Project Jupyter},
   title = {JupyterLab},
   url = {https://jupyter.org/},
   year = {2018},
}
@inproceedings{Kluyver2016,
   author = {Thomas Kluyver and Benjamin Ragan-Kelley and Fernando Pérez and Brian Granger and Matthias Bussonnier and Jonathan Frederic and Kyle Kelley and Jessica Hamrick and Jason Grout and Sylvain Corlay and Paul Ivanov and Damián Avila and Safia Abdalla and Carol Willing},
   journal = {Positioning and Power in Academic Publishing: Players, Agents and Agendas},
   pages = {87-90},
   publisher = {IOS Press BV},
   title = {Jupyter Notebooks—a publishing format for reproducible computational workflows},
   year = {2016},
}
@article{Knuth1984,
   author = {Donald E. Knuth},
   journal = {The Computer Journal},
   pages = {97-111},
   title = {Literate Programming},
   year = {1984},
}
@inproceedings{Zhang2020a,
   author = {Amy X. Zhang and Michael Muller and Dakuo Wang},
   issue = {CSCW1},
   journal = {Human-Computer Interaction},
   pages = {1-23},
   title = {How do Data Science Workers Collaborate? Roles, Workflows, and Tools},
   volume = {4},
   year = {2020},
}
@article{Bangor2008,
   author = {Aaron Bangor and Philip T. Kortum and James T. Miller},
   issue = {6},
   journal = {International Journal of Human-Computer Interaction},
   pages = {574-594},
   title = {An Empirical Evaluation of the System Usability Scale},
   volume = {24},
   year = {2008},
}
@inproceedings{Inselberg1990,
   author = {Alfred Inselberg and Bernard Dimsdale},
   journal = {IEEE Conference on Visualization},
   pages = {361-378},
   title = {Parallel Coordinates: A Tool for Visualizing Multi-Dimensional Geometry},
   year = {1990},
}
@article{Kuhn1955,
   author = {H. W. Kuhn},
   issue = {1-2},
   journal = {Naval research logistics quarterly},
   pages = {83-97},
   title = {The Hungarian method for the assignment problem},
   volume = {2},
   year = {1955},
}
@book_section{Serrat2017,
   author = {Olivier Serrat},
   journal = {Knowledge Solutions: Tools, Methods, and Approaches to Drive Organizational Performance},
   pages = {307-310},
   publisher = {Springer Singapore},
   title = {The Five Whys Technique},
   year = {2017},
}
@article{Pearson1901,
   author = {Karl Pearson},
   issn = {1941-5982},
   issue = {11},
   journal = {The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
   pages = {559-572},
   title = {LIII. On lines and planes of closest fit to systems of points in space},
   volume = {2},
   year = {1901},
}
@inproceedings{Schaaf2019,
   author = {Nina Schaaf and Marco Huber and Johannes Maucher},
   journal = {IEEE International Conference on Machine Learning and Applications},
   keywords = {Artificial intelligence,Decision tree,Deep learning,Explainability,Machine learning,Neural networks,Regularization,Xai},
   pages = {42-49},
   title = {Enhancing Decision Tree based Interpretation of Deep Neural Networks through L1-Orthogonal Regularization},
   year = {2019},
}
@article{Lipton2018,
   author = {Zachary C. Lipton},
   issue = {3},
   journal = {Queue},
   pages = {31-57},
   title = {The Mythos of Model Interpretability: In Machine Learning, the Concept of Interpretability is Both Important and Slippery},
   volume = {16},
   year = {2018},
}
@book{Cohen1988,
   author = {Jacob Cohen},
   pages = {20-26},
   publisher = {Lawrence Earlbaum Associates},
   title = {Statistical Power Analysis for the Behavioral Sciences},
   year = {1988},
}
@article{Zoller2022,
   abstract = {In the last ten years, various automated machine learning (AutoML) systems have been proposed to build end-to-end machine learning (ML) pipelines with minimal human interaction. Even though such automatically synthesized ML pipelines are able to achieve a competitive performance, recent studies have shown that users do not trust models constructed by AutoML due to missing transparency of AutoML systems and missing explanations for the constructed ML pipelines. In a requirements analysis study with 26 domain experts, data scientists, and AutoML researchers from different professions with vastly different expertise in ML, we collect detailed informational needs to establish trust in AutoML. We propose XAutoML, an interactive visual analytics tool for explaining arbitrary AutoML optimization procedures and ML pipelines constructed by AutoML. XAutoML combines interactive visualizations with established techniques from explainable artificial intelligence (XAI) to make the complete AutoML procedure transparent and explainable. By integrating XAutoML with JupyterLab, experienced users can extend the visual analytics with ad-hoc visualizations based on information extracted from XAutoML. We validate our approach in a user study with the same diverse user group from the requirements analysis. All participants were able to extract useful information from XAutoML, leading to a significantly increased trust in ML pipelines produced by AutoML and the AutoML optimization itself.},
   author = {Marc-André Zöller and Waldemar Titov and Thomas Schlegel and Marco F. Huber},
   journal = {arXiv: 2202.11954},
   keywords = {AutoML,Automated Machine Learning,Explainable AI,Transparency,XAI},
   publisher = {Association for Computing Machinery},
   title = {XAutoML: A Visual Analytics Tool for Understanding and Validating Automated Machine Learning},
   url = {http://arxiv.org/abs/2202.11954},
   year = {2022},
}
@inproceedings{Shah2021,
   abstract = {A large number of time series forecasting models including traditional statistical models, machine learning models and more recently deep learning have been proposed in the literature. However, choosing the right model along with good parameter values that performs well on a given data is still challenging. Automatically providing a good set of models to users for a given dataset saves both time and effort from using trial-and-error approaches with a wide variety of available models along with parameter optimization. We present AutoAI for Time Series Forecasting (AutoAI-TS) that provides users with a zero configuration (zero-conf) system to efficiently train, optimize and choose best forecasting model among various classes of models for the given dataset. With its flexible zero-conf design, AutoAI-TS automatically performs all the data preparation, model creation, parameter optimization, training and model selection for users and provides a trained model that is ready to use. For given data, AutoAI-TS utilizes a wide variety of models including classical statistical models, Machine Learning (ML) models, statistical-ML hybrid models and deep learning models along with various transformations to create forecasting pipelines. It then evaluates and ranks pipelines using the proposed T-Daub mechanism to choose the best pipeline. The paper describe in detail all the technical aspects of AutoAI-TS along with extensive benchmarking on a variety of real world data sets for various use-cases. Benchmark results show that AutoAI-TS, with no manual configuration from the user, automatically trains and selects pipelines that on average outperform existing state-of-the-art time series forecasting toolkits.},
   author = {Syed Yousaf Shah and Dhaval Patel and Long Vu and Xuan Hong Dang and Bei Chen and Peter Kirchner and Horst Samulowitz and David Wood and Gregory Bramble and Wesley M. Gifford and Giridhar Ganapavarapu and Roman Vaculin and Petros Zerfos},
   isbn = {9781450383431},
   issn = {07308078},
   booktitle = {SIGMOD},
   keywords = {automl,machine learning,ml pipelines,optimization,time series},
   pages = {2584-2596},
   title = {AutoAI-TS: AutoAI for Time Series Forecasting},
   year = {2021},
}
@article{Paldino2021,
   abstract = {The availability of massive amounts of temporal data opens new perspectives of knowledge extraction and automated decision making for companies and practitioners. However, learning forecasting models from data requires a knowledgeable data science or machine learning (ML) background and expertise, which is not always available to end-users. This gap fosters a growing demand for frameworks automating the ML pipeline and ensuring broader access to the general public. Automatic machine learning (AutoML) provides solutions to build and validate machine learning pipelines minimizing the user intervention. Most of those pipelines have been validated in static supervised learning settings, while an extensive validation in time series prediction is still missing. This issue is particularly important in the forecasting community, where the relevance of machine learning approaches is still under debate. This paper assesses four existing AutoML frameworks (AutoGluon, H2O, TPOT, Auto-sklearn) on a number of forecasting challenges (univariate and multivariate, single-step and multi-step ahead) by benchmarking them against simple and conventional forecasting strategies (e.g., naive and exponential smoothing). The obtained results highlight that AutoML approaches are not yet mature enough to address generic forecasting tasks once compared with faster yet more basic statistical forecasters. In particular, the tested AutoML configurations, on average, do not significantly outperform a Naive estimator. Those results, yet preliminary, should not be interpreted as a rejection of AutoML solutions in forecasting but as an encouragement to a more rigorous validation of their limits and perspectives.},
   author = {Gian Marco Paldino and Jacopo De Stefani and Fabrizio De Caro and Gianluca Bontempi},
   doi = {10.3390/engproc2021005036},
   issue = {36},
   journal = {Engineering Proceedings},
   pages = {1-10},
   title = {Does AutoML Outperform Naive Forecasting?},
   volume = {5},
   year = {2021},
}
@phdthesis{Morten2020,
   author = {Siem Morten Johannes Dahl},
   school = {Universidade Nova de Lisboa},
   title = {TSPO: An AutoML Approach to Time Series Forecasting},
   year = {2020},
}
@inproceedings{Kurian2021,
   author = {John Joy Kurian and Marcel Dix and Ido Amihai and Glenn Ceusters and Ajinkya Prabhune},
   isbn = {9781665434836},
   booktitle = {IEEE BigDataService},
   pages = {17-24},
   title = {BOAT: A Bayesian Optimization AutoML Time-series Framework for Industrial Applications},
   year = {2021},
}
@inproceedings{Javeri2021,
   abstract = {Statistical methods such as the Box-Jenkins method for time-series forecasting have been prominent since their development in 1970. Many researchers rely on such models as they can be efficiently estimated and also provide interpretability. However, advances in machine learning research indicate that neural networks can be powerful data modeling techniques, as they can give higher accuracy for a plethora of learning problems and datasets. In the past, they have been tried on time-series forecasting as well, but their overall results have not been significantly better than the statistical models especially for intermediate length times series data. Their modeling capacities are limited in cases where enough data may not be available to estimate the large number of parameters that these non-linear models require. This paper presents an easy to implement data augmentation method to significantly improve the performance of such networks. Our method, Augmented-Neural-Network, which involves using forecasts from statistical models, can help unlock the power of neural networks on intermediate length time-series and produces competitive results. It shows that data augmentation, when paired with Automated Machine Learning techniques such as Neural Architecture Search, can help to find the best neural architecture for a given time-series. Using the combination of these, demonstrates significant enhancement in the forecasting accuracy of three neural network-based models for a COVID-19 dataset, with a maximum improvement in forecasting accuracy by 21.41%, 24.29%, and 16.42%, respectively, over the neural networks that do not use augmented data.},
   author = {Indrajeet Y. Javeri and Mohammadhossein Toutiaee and Ismailcem B. Arpinar and John A. Miller and Tom W. Miller},
   isbn = {9781665434836},
   booktitle = {IEEE BigDataService},
   pages = {1-8},
   title = {Improving Neural Networks for Time-Series Forecasting using Data Augmentation and AutoML},
   year = {2021},
}
@inproceedings{Xu2021,
   abstract = {Analyzing better time series with limited human effort is of interest to academia and industry. Driven by business scenarios, we organized the first Automated Time Series Regression challenge (AutoSeries) for the WSDM Cup 2020. We present its design, analysis, and post-hoc experiments. The code submission requirement precluded participants from any manual intervention, testing automated machine learning capabilities of solutions, across many datasets, under hardware and time limitations. We prepared 10 datasets from diverse application domains (sales, power consumption, air quality, traffic, and parking), featuring missing data, mixed continuous and categorical variables, and various sampling rates. Each dataset was split into a training and a test sequence (which was streamed, allowing models to continuously adapt). The setting of “time series regression”, differs from classical forecasting in that covariates at the present time are known. Great strides were made by participants to tackle this AutoSeries problem, as demonstrated by the jump in performance from the sample submission, and post-hoc comparisons with AutoGluon. Simple yet effective methods were used, based on feature engineering, LightGBM, and random search hyper-parameter tuning, addressing all aspects of the challenge. Our post-hoc analyses revealed that providing additional time did not yield significant improvements. The winners’ code was open-sourced (https://www.4paradigm.com/competition/autoseries2020 ).},
   author = {Zhen Xu and Wei Wei Tu and Isabelle Guyon},
   doi = {10.1007/978-3-030-86517-7_3},
   isbn = {9783030865160},
   issn = {16113349},
   journal = {Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
   pages = {36-51},
   title = {AutoML Meets Time Series Regression Design and Analysis of the AutoSeries Challenge},
   year = {2021},
}
@inproceedings{Parmentier2021,
   abstract = {Nowadays Automated Machine Learning, abbreviated AutoML, is recognized as a good solution to quickly find a model without spending too much time on the tedious task of selecting an algorithm and its associated hyperparameters. AutoML is well studied on traditional classification problems but has never been explored on Time Series Classification (TSC) problems. Yet, we show in this article that this problem is different enough to require specific approaches. Indeed, while the preprocessing phases need to be defined with classical ML algorithms, most of them are embedded within the algorithms for TSC. This particularity is mainly due to the fact that we are dealing with ordered data. Over the last decade, there has been a lot of interest for this problem and many new ML algorithms oriented toward TSC (ML-TSC) have blossomed. A practitioner facing a TSC use case, and searching for the most adequate algorithm now has a wide range of options, and will generally end up trying a few algorithms with standard hyperparameters, similarly to what happens in classical ML. Clearly, this is suboptimal. In this article we propose an AutoML solution called AutoTSC based on Evolutionary Algorithms (EAs) and its associated ML-TSC search space. AutoTSC, when tested against standard datasets from the UCR archive, outperforms both a Random Search on the proposed search space and TPOT a well known standard AutoML tool.},
   author = {Laurent Parmentier and Olivier Nicol and Laetitia Jourdan and Marie-Eleonore Kessaci},
   doi = {10.1109/ICTAI52525.2021.00067},
   isbn = {9781665408981},
   issn = {10823409},
   journal = {International Conference on Tools with Artificial Intelligence},
   keywords = {AutoML,Evolutionary Algorithms,Time Series Classification},
   pages = {412-419},
   publisher = {IEEE},
   title = {AutoTSC: Optimization Algorithm to Automatically Solve the Time Series Classification Problem},
   year = {2021},
}
@article{Faouzi2020,
   author = {Johann Faouzi and Hicham Janati},
   issn = {15337928},
   journal = {Journal of Machine Learning Research},
   keywords = {Classification,Machine learning,Python,Time series},
   pages = {1-6},
   title = {pyts: A Python Package for Time Series Classification},
   volume = {21},
   year = {2020},
}
@article{Lindauer2019,
   abstract = {Hyperparameter optimization and neural architecture search can become prohibitively expensive for regular black-box Bayesian optimization because the training and evaluation of a single model can easily take several hours. To overcome this, we introduce a comprehensive tool suite for effective multi-fidelity Bayesian optimization and the analysis of its runs. The suite, written in Python, provides a simple way to specify complex design spaces, a robust and efficient combination of Bayesian optimization and HyperBand, and a comprehensive analysis of the optimization process and its outcomes.},
   author = {Marius Lindauer and Joshua Marben and Philipp Müller and Katharina Eggensperger and Matthias Feurer and André Biedenkapp and Frank Hutter},
   journal = {arXiv: 1908.0675},
   pages = {1-5},
   title = {BOAH: A Tool Suite for Multi-Fidelity Bayesian Optimization & Analysis of Hyperparameters},
   url = {http://arxiv.org/abs/1908.06756},
   year = {2019},
}
@article{Gigerenzer2009,
   author = {Gerd Gigerenzer and Henry Brighton},
   doi = {10.1111/j.1756-8765.2008.01006.x},
   issn = {17568757},
   issue = {1},
   journal = {Topics in Cognitive Science},
   keywords = {Decision-making,Heuristics,Induction,Inferences,Rationality,Uncertainity},
   pages = {107-143},
   pmid = {25164802},
   title = {Homo Heuristicus: Why Biased Minds Make Better Inferences},
   volume = {1},
   year = {2009},
}
@article{Hasebrook2022,
   author = {Niklas Hasebrook and Felix Morsbach and Niclas Kennengießer and Jörg Franke and Frank Hutter and Ali Sunyaev},
   journal = {arXiv: 2203.01717},
   pages = {1-12},
   title = {Why Do Machine Learning Practitioners Still Use Manual Tuning ? A Qualitative Study},
   year = {2022},
}
@article{Hyndman2020,
   abstract = {Forecasting competitions are now so widespread that it is often forgotten how controversial they were when first held, and how influential they have been over the years. I briefly review the history of forecasting competitions, and discuss what we have learned about their design and implementation, and what they can tell us about forecasting. I also provide a few suggestions for potential future competitions, and for research about forecasting based on competitions.},
   author = {Rob J. Hyndman},
   doi = {10.1016/j.ijforecast.2019.03.015},
   issn = {01692070},
   issue = {1},
   journal = {International Journal of Forecasting},
   keywords = {Evaluation,Forecasting accuracy,Kaggle,M competitions,Neural networks,Prediction intervals,Probability scoring,Time series},
   pages = {7-14},
   title = {A brief history of forecasting competitions},
   volume = {36},
   year = {2020},
}
@article{Makridakis2020,
   author = {Spyros Makridakis and Evangelos Spiliotis and Vassilios Assimakopoulos},
   issn = {01692070},
   issue = {1},
   journal = {International Journal of Forecasting},
   pages = {54-74},
   publisher = {Elsevier},
   title = {The M4 Competition: 100,000 time series and 61 forecasting methods},
   volume = {36},
   year = {2020},
}
@article{Christ2018,
   author = {Maximilian Christ and Nils Braun and Julius Neuffer and Andreas W. Kempa-Liehr},
   doi = {10.1016/j.neucom.2018.03.067},
   issn = {18728286},
   journal = {Neurocomputing},
   pages = {72-77},
   publisher = {Elsevier},
   title = {Time Series FeatuRe Extraction on basis of Scalable Hypothesis tests (tsfresh – A Python package)},
   volume = {307},
   url = {https://doi.org/10.1016/j.neucom.2018.03.067},
   year = {2018},
}
@article{Ratz2019,
   author = {Martin Rätz and Amir Pasha Javadi and Marc Baranski and Konstantin Finkbeiner and Dirk Müller},
   journal = {Energy and Buildings},
   keywords = {Automated machine learning,Building automation and control,Building energy modeling,Data-driven modeling,Regression,Time-series forecasting},
   title = {Automated Data-driven Modeling of Building Energy Systems via Machine Learning Algorithms},
   volume = {202},
   year = {2019},
}
@article{Pereira2018,
   abstract = {Distributed computing is bringing many advantages in cost, flexibility and availability. However, it increases the demand for performance and reliability. Resources such as CPU, memory, storage and network bandwidth, are very susceptible of presenting software aging issues. Therefore, proactive actions, also known as software rejuvenation must be performed to avoid these issues. The identification of the best moment to perform software rejuvenation is not a simple task, mostly because it may affect the system's availability and reliability. To overcome this problem, we propose an automatic forecasting strategy to support the system administrators to choose the best moment to perform software rejuvenation. Our strategy uses six time series techniques: Drift, Simple Exponential Smoothing, Holt, Holt-Winters, Linear Regression, and ARIMA. In our proposal, the most suitable one is chosen automatically as the best fit for a particular scenario. Three case studies were performed to evaluate the efficiency of our automatic strategy. Our proposal aims to increase the system's availability while decreasing the QoS violation probability. In one of our experiments, we can observe a reduction of 92.3% in the system's downtime. This research supports decision making activities and opens possibilities to foster the usage of forecasting strategies when dealing with software aging phenomenon.},
   author = {Paulo Pereira and Jean Araujo and Rubens Matos and Nuno Preguica and Paulo Maciel},
   doi = {10.1109/PCCC.2018.8711347},
   isbn = {9781538668085},
   journal = {2018 IEEE 37th International Performance Computing and Communications Conference, IPCCC 2018},
   keywords = {forecasting,software aging,software rejuvenation,time series},
   publisher = {IEEE},
   title = {Software Rejuvenation in Computer Systems: An Automatic Forecasting Approach Based on Time Series},
   year = {2018},
}
@inproceedings{Zufle2020,
   author = {Marwin Zufle and Samuel Kounev},
   doi = {10.15439/2020F101},
   isbn = {9788395541674},
   journal = {Federated Conference on Computer Science and Information Systems},
   pages = {141-144},
   title = {A Framework for Time Series Preprocessing and History-based Forecasting Method Recommendation},
   volume = {21},
   year = {2020},
}
@inproceedings{Hvarfner2022,
   author = {Carl Hvarfner and Danny Stoll and Artyr Souza and Marius Lindauer and Frank Hutter and Luigi Nardi},
   booktitle = {ICLR},
   pages = {1-15},
   title = {piBO: Augmenting Acquisition Functions with User Beliefs for Bayesian Optimization},
   year = {2022},
}
@inproceedings{Deng2022,
   author = {Difan Deng and Florian Karl and Frank Hutter and Bernd Bischl and Marius Lindauer},
   issue = {Dl},
   booktitle = {ECML},
   keywords = {automl,deep learning,neural archi-,time series forecasting},
   title = {Efficient Automated Deep Learning for Time Series Forecasting},
   year = {2022},
}
@article{Alsahref2022,
   author = {Ahmad Alsahref and Karan Aggarwal and Sonia Manoj and Kumar Ashutosh},
   isbn = {0123456789},
   issn = {1886-1784},
   journal = {Archives of Computational Methods in Engineering},
   publisher = {Springer Netherlands},
   title = {Review of ML and AutoML Solutions to Forecast Time‑Series Data},
   year = {2022},
}
@article{Loning2019,
   author = {Markus Löning and Anthony Bagnall and Sajaysurya Ganesh and Viktor Kazakov and Jason Lines and Franz J. Király},
   journal = {arXiv: 1909.07872},
   title = {sktime: A Unified Interface for Machine Learning with Time Series},
   year = {2019},
}
@inproceedings{Hanussek2020,
   author = {Marc Hanussek and Matthias Blohm and Maximilien Kintz},
   doi = {10.1145/3448326.3448353},
   isbn = {9781450389266},
   journal = {International Conference on Artificial Intelligence, Robotics and Control},
   keywords = {automl,automl benchmark,machine learning,openml},
   pages = {29-32},
   title = {Can AutoML outperform humans? An evaluation on popular OpenML datasets using AutoML Benchmark},
   year = {2020},
}
@web_page{Guo2020,
   author = {Lei Guo and Jiaxin Zhang},
   title = {AutoML Faceoff: 15 Humans VS 2 Machines. Who won?},
   url = {https://towardsdatascience.com/automl-faceoff-2-machines-vs-15-humans-bfc9d03e590f},
   year = {2020},
}
@article{Wold1939,
   author = {Herman Wold},
   issue = {2},
   journal = {Journal of the Royal Statistical Society},
   pages = {295-298},
   title = {A Study in Analysis of Stationary Time Series},
   volume = {102},
   year = {1939},
}
@article{Mcknight2011,
   abstract = {Trust plays an important role in many Information Systems (IS)-enabled situations. Most IS research employs trust as a measure of interpersonal or person-to-firm relations, such as trust in a Web vendor or a virtual team member. Although trust in other people is important, this article suggests that trust in the Information Technology (IT) itself also plays a role in shaping IT-related beliefs and behavior. To advance trust and technology research, this article presents a set of trust in technology construct definitions and measures.We also empirically examine these constructmeasures using tests of convergent, discriminant, and nomological validity. This study contributes to the literature by providing: (a) a framework that differentiates trust in technology from trust in people, (b) a theory-based set of definitions necessary for investigating different kinds of trust in technology, and (c) validated trust in technology measures useful to research and practice. © 2011 ACM.},
   author = {D. Harrison McKnight and Michelle Carter and Jason Bennett Thatcher and Paul F. Clay},
   doi = {10.1145/1985347.1985353},
   issn = {2158656X},
   issue = {2},
   journal = {ACM Transactions on Management Information Systems},
   keywords = {Construct development,Trust,Trust in technology},
   pages = {1-25},
   title = {Trust in a Specific Technology: An Investigation of Its Components and Measures},
   volume = {2},
   year = {2011},
}
@generic{Zhang2022,
   author = {Chanyuan (Abigail) Zhang and Soohyun Cho and Miklos Vasarhelyi},
   journal = {International Journal of Accounting Information Systems},
   title = {Explainable Artificial Intelligence (XAI) in Auditing},
   year = {2022},
}
@article{Mohseni2021,
   abstract = { The need for interpretable and accountable intelligent systems grows along with the prevalence of artificial intelligence ( AI ) applications used in everyday life. Explainable AI ( XAI ) systems are intended to self-explain the reasoning behind system decisions and predictions. Researchers from different disciplines work together to define, design, and evaluate explainable systems. However, scholars from different disciplines focus on different objectives and fairly independent topics of XAI research, which poses challenges for identifying appropriate design and evaluation methodology and consolidating knowledge across efforts. To this end, this article presents a survey and framework intended to share knowledge and experiences of XAI design and evaluation methods across multiple disciplines. Aiming to support diverse design goals and evaluation methods in XAI research, after a thorough review of XAI related papers in the fields of machine learning, visualization, and human-computer interaction, we present a categorization of XAI design goals and evaluation methods. Our categorization presents the mapping between design goals for different XAI user groups and their evaluation methods. From our findings, we develop a framework with step-by-step design guidelines paired with evaluation methods to close the iterative design and evaluation cycles in multidisciplinary XAI teams. Further, we provide summarized ready-to-use tables of evaluation methods and recommendations for different goals in XAI research. },
   author = {Sina Mohseni and Niloofar Zarei and Eric D. Ragan},
   doi = {10.1145/3387166},
   issn = {2160-6455},
   issue = {3-4},
   journal = {ACM Transactions on Interactive Intelligent Systems},
   pages = {1-45},
   title = {A Multidisciplinary Survey and Framework for Design and Evaluation of Explainable AI Systems},
   volume = {11},
   year = {2021},
}
@article{Alshboul2021,
   author = {Odey Alshboul and Ali Shehadeh and Maha Al-Kasasbeh and Rabia Emhamed Al Mamlook and Neda Halalsheh and Muna Alkasasbeh},
   doi = {10.1108/ECAM-08-2020-0614},
   issn = {09699988},
   journal = {Engineering, Construction and Architectural Management},
   keywords = {Construction,Construction equipment,Construction planning},
   title = {Deep and machine learning approaches for forecasting the residual value of heavy construction equipment: a management decision support model},
   year = {2021},
}
@article{Shehadeh2021,
   author = {Ali Shehadeh and Odey Alshboul and Rabia Emhamed Al Mamlook and Ola Hamedat},
   doi = {10.1016/j.autcon.2021.103827},
   issn = {09265805},
   issue = {July},
   journal = {Automation in Construction},
   keywords = {Construction equipment,Machine learning,Performance metrics,Residual value},
   pages = {103827},
   publisher = {Elsevier B.V.},
   title = {Machine learning models for predicting the residual value of heavy construction equipment: An evaluation of modified decision tree, LightGBM, and XGBoost regression},
   volume = {129},
   url = {https://doi.org/10.1016/j.autcon.2021.103827},
   year = {2021},
}
@inproceedings{Mauthe2022,
   abstract = {The prognosis of the remaining useful life is one of the key tasks in prognostics and health management. This paper compares the performance of currently very popular neural network architectures in time series forecasting for remaining useful life prognosis under defined operating conditions. These include long short-term memory networks, gated recurrent unit networks, as well as temporal convolutional networks. In addition, feedforward neural networks and one-dimensional convolutional neural networks are considered. Furthermore, metrics for performance evaluation of remaining useful life prognosis are reviewed in this paper. Established metrics and new metrics specially adapted to the remaining useful life prognosis are both used for the performance evaluation of the neuronal network architectures. By the specific metrics, the requirements for the prognosis are considered more strongly. The evaluation of the networks for remaining useful life prognosis in this paper complements previous general assessments regarding the suitability of the approaches for time series forecasting. As it turns out, there are significant performance differences between the architectures.},
   author = {Fabian Mauthe and Marcel Braig and Peter Zeiler},
   doi = {10.3850/981-973-0000-00-0_esrel2022-paper},
   isbn = {981-973-0000-00-0},
   journal = {European Safety and Reliability Conference},
   keywords = {feedforward neural network,filter clogging,machine learning,operating conditions,prognosis,prognostics and health management,recurrent neural network,remaining useful life,temporal convolutional network},
   title = {Performance Evaluation of Neural Network Architectures on Time Series Condition Data for Remaining Useful Life Prognosis Under Defined Operating Conditions},
   year = {2022},
}
@inproceedings{Tornede2021,
   abstract = {Automated machine learning (AutoML) strives for automatically constructing and configuring compositions of machine learning algorithms, called pipelines, with the goal to optimize a suitable performance measure on a concrete learning task. So far, most AutoML tools are focused on standard problem classes, such as classification and regression. In the field of predictive maintenance, especially the estimation of remaining useful lifetime (RUL), the task of AutoML becomes more complex. In particular, a good feature representation for multivariate sensor data is essential to achieve good performance. Due to the need for methods generating feature representations, the search space of candidate pipelines enlarges. Moreover, the runtime of a single pipeline increases substantially. In this paper, we tackle these problems by partitioning the search space into two sub-spaces, one for feature extraction methods and one for regression methods, and employ cooperative coevolution for searching a good combination. Thereby, we benefit from the fact that the generated feature representations can be cached, whence the evaluation of multiple regressors based on the same feature representation speeds up, allowing the evaluation of more candidate pipelines. Experimentally, we show that our coevolutionary strategy performs superior to the baselines.},
   author = {Tanja Tornede and Alexander Tornede and Marcel Wever and Eyke Hüllermeier},
   doi = {10.1145/3449639.3459395},
   isbn = {9781450383509},
   journal = {Genetic and Evolutionary Computation Conference},
   keywords = {AutoML,Coevolution,Predictive maintenance,Remaining useful lifetime},
   pages = {368-376},
   title = {Coevolution of Remaining Useful Lifetime Estimation Pipelines for Automated Predictive Maintenance},
   year = {2021},
}
@article{Hasebrook2022,
   abstract = {Current advanced hyperparameter optimization (HPO) methods, such as Bayesian optimization, have high sampling efficiency and facilitate replicability. Nonetheless, machine learning (ML) practitioners (e.g., engineers, scientists) mostly apply less advanced HPO methods, which can increase resource consumption during HPO or lead to underoptimized ML models. Therefore, we suspect that practitioners choose their HPO method to achieve different goals, such as decrease practitioner effort and target audience compliance. To develop HPO methods that align with such goals, the reasons why practitioners decide for specific HPO methods must be unveiled and thoroughly understood. Because qualitative research is most suitable to uncover such reasons and find potential explanations for them, we conducted semi-structured interviews to explain why practitioners choose different HPO methods. The interviews revealed six principal practitioner goals (e.g., increasing model comprehension), and eleven key factors that impact decisions for HPO methods (e.g., available computing resources). We deepen the understanding about why practitioners decide for different HPO methods and outline recommendations for improvements of HPO methods by aligning them with practitioner goals.},
   author = {Niklas Hasebrook and Felix Morsbach and Niclas Kannengießer and Jörg Franke and Frank Hutter and Ali Sunyaev},
   title = {Why Do Machine Learning Practitioners Still Use Manual Tuning? A Qualitative Study},
   url = {http://arxiv.org/abs/2203.01717},
   year = {2022},
}
@inproceedings{daSilva2022,
   author = {Felipe Rooke da Silva and Alex Borges Vieira and Heder Soares Bernardino and Victor Aquiles Alencar and Lucas Ribeiro Pessamilio and Helio Jose Correa Barbosa},
   isbn = {978-1-6654-6708-7},
   booktitle = {IEEE CEC},
   pages = {1-7},
   title = {Automated Machine Learning for Time Series Prediction},
   year = {2022},
}
@article{Meisenbacher2022,
   author = {Stefan Meisenbacher and Marian Turowski and Kaleb Phipps and Martin Rätz and Dirk Müller and Veit Hagenmeyer and Ralf Mikut},
   issn = {1942-4787},
   journal = {WIREs Data Mining and Knowledge Discovery},
   title = {Review of automated time series forecasting pipelines},
   year = {2022},
}
@article{Elsayed2021,
   abstract = {Time series forecasting is a crucial task in machine learning, as it has a wide range of applications including but not limited to forecasting electricity consumption, traffic, and air quality. Traditional forecasting models rely on rolling averages, vector auto-regression and auto-regressive integrated moving averages. On the other hand, deep learning and matrix factorization models have been recently proposed to tackle the same problem with more competitive performance. However, one major drawback of such models is that they tend to be overly complex in comparison to traditional techniques. In this paper, we report the results of prominent deep learning models with respect to a well-known machine learning baseline, a Gradient Boosting Regression Tree (GBRT) model. Similar to the deep neural network (DNN) models, we transform the time series forecasting task into a window-based regression problem. Furthermore, we feature-engineered the input and output structure of the GBRT model, such that, for each training window, the target values are concatenated with external features, and then flattened to form one input instance for a multi-output GBRT model. We conducted a comparative study on nine datasets for eight state-of-the-art deep-learning models that were presented at top-level conferences in the last years. The results demonstrate that the window-based input transformation boosts the performance of a simple GBRT model to levels that outperform all state-of-the-art DNN models evaluated in this paper.},
   author = {Shereen Elsayed and Daniela Thyssens and Ahmed Rashed and Hadi Samer Jomaa and Lars Schmidt-Thieme},
   journal = {arXiv:2102.02118},
   title = {Do We Really Need Deep Learning Models for Time Series Forecasting?},
   year = {2021},
}
@article{Khuat2022,
   abstract = {As automated machine learning (AutoML) systems continue to progress in both sophistication and performance, it becomes important to understand the `how' and `why' of human-computer interaction (HCI) within these frameworks, both current and expected. Such a discussion is necessary for optimal system design, leveraging advanced data-processing capabilities to support decision-making involving humans, but it is also key to identifying the opportunities and risks presented by ever-increasing levels of machine autonomy. Within this context, we focus on the following questions: (i) How does HCI currently look like for state-of-the-art AutoML algorithms, especially during the stages of development, deployment, and maintenance? (ii) Do the expectations of HCI within AutoML frameworks vary for different types of users and stakeholders? (iii) How can HCI be managed so that AutoML solutions acquire human trust and broad acceptance? (iv) As AutoML systems become more autonomous and capable of learning from complex open-ended environments, will the fundamental nature of HCI evolve? To consider these questions, we project existing literature in HCI into the space of AutoML; this connection has, to date, largely been unexplored. In so doing, we review topics including user-interface design, human-bias mitigation, and trust in artificial intelligence (AI). Additionally, to rigorously gauge the future of HCI, we contemplate how AutoML may manifest in effectively open-ended environments. This discussion necessarily reviews projected developmental pathways for AutoML, such as the incorporation of reasoning, although the focus remains on how and why HCI may occur in such a framework rather than on any implementational details. Ultimately, this review serves to identify key research directions aimed at better facilitating the roles and modes of human interactions with both current and future AutoML systems.},
   author = {Thanh Tung Khuat and David Jacob Kedziora and Bogdan Gabrys},
   title = {The Roles and Modes of Human Interactions with Automated Machine Learning Systems},
   url = {http://arxiv.org/abs/2205.04139},
   year = {2022},
}
@inproceedings{Oreshkin2019,
   abstract = {We focus on solving the univariate times series point forecasting problem using deep learning. We propose a deep neural architecture based on backward and forward residual links and a very deep stack of fully-connected layers. The architecture has a number of desirable properties, being interpretable, applicable without modification to a wide array of target domains, and fast to train. We test the proposed architecture on several well-known datasets, including M3, M4 and TOURISM competition datasets containing time series from diverse domains. We demonstrate state-of-the-art performance for two configurations of N-BEATS for all the datasets, improving forecast accuracy by 11% over a statistical benchmark and by 3% over last year's winner of the M4 competition, a domain-adjusted hand-crafted hybrid between neural network and statistical time series models. The first configuration of our model does not employ any time-series-specific components and its performance on heterogeneous datasets strongly suggests that, contrarily to received wisdom, deep learning primitives such as residual blocks are by themselves sufficient to solve a wide range of forecasting problems. Finally, we demonstrate how the proposed architecture can be augmented to provide outputs that are interpretable without considerable loss in accuracy.},
   author = {Boris N. Oreshkin and Dmitri Carpov and Nicolas Chapados and Yoshua Bengio},
   booktitle = {ICLR},
   title = {N-BEATS: Neural basis expansion analysis for interpretable time series forecasting},
   year = {2019},
}
@article{Hagmeyer2021,
   abstract = {For a successful realization of prognostics and health management (PHM), the availability of sufficient run-to-failure data sets is a crucial factor. The sheer number of given data points holds less importance than the full coverage of the potential state space. However, full coverage is a major challenge in most industrial applications. Among other things, high investment and operating costs as well as the long service life of many technical systems make it difficult to acquire complete run-to-failure data sets. Consequently, in industrial applications data sets with specific deficiencies are frequently encountered. The development of appropriate methods to address such data scenarios is a fundamental research issue. Therefore, the purpose of this paper is to provide facilitation for this research. Accordingly, the paper starts by specifying the value and availability of data in PHM. Subsequently, criteria for characterizing data sets are defined independent of the actual PHM application. The criteria are used to identify typical data scenarios with specific deficiencies that possess significant relevance for industrial applications. Thereafter, the most comprehensive overview of data sets suitable for PHM and currently publicly accessible is provided. Thereby, not all previously identified data scenarios with their specific deficiencies are addressed by at least one data set. A program is established for the aforementioned facilitation of further research. One objective of the program is to create data sets reflecting these data scenarios using a test bench. First, possible applications and their degradation processes to be studied on the test bench are briefly characterized. Thereby, the final decision to select filtration as a test bench application is argued. Subsequently, the test bench created is introduced, including a description of the functional concept, pneumatic layout and components involved, as well as the filter media and test dusts employed. Typical run-to-failure trajectories are illustrated. Thereafter, the data set published under the name Preventive to Predictive Maintenance is presented. Additionally, a schedule for future releases of data sets on further industry-relevant data scenarios is sketched.},
   author = {Simon Hagmeyer and Fabian Mauthe and Peter Zeiler},
   doi = {10.36001/ijphm.2021.v12i2.3087},
   issn = {2153-2648},
   issue = {2},
   journal = {International Journal of Prognostics and Health Management},
   publisher = {PHM Society},
   title = {Creation of Publicly Available Data Sets for Prognostics and Diagnostics Addressing Data Scenarios Relevant to Industrial Applications},
   volume = {12},
   year = {2021},
}
@inproceedings{Zhou2020,
   abstract = {An essential task in predictive maintenance is the prediction of the Remaining Useful Life (RUL) through the analysis of multivariate time series. Using the sliding window method, Convolutional Neural Network (CNN) and conventional Recurrent Neural Network (RNN) approaches have produced impressive results on this matter, due to their ability to learn optimized features. However, sequence information is only partially modeled by CNN approaches. Due to the flatten mechanism in conventional RNNs, like Long Short Term Memories (LSTM), the temporal information within the window is not fully preserved. To exploit the multi-level temporal information, many approaches are proposed which combine CNN and RNN models. In this work, we propose a new LSTM variant called embedded convolutional LSTM (ECLSTM). In ECLSTM a group of different 1D convolutions is embedded into the LSTM structure. Through this, the temporal information is preserved between and within windows. Since the hyper-parameters of models require careful tuning, we also propose an automated prediction framework based on the Bayesian optimization with hyperband optimizer, which allows for efficient optimization of the network architecture. Finally, we show the superiority of our proposed ECLSTM approach over the state-of-the-art approaches on several widely used benchmark data sets for RUL Estimation.},
   author = {Yexu Zhou and Yuting Gao and Yiran Huang and Michael Hefenbrock and Till Riedel and Michael Beigl},
   journal = {European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases},
   pages = {461-477},
   title = {Automatic Remaining Useful Life Estimation Framework with Embedded Convolutional LSTM as the Backbone},
   year = {2020},
}
@article{Kamat2021,
   abstract = {Remaining Useful Life (RUL) estimation of rotating machinery based on their degradation data is vital for machine supervisors. Deep learning models are effectiveand popular methods for forecasting when rotating machinery such as bearings maymalfunction and ultimately break down. During healthy functioning of themachinery, however, RUL is ill-defined. To address this issue, this study recommendsusing anomaly monitoring during both RUL estimator training and operation.Essential time-domain data is extracted from the raw bearing vibration data, anddeep learning models are used to detect the onset of the anomaly. This further acts asa trigger for data-driven RUL estimation. The study employs an unsupervisedclustering approach for anomaly trend analysis and a semi-supervised method foranomaly detection and RUL estimation. The novel combined deep learning-basedanomaly-onset aware RUL estimation framework showed enhanced results on thebenchmarked PRONOSTIA bearings dataset under non-varying operatingconditions. The framework consisting of Autoencoder and Long Short TermMemory variants achieved an accuracy of over 90% in anomaly detection and RULprediction. In the future, the framework can be deployed under varying operationalsituations using the transfer learning approach},
   author = {Pooja Vinayak Kamat and Rekha Sugandhi and Satish Kumar},
   doi = {10.7717/peerj-cs.795},
   issn = {23765992},
   journal = {PeerJ Computer Science},
   keywords = {Anomaly detection,Autoencoder,Bearing,Clustering,Deep learning,K-means,Lstm,Predictive maintenance,Remaining useful life},
   publisher = {PeerJ Inc.},
   title = {Deep learning-based anomaly-onset aware remaining useful life estimation of bearings},
   volume = {7},
   year = {2021},
}
@article{Luo2022,
   abstract = {Accurate online capacity estimation and life prediction of lithium-ion batteries (LIBs) are crucial to large-scale commercial use for electric vehicles. The data-driven method lately has drawn great attention in this field due to efficient machine learning, but it remains an ongoing challenge in the feature extraction related to battery lifespan. Some studies focus on the features only in the battery constant current (CC) charging phase, regardless of the joint impact including the constant voltage (CV) charging phase on the battery aging, which can lead to estimation deviation. In this study, we analyze the features of the CC and CV phases using the optimized incremental capacity (IC) curve, showing the strong relevance between the IC curve in the CC phase as well as charging capacity in the CV phase and battery lifespan. Then, the life prediction model based on automated machine learning (AutoML) is established, which can automatically generate a suitable pipeline with less human intervention, overcoming the problem of redundant model information and high computational cost. The proposed method is verified on NASA’s LIBs cycle life datasets, with the MAE increased by 52.8% and RMSE increased by 48.3% compared to other methods using the same datasets and training method, accomplishing an obvious enhancement in online life prediction with small-scale datasets.},
   author = {Chenqiang Luo and Zhendong Zhang and Dongdong Qiao and Xin Lai and Yongying Li and Shunli Wang},
   doi = {10.3390/en15134594},
   issn = {19961073},
   issue = {13},
   journal = {Energies},
   keywords = {automated machine learning,incremental capacity,life prediction,lithium-ion battery},
   publisher = {MDPI},
   title = {Life Prediction under Charging Process of Lithium-Ion Batteries Based on AutoML},
   volume = {15},
   year = {2022},
}
@article{Erickson2020,
   abstract = {We introduce AutoGluon-Tabular, an open-source AutoML framework that requires only a single line of Python to train highly accurate machine learning models on an unprocessed tabular dataset such as a CSV file. Unlike existing AutoML frameworks that primarily focus on model/hyperparameter selection, AutoGluon-Tabular succeeds by ensembling multiple models and stacking them in multiple layers. Experiments reveal that our multi-layer combination of many models offers better use of allocated training time than seeking out the best. A second contribution is an extensive evaluation of public and commercial AutoML platforms including TPOT, H2O, AutoWEKA, auto-sklearn, AutoGluon, and Google AutoML Tables. Tests on a suite of 50 classification and regression tasks from Kaggle and the OpenML AutoML Benchmark reveal that AutoGluon is faster, more robust, and much more accurate. We find that AutoGluon often even outperforms the best-in-hindsight combination of all of its competitors. In two popular Kaggle competitions, AutoGluon beat 99% of the participating data scientists after merely 4h of training on the raw data.},
   author = {Nick Erickson and Jonas Mueller and Alexander Shirkov and Hang Zhang and Pedro Larroy and Mu Li and Alexander Smola},
   journal = {arXiv: 2003:06505},
   title = {AutoGluon-Tabular: Robust and Accurate AutoML for Structured Data},
   year = {2020},
}
@article{Nikitin2021,
   abstract = {The effectiveness of the machine learning methods for real-world tasks depends on the proper structure of the modeling pipeline. The proposed approach is aimed to automate the design of composite machine learning pipelines, which is equivalent to computation workflows that consist of models and data operations. The approach combines key ideas of both automated machine learning and workflow management systems. It designs the pipelines with a customizable graph-based structure, analyzes the obtained results, and reproduces them. The evolutionary approach is used for the flexible identification of pipeline structure. The additional algorithms for sensitivity analysis, atomization, and hyperparameter tuning are implemented to improve the effectiveness of the approach. Also, the software implementation on this approach is presented as an open-source framework. The set of experiments is conducted for the different datasets and tasks (classification, regression, time series forecasting). The obtained results confirm the correctness and effectiveness of the proposed approach in the comparison with the state-of-the-art competitors and baseline solutions.},
   author = {Nikolay O. Nikitin and Pavel Vychuzhanin and Mikhail Sarafanov and Iana S. Polonskaia and Ilia Revin and Irina V. Barabanova and Gleb Maximov and Anna V. Kalyuzhnaya and Alexander Boukhanovsky},
   doi = {10.1016/j.future.2021.08.022},
   journal = {Future Generation Computer Systems},
   title = {Automated Evolutionary Approach for the Design of Composite Machine Learning Pipelines},
   url = {http://arxiv.org/abs/2106.15397 http://dx.doi.org/10.1016/j.future.2021.08.022},
   year = {2021},
}
@article{Elsken2019,
   abstract = {Deep Learning has enabled remarkable progress over the last years on a variety of tasks, such as image recognition, speech recognition, and machine translation. One crucial aspect for this progress are novel neural architectures. Currently employed architectures have mostly been developed manually by human experts, which is a time-consuming and error-prone process. Because of this, there is growing interest in automated neural architecture search methods. We provide an overview of existing work in this field of research and categorize them according to three dimensions: search space, search strategy, and performance estimation strategy.},
   author = {Thomas Elsken and Jan Hendrik Metzen and Frank Hutter},
   journal = {Journal of Machine Learning Research},
   keywords = {AutoDL,AutoML,Neural Architecture Search,Performance Estimation Strategy,Search Space Design,Search Strategy},
   pages = {1-21},
   title = {Neural Architecture Search: A Survey},
   volume = {20},
   url = {http://jmlr.org/papers/v20/18-598.html.},
   year = {2019},
}
@article{Khelif2017,
   abstract = {Prognostics is a major activity in the field of prognostics and health management. It aims at increasing the reliability and safety of systems while reducing the maintenance cost by providing an estimate of the current health status and remaining useful life (RUL). Classical RUL estimation techniques are usually composed of different steps: estimations of a health indicator, degradation states, a failure threshold, and finally the RUL. In this work, a procedure that is able to estimate the RUL of equipment directly from sensor values without the need for estimating degradation states or a failure threshold is developed. A direct relation between sensor values or health indicators is modeled using a support vector regression. Using this procedure, the RUL can be estimated at any time instant of the degradation process. In addition, an offline wrapper variable selection is applied before training the prediction model. This step has a positive impact on the accuracy of the prediction while reducing the computational time compared to existing indirect RUL prediction methods. To assess the performance of the proposed approach, the Turbofan dataset, widely considered in the literature, is used. Experimental results show that the performance of the proposed method is competitive with other existing approaches.},
   author = {Racha Khelif and Brigitte Chebel-Morello and Simon Malinowski and Emna Laajili and Farhat Fnaiech and Noureddine Zerhouni},
   doi = {10.1109/TIE.2016.2623260},
   issn = {02780046},
   issue = {3},
   journal = {IEEE Transactions on Industrial Electronics},
   keywords = {Maintenance,monitoring,reliability},
   pages = {2276-2285},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Direct Remaining Useful Life Estimation Based on Support Vector Regression},
   volume = {64},
   year = {2017},
}
@inproceedings{Zheng2017,
   abstract = {Remaining Useful Life (RUL) of a component or a system is defined as the length from the current time to the end of the useful life. Accurate RUL estimation plays a critical role in Prognostics and Health Management(PHM). Data driven approaches for RUL estimation use sensor data and operational data to estimate RUL. Traditional regression based approaches and recent Convolutional Neural Network (CNN) approach use features created from sliding windows to build models. However, sequence information is not fully considered in these approaches. Sequence learning models such as Hidden Markov Models (HMMs) and Recurrent Neural Networks (RNNs) have flaws when modeling sequence information. HMMs are limited to discrete hidden states and are known to have issues when modeling long-term dependencies in the data. RNNs also have issues with long-term dependencies. In this work, we propose a Long Short-Term Memory (LSTM) approach for RUL estimation, which can make full use of the sensor sequence information and expose hidden patterns within sensor data with multiple operating conditions, fault and degradation models. Extensive experiments using three widely adopted Prognostics and Health Management data sets show that LSTM for RUL estimation significantly outperforms traditional approaches for RUL estimation as well as Convolutional Neural Network (CNN).},
   author = {Shuai Zheng and Kosta Ristovski and Ahmed Farahat and Chetan Gupta},
   doi = {10.1109/ICPHM.2017.7998311},
   isbn = {9781509057108},
   journal = {IEEE Conference on Prognostics and Health Management},
   pages = {88-95},
   title = {Long Short-Term Memory Network for Remaining Useful Life estimation},
   year = {2017},
}
@article{Singh2022,
   abstract = {Li-ion batteries have diversified applications in everyday life. The temperature change, overcharging and over-discharging, is playing critical roles in affecting battery life in a significant manner. In this paper, the deep learning-based method is applied for the prognostics of a single Li-ion battery. The proposed design uses a recurrent neural network variant, long–short-term memory. The model’s parameters are optimized through a genetic algorithm-based parameter selector. The method applies to a sequence of data values comprising of the voltage, the charge capacity, the current, and the temperature. The estimation of battery capacity is not only based on the current or defined state of battery, instead, it is generated on the complete data profile. The robustness of the model is tested by comparing it with techniques such as support vector regressor, Kalman filter, and neural networks on normal and noisy test sets. The paper also proposes a feature selection and engineering scheme for battery capacity prediction. The proposed model outperforms the techniques available in the literature with high generalization to noise and other perturbations. The model is independent of the section of the charging curve used for the prediction of battery capacity. Various experimentation has been conducted on the model and the results have been validated.},
   author = {Mukul Singh and Shrey Bansal and Vandana and B. K. Panigrahi and Akhil Garg},
   doi = {10.1115/1.4053326},
   issn = {1530-9827},
   issue = {4},
   journal = {Journal of Computing and Information Science in Engineering},
   publisher = {ASME International},
   title = {A Genetic Algorithm and RNN-LSTM Model for Remaining Battery Capacity Prediction},
   volume = {22},
   year = {2022},
}
@inproceedings{Pautrat2018,
   abstract = {One of the most interesting features of Bayesian optimization for direct policy search is that it can leverage priors (e.g., from simulation or from previous tasks) to accelerate learning on a robot. In this paper, we are interested in situations for which several priors exist but we do not know in advance which one fits best the current situation. We tackle this problem by introducing a novel acquisition function, called Most Likely Expected Improvement (MLEI), that combines the likelihood of the priors and the expected improvement. We evaluate this new acquisition function on a transfer learning task for a 5-DOF planar arm and on a possibly damaged, 6-legged robot that has to learn to walk on flat ground and on stairs, with priors corresponding to different stairs and different kinds of damages. Our results show that MLEI effectively identifies and exploits the priors, even when there is no obvious match between the current situations and the priors.},
   author = {Remi Pautrat and Konstantinos Chatzilygeroudis and Jean Baptiste Mouret},
   doi = {10.1109/ICRA.2018.8463197},
   isbn = {9781538630815},
   issn = {10504729},
   journal = {Proceedings - IEEE International Conference on Robotics and Automation},
   pages = {7571-7578},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Bayesian Optimization with Automatic Prior Selection for Data-Efficient Direct Policy Search},
   year = {2018},
}
@article{Mo2021,
   abstract = {With the advent of Industry 4.0, making accurate predictions of the remaining useful life (RUL) of industrial components has become a crucial aspect in predictive maintenance (PdM). To this aim, various Deep Neural Network (DNN) models have been proposed in the recent literature. However, while the architectures of these models have a large impact on their performance, they are usually determined empirically. To exclude the time-consuming process and the unnecessary computational cost of manually engineering these models, we present a Neural Architecture Search (NAS) technique based on an Evolutionary Algorithm (EA) applied to optimize the architecture of a DNN used to predict the RUL. The EA explores the combinatorial parameter space of a multi-head Convolutional Neural Network with Long Short Term Memory (CNN-LSTM) to search for the best architecture. In particular, our method requires minimum computational resources by making use of an early stopping policy and a history of the evaluated architectures. We dub the proposed method ENAS-PdM. To our knowledge, this is the first work where an EA-based NAS is used to optimize a CNN-LSTM architecture in the field of PdM. In our experiments, we use the well-established Commercial Modular Aero-Propulsion System Simulation (C-MAPSS) dataset from NASA. Compared to the current state-of-the-art, our method obtains better results in terms of two different metrics, RMSE and Score, when aggregating across all the C-MAPSS sub-datasets. Without aggregation, we achieve lower RMSE in 3 out of 4 sub-datasets. Our experimental results verify that the proposed method is a reliable tool for obtaining state-of-the-art RUL predictions and as such it can have a strong impact in several industrial applications, especially those with limited available computing power.},
   author = {Hyunho Mo and Leonardo Lucio Custode and Giovanni Iacca},
   doi = {10.1016/j.asoc.2021.107474},
   issn = {15684946},
   journal = {Applied Soft Computing},
   keywords = {C-MAPSS,Convolutional neural network,Evolutionary algorithm,Long short term memory,Remaining useful life},
   publisher = {Elsevier Ltd},
   title = {Evolutionary neural architecture search for remaining useful life prediction},
   volume = {108},
   year = {2021},
}
@article{Ahmad2012,
   abstract = {This paper presents an overview of two maintenance techniques widely discussed in the literature: time-based maintenance (TBM) and condition-based maintenance (CBM). The paper discusses how the TBM and CBM techniques work toward maintenance decision making. Recent research articles covering the application of each technique are reviewed. The paper then compares the challenges of implementing each technique from a practical point of view, focusing on the issues of required data determination and collection, data analysis/modelling, and decision making. The paper concludes with significant considerations for future research. Each of the techniques was found to have unique concepts/principles, procedures, and challenges for real industrial practise. It can be concluded that the application of the CBM technique is more realistic, and thus more worthwhile to apply, than the TBM one. However, further research on CBM must be carried out in order to make it more realistic for making maintenance decisions. The paper provides useful information regarding the application of the TBM and CBM techniques in maintenance decision making and explores the challenges in implementing each technique from a practical perspective.© 2012 Elsevier Ltd. All rights reserved.},
   author = {Rosmaini Ahmad and Shahrul Kamaruddin},
   doi = {10.1016/j.cie.2012.02.002},
   issn = {03608352},
   issue = {1},
   journal = {Computers and Industrial Engineering},
   keywords = {Condition-based maintenance,Industrial application,Maintenance decision making,Maintenance techniques,Preventive maintenance,Time-based maintenance},
   pages = {135-149},
   publisher = {Elsevier Ltd},
   title = {An overview of time-based and condition-based maintenance in industrial application},
   volume = {63},
   year = {2012},
}
@article{Hartman1970,
   abstract = {Data are presented for fatigue crack propagation of two afu~nium alloys 12024-T3 Alcfad-7075-I% clad) in different environments and for several loading frequencies. Correlation of the data was attempted by the stress-intensity factor by application of the equation for crack growth proposed by Forman. The result was that the influence of the stress ratio on the crack growth was predicted by the equation in agreement with the test results but that the effects of the environment and the load frequency could not be coped with by changes in the constants of the equation. There may be a threshold level of the stress-intensity factor. strongly dependent on the environment and the alloy. in order to make the crack grow.},
   author = {A. Hartman and J Schijve},
   issue = {4},
   journal = {Experimental Fluid Mechanics},
   pages = {615-631},
   title = {The effects of environment and load frequency on the crack propagation law for macro fatigue crack growth in aluminium alloys},
   volume = {1},
   year = {1970},
}
@article{Li2019b,
   abstract = {Remaining useful life (RUL) prediction has attracted more and more attention in recent years because of its significance in predictive maintenance. The degradation processes of systems from the same population are generally different from one another due to their various operational conditions and health states. This behavior is defined as unit-to-unit variability (UtUV), which brings difficulty to RUL prediction. To handle this problem, this paper develops a Wiener-process-model (WPM)-based method for RUL prediction with the consideration of the UtUV. In this method, an age- A nd state-dependent WPM is specially designed to describe the various degradation processes of different units. A unit maximum likelihood estimation (UMLE) algorithm is proposed to estimate the UtUV parameter according to the measurements of training units, without any restriction to the distribution pattern of the parameter. The UtUV parameter is further updated via particle filtering (PF) according to the measurements of the testing unit. In the particle updating process, a fuzzy resampling algorithm is developed to handle the sample impoverishment problem of PF. With the updated parameter, the RUL is predicted through a degradation process simulation algorithm. The effectiveness of the proposed method is verified through a simulation study and a turbofan engine degradation dataset.},
   author = {Naipeng Li and Yaguo Lei and Tao Yan and Ningbo Li and Tianyu Han},
   doi = {10.1109/TIE.2018.2838078},
   issn = {02780046},
   issue = {3},
   journal = {IEEE Transactions on Industrial Electronics},
   keywords = {Particle filtering (PF),Wiener process model (WPM),remaining useful life (RUL) prediction,unit maximum likelihood estimation (UMLE),unit-to-unit variability (UtUV)},
   pages = {2092-2101},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {A Wiener-Process-Model-Based Method for Remaining Useful Life Prediction Considering Unit-to-Unit Variability},
   volume = {66},
   year = {2019},
}
@article{Paris1963,
   abstract = {<p>The practice of attempting validation of crack-propagation laws (i.e., the laws of Head, Frost and Dugdale, McEvily and Illg, Liu, and Paris) with a small amount of data, such as a few single specimen test results, is questioned. It is shown that all the laws, though they are mutually contradictory, can be in agreement with the same small sample of data. It is suggested that agreement with a wide selection of data from many specimens and over many orders of magnitudes of crack-extension rates may be necessary to validate crack-propagation laws. For such a wide comparison of data a new simple empirical law is given which fits the broad trend of the data.</p>},
   author = {P. Paris and F. Erdogan},
   doi = {10.1115/1.3656900},
   issn = {0021-9223},
   issue = {4},
   journal = {Journal of Basic Engineering},
   pages = {528-533},
   title = {A Critical Analysis of Crack Propagation Laws},
   volume = {85},
   year = {1963},
}
@article{,
   author = {P.J. García Nieto and E. García-Gonzalo and F. Sánchez Lasheras and F.J. de Cos Juez},
   doi = {10.1016/j.ress.2015.02.001},
   issn = {09518320},
   journal = {Reliability Engineering and System Safety},
   pages = {219-231},
   title = {Hybrid PSO–SVM-based method for forecasting of the remaining useful life for aircraft engines and evaluation of its reliability},
   volume = {138},
   year = {2015},
}
@article{Yu2020,
   abstract = {Remaining useful life (RUL) estimation of a degrading system is the major prognostic activity in many industry applications. This paper presents an improved version of the similarity-based curve matching method for the remaining useful life estimation of a mechanical system, which is a companion paper of our previous work on RUL estimations using a bidirectional recurrent neural network (RNN) based autoencoder scheme. We propose a zero-centering rule to tackle the varying initial health across instances (systems) when using the similarity-based health index curve matching technique to identify the training instances that share a similar degradation pattern with the test instance whose RUL needs to be determined. However, this rule will also induce a significant prediction error, especially when the off-line training instances are abundant, or the true RULs of the on-line test instances are large. Thus, an ensemble approach that integrates the RUL estimations obtained from the similarity-based curve matching techniques, with and without the zero-centering rules, is introduced to increase the robustness and accuracy of proposed method for RUL estimations. We evaluate the prognostic performance of the ensemble algorithm and standalone algorithms on four publicly available turbofan engine degradation datasets. The results demonstrate that the proposed ensemble approach gives more robust and reliable RUL estimations compared to any independent algorithm used on all the studied datasets.},
   author = {Wennian Yu and II Yong Kim and Chris Mechefske},
   doi = {10.1016/j.ress.2020.106926},
   issn = {09518320},
   journal = {Reliability Engineering and System Safety},
   keywords = {Ensemble,Health index,Remaining useful life,Similarity-based interpolation},
   publisher = {Elsevier Ltd},
   title = {An improved similarity-based prognostic algorithm for RUL estimation using an RNN autoencoder scheme},
   volume = {199},
   year = {2020},
}
@article{Mo2021a,
   abstract = {Remaining Useful Life (RUL) estimation is a fundamental task in the prognostic and health management (PHM) of industrial equipment and systems. To this end, we propose a novel approach for RUL estimation in this paper, based on deep neural architecture due to its great success in sequence learning. Specifically, we take the Transformer encoder as the backbone of our model to capture short- and long-term dependencies in a time sequence. Compared with convolutional neural network based methods, there is no limitation from the kernel size for a complete receptive field of all time steps. While compared with recurrent neural network based methods, we develop our model based on dot-product self-attention, enabling it to fully exploit parallel computation. Moreover, we further propose a gated convolutional unit to facilitate the model’s ability of incorporating local contexts at each time step, for the attention mechanism used in the Transformer encoder makes the output high-level features insensitive to local contexts. We conduct experiments on the C-MAPSS datasets and show that, the performance of our model is superior or comparable to those of other existing methods. We also carry out ablation studies and demonstrate the necessity and effectiveness of each component used in the proposed model.},
   author = {Yu Mo and Qianhui Wu and Xiu Li and Biqing Huang},
   doi = {10.1007/s10845-021-01750-x},
   issn = {15728145},
   issue = {7},
   journal = {Journal of Intelligent Manufacturing},
   keywords = {Gated convolutional unit,Remaining useful life estimation,Transformer encoder,Turbofan engine},
   pages = {1997-2006},
   publisher = {Springer},
   title = {Remaining useful life estimation via transformer encoder enhanced by a gated convolutional unit},
   volume = {32},
   year = {2021},
}
@article{Chen2021,
   abstract = {For prognostics and health management of mechanical systems, a core task is to predict the machine remaining useful life (RUL). Currently, deep structures with automatic feature learning, such as long short-term memory (LSTM), have achieved great performances for the RUL prediction. However, the conventional LSTM network only uses the learned features at last time step for regression or classification, which is not efficient. Besides, some handcrafted features with domain knowledge may convey additional information for the prediction of RUL. It is thus highly motivated to integrate both those handcrafted features and automatically learned features for the RUL prediction. In this article, we propose an attention-based deep learning framework for machine's RUL prediction. The LSTM network is employed to learn sequential features from raw sensory data. Meanwhile, the proposed attention mechanism is able to learn the importance of features and time steps, and assign larger weights to more important ones. Moreover, a feature fusion framework is developed to combine the handcrafted features with automatically learned features to boost the performance of the RUL prediction. Extensive experiments have been conducted on two real datasets and experimental results demonstrate that our proposed approach outperforms the state-of-the-arts.},
   author = {Zhenghua Chen and Min Wu and Rui Zhao and Feri Guretno and Ruqiang Yan and Xiaoli Li},
   doi = {10.1109/TIE.2020.2972443},
   issn = {15579948},
   issue = {3},
   journal = {IEEE Transactions on Industrial Electronics},
   keywords = {Attention mechanism,feature fusion,handcrafted features,long short-term memory (LSTM),machine remaining useful life (RUL) prediction,prognostics and health management (PHM)},
   pages = {2521-2531},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Machine Remaining Useful Life Prediction via an Attention-Based Deep Learning Approach},
   volume = {68},
   year = {2021},
}
@article{Li2018b,
   abstract = {Traditionally, system prognostics and health management (PHM) depends on sufficient prior knowledge of critical components degradation process in order to predict the remaining useful life (RUL). However, the accurate physical or expert models are not available in most cases. This paper proposes a new data-driven approach for prognostics using deep convolution neural networks (DCNN). Time window approach is employed for sample preparation in order for better feature extraction by DCNN. Raw collected data with normalization are directly used as inputs to the proposed network, and no prior expertise on prognostics and signal processing is required, that facilitates the application of the proposed method. In order to show the effectiveness of the proposed approach, experiments on the popular C-MAPSS dataset for aero-engine unit prognostics are carried out. High prognostic accuracy on the RUL estimation is achieved. The superiority of the proposed method is demonstrated by comparisons with other popular approaches and the state-of-the-art results on the same dataset. The results of this study suggest that the proposed data-driven prognostic method offers a new and promising approach.},
   author = {Xiang Li and Qian Ding and Jian-Qiao Sun},
   journal = {Reliability Engineering and System Safety},
   keywords = {Convolution neural network,Deep learning,Prognostics and health management,Remaining useful life},
   pages = {1-11},
   title = {Remaining Useful Life Estimation in Prognostics Using Deep Convolution Neural Networks},
   volume = {172},
   url = {http://www.elsevier.com/open-access/userlicense/1.0/},
   year = {2017},
}
@inproceedings{Saxena2008,
   abstract = {This paper describes how damage propagation can be modeled within the modules of aircraft gas turbine engines. To that end, response surfaces of all sensors are generated via a thermo-dynamical simulation model for the engine as a function of variations of flow and efficiency of the modules of interest. An exponential rate of change for flow and efficiency loss was imposed for each data set, starting at a randomly chosen initial deterioration set point. The rate of change of the flow and efficiency denotes an otherwise unspecified fault with increasingly worsening effect. The rates of change of the faults were constrained to an upper threshold but were otherwise chosen randomly. Damage propagation was allowed to continue until a failure criterion was reached. A health index was defined as the minimum of several superimposed operational margins at any given time instant and the failure criterion is reached when health index reaches zero. Output of the model was the time series (cycles) of sensed measurements typically available from aircraft gas turbine engines. The data generated were used as challenge data for the Prognostics and Health Management (PHM) data competition atPHM'08.},
   author = {Abhinav Saxena and Kai Goebel and Don Simon and Neil Eklund},
   journal = {IEEE Conference on Prognostics and Health Management},
   keywords = {C-MAPSS,Index Terms-Damage modeling,Performance Evaluation,Prognostics,Turbofan engines},
   title = {Damage Propagation Modeling for Aircraft Engine Run-to-Failure Simulation},
   url = {http://ti.arc.nasa.gov/project/prognostic-data-repository},
   year = {2008},
}
@web_page{Giordano2020,
   author = {Danilo Giordano and Daniel Gagar},
   journal = {European Conference of the Prognostics and Health Management Society},
   title = {PHME 2020 Data Challenge},
   url = {http://phmeurope.org/2020/data-challenge-2020},
   year = {2020},
}
@inproceedings{Kuersat2020,
   abstract = {Maintenance costs of industrial systems often exceed the initial investment cost. Predictive maintenance, which analyzes the health of the system and suggests maintenance planning, is one of the strategies implemented to reduce maintenance costs. Health status and life estimation of the machinery are the most researched topics in this context. In this paper, we present our analysis for Fifth European Conference of the Prognostics and Health Management Society 2020 Data Challenge , which introduces an experimental filtration system for different experiment setups, and asks for remaining useful life predictions. We compared random forest, gradient boosting , and Gaussian process regression algorithms to predict the useful life of the experimental system. With the help of a new fault-based piecewise linear RUL assignment strategy, our gradient boosting based solution has been ranked 3 rd in the data challenge.},
   author = {Ince Kürsat and Engin Sirkeci and Yakup Genç},
   journal = {European Conference of the Prognostics and Health Management Society},
   title = {Remaining Useful Life Prediction for Experimental Filtration System: A Data Challenge},
   year = {2020},
}
@inproceedings{,
   abstract = {This paper describes the method used by the Uptime team for the estimation of the remaining useful life of a filter during the 2020 PHM Conference Data Challenge. The proposed method is a hybrid of two methods: (1) based on median lifetime of a filter for a particular contamination profile and (2) kernel regression for a sensor-based prediction after a certain threshold of differential pressure is reached. The threshold value was chosen based on visual assessment followed by grid search for fine tuning. Median lifetime of a filter for unseen contamination profiles was estimated using interpolation. Choosing the right interpolation method was a challenge as training data contained samples with only two values of contamination particle size. Interpolation was chosen based on other publicly available information about the relationship between contamination profile and filter lifetime. The results (ranked 1 st with the total penalty score of 49.67) showed that an observation made based on one dataset can be useful for solving similar problems in the case of limited data availability. This suggests that there is a potential for using transfer learning in PHM applications.},
   author = {Roman Łomowski and Szczepan Hummel},
   journal = {European Conference of the Prognostics and Health Management Society},
   title = {A Method to Estimate the Remaining Useful Life of a Filter Using a Hybrid Approach Based on Kernel Regression and Simple Statistics},
   year = {2020},
}
@inproceedings{Beirami2020,
   abstract = {This paper illustrates a data-driven approach adopted to address the PHME2020 Data Challenge competition. The aim of the challenge was to estimate the Remaining Useful Lifetime (RUL) of an experimental filtration device analyzing its clogging status by means of static (e.g. data sheets, fluid type, sensors) and dynamic (e.g. sensing data) information. We address the problem employing different state-of-the-art feature extraction, feature selection, and machine learning techniques. In this paper, we describe the approach followed to assess the problem and to generate robust and adaptable prediction models together with a corresponding performance assessment and robustness evaluation. The performance of the proposed solution is calculated in term of penalty score. The final penalty score 57.24 ranked 2nd in the above-mentioned data challenge competition.},
   author = {H Beirami and D Calzà and A Cimatti and M Islam and M Roveri and P Svaizer},
   journal = {European Conference of the Prognostics and Health Management Society},
   title = {A Data-driven Approach for RUL Prediction of an Experimental Filtration System},
   year = {2020},
}
@web_page{Saha2007,
   author = {B. Saha and K. Goebel},
   journal = {NASA Ames Prognostics Data Repository},
   title = {Battery Data Set},
   url = {http://ti.arc.nasa.gov/project/prognostic-data-repository},
   year = {2007},
}
@article{Bauer2020,
   abstract = {Machine learning (ML) techniques are rapidly evolving, both in academia and practice. However, enterprises show different maturity levels in successfully implementing ML techniques. Thus, we review the state of adoption of ML in enterprises. We find that ML technologies are being increasingly adopted in enterprises, but that small and medium-size enterprises (SME) are struggling with the introduction in comparison to larger enterprises. In order to identify enablers and success factors we conduct a qualitative empirical study with 18 companies in different industries. The results show that especially SME fail to apply ML technologies due to insufficient ML knowhow. However, partners and appropriate tools can compensate this lack of resources. We discuss approaches to bridge the gap for SME.},
   author = {Markus Bauer and Clemens van Dinther and Daniel Kiefer and van Dinther},
   journal = {AMCIS},
   keywords = {demand forecasting,machine learning,small and medium sized enterprises,success factors and enablers},
   title = {Machine Learning in SME: An Empirical Study on Enablers and Success Factors Success Factors},
   volume = {3},
   year = {2020},
}
@article{Christ2016,
   abstract = {The all-relevant problem of feature selection is the identification of all strongly and weakly relevant attributes. This problem is especially hard to solve for time series classification and regression in industrial applications such as predictive maintenance or production line optimization, for which each label or regression target is associated with several time series and meta-information simultaneously. Here, we are proposing an efficient, scalable feature extraction algorithm for time series, which filters the available features in an early stage of the machine learning pipeline with respect to their significance for the classification or regression task, while controlling the expected percentage of selected but irrelevant features. The proposed algorithm combines established feature extraction methods with a feature importance filter. It has a low computational complexity, allows to start on a problem with only limited domain knowledge available, can be trivially parallelized, is highly scalable and based on well studied non-parametric hypothesis tests. We benchmark our proposed algorithm on all binary classification problems of the UCR time series classification archive as well as time series from a production line optimization project and simulated stochastic processes with underlying qualitative change of dynamics.},
   author = {Maximilian Christ and Andreas W. Kempa-Liehr and Michael Feindt},
   journal = {arXiv: 1610.07717},
   title = {Distributed and parallel time series feature extraction for industrial big data applications},
   url = {http://arxiv.org/abs/1610.07717},
   year = {2016},
}
@generic{Yamashita2018,
   abstract = {Abstract: Convolutional neural network (CNN), a class of artificial neural networks that has become dominant in various computer vision tasks, is attracting interest across a variety of domains, including radiology. CNN is designed to automatically and adaptively learn spatial hierarchies of features through backpropagation by using multiple building blocks, such as convolution layers, pooling layers, and fully connected layers. This review article offers a perspective on the basic concepts of CNN and its application to various radiological tasks, and discusses its challenges and future directions in the field of radiology. Two challenges in applying CNN to radiological tasks, small dataset and overfitting, will also be covered in this article, as well as techniques to minimize them. Being familiar with the concepts and advantages, as well as limitations, of CNN is essential to leverage its potential in diagnostic radiology, with the goal of augmenting the performance of radiologists and improving patient care. Key Points: • Convolutional neural network is a class of deep learning methods which has become dominant in various computer vision tasks and is attracting interest across a variety of domains, including radiology. • Convolutional neural network is composed of multiple building blocks, such as convolution layers, pooling layers, and fully connected layers, and is designed to automatically and adaptively learn spatial hierarchies of features through a backpropagation algorithm. • Familiarity with the concepts and advantages, as well as limitations, of convolutional neural network is essential to leverage its potential to improve radiologist performance and, eventually, patient care.},
   author = {Rikiya Yamashita and Mizuho Nishio and Richard Kinh Gian Do and Kaori Togashi},
   doi = {10.1007/s13244-018-0639-9},
   issn = {18694101},
   issue = {4},
   journal = {Insights into Imaging},
   keywords = {Convolutional neural network,Deep learning,Machine learning,Medical imaging,Radiology},
   pages = {611-629},
   publisher = {Springer Verlag},
   title = {Convolutional neural networks: an overview and application in radiology},
   volume = {9},
   year = {2018},
}
@article{Hochreiter1997,
   author = {Sepp Hochreiter and Jürger Schmidhuber},
   issue = {8},
   journal = {Neural Computation},
   pages = {1735-1780},
   title = {Long Short-Term Memory},
   volume = {9},
   year = {1997},
}
@article{Cho2014,
   abstract = {Neural machine translation is a relatively new approach to statistical machine translation based purely on neural networks. The neural machine translation models often consist of an encoder and a decoder. The encoder extracts a fixed-length representation from a variable-length input sentence, and the decoder generates a correct translation from this representation. In this paper, we focus on analyzing the properties of the neural machine translation using two models; RNN Encoder--Decoder and a newly proposed gated recursive convolutional neural network. We show that the neural machine translation performs relatively well on short sentences without unknown words, but its performance degrades rapidly as the length of the sentence and the number of unknown words increase. Furthermore, we find that the proposed gated recursive convolutional network learns a grammatical structure of a sentence automatically.},
   author = {Kyunghyun Cho and Bart van Merrienboer and Dzmitry Bahdanau and Yoshua Bengio},
   journal = {arXiv: 1409.1259},
   title = {On the Properties of Neural Machine Translation: Encoder-Decoder Approaches},
   url = {http://arxiv.org/abs/1409.1259},
   year = {2014},
}
@inproceedings{Lea2016,
   abstract = {The dominant paradigm for video-based action segmentation is composed of two steps: first, for each frame, compute low-level features using Dense Trajectories or a Convolutional Neural Network that encode spatiotemporal information locally, and second, input these features into a classifier that captures high-level temporal relationships, such as a Recurrent Neural Network (RNN). While often effective, this decoupling requires specifying two separate models, each with their own complexities, and prevents capturing more nuanced long-range spatiotemporal relationships. We propose a unified approach, as demonstrated by our Temporal Convolutional Network (TCN), that hierarchically captures relationships at low-, intermediate-, and high-level time-scales. Our model achieves superior or competitive performance using video or sensor data on three public action segmentation datasets and can be trained in a fraction of the time it takes to train an RNN.},
   author = {Colin Lea and Rene Vidal and Austin Reiter and Gregory D. Hager},
   journal = {ECCV},
   title = {Temporal Convolutional Networks: A Unified Approach to Action Segmentation},
   url = {http://arxiv.org/abs/1608.08242},
   year = {2016},
}
@report{Ardic2011,
   author = {Oya Pinar Ardic and Nataliya Mylenko and Valentina Saltane},
   title = {Small and Medium Enterprises: A Cross-Country Analysis with a New Data},
   url = {http://www.cgap.org/financialindicators},
   year = {2011},
}
@inproceedings{Nectoux2012,
   abstract = {This paper deals with the presentation of an experimental platform called PRONOSTIA, which enables testing, verifying and validating methods related to bearing health assessment, diagnostic and prognostic. The choice of bearings is justified by the fact that most of failures of rotating machines are related to these components. Therefore, bearings can be considered as critical as their failure significantly decreases availability and security of machines. The main objective of PRONOSTIA is to provide real data related to accelerated degradation of bearings performed under constant and/or variable operating conditions, which are online controlled. The operating conditions are characterized by two sensors: a rotating speed sensor and a force sensor. In PRONOSTIA platform, the bearing's health monitoring is ensured by gathering online two types of signals: temperature and vibration (horizontal and vertical accelerometers). Furthermore, the data are recorded with a specific sampling frequency which allows catching all the frequency spectrum of the bearing during its whole degradation. Finally, the monitoring data provided by the sensors can be used for further processing in order to extract relevant features and continuously assess the health condition of the bearing. During the PHM conference, a "IEEE PHM 2012 Prognostic Challenge" is organized. For this purpose, a web link to the degradation data is provided to the competitors to allow them testing and verifying their prognostic methods. The results of each method can then be evaluated regarding its capability to accurately estimate the remaining useful life of the tested bearings.},
   author = {Patrick Nectoux and Rafael Gouriveau and Kamal Medjaher and Emmanuel Ramasso and Brigitte Chebel-Morello and Noureddine Zerhouni and Christophe Varnier},
   journal = {IEEE Conference on Prognostics and Health Management},
   keywords = {()},
   pages = {1-8},
   title = {PRONOSTIA: An Experimental Platform for Bearings Accelerated Degradation Tests},
   url = {https://hal.archives-ouvertes.fr/hal-00719503},
   year = {2012},
}
@article{Nieto2015,
   abstract = {The present paper describes a hybrid PSO-SVM-based model for the prediction of the remaining useful life of aircraft engines. The proposed hybrid model combines support vector machines (SVMs), which have been successfully adopted for regression problems, with the particle swarm optimization (PSO) technique. This optimization technique involves kernel parameter setting in the SVM training procedure, which significantly influences the regression accuracy. However, its use in reliability applications has not been yet widely explored. Bearing this in mind, remaining useful life values have been predicted here by using the hybrid PSO-SVM-based model from the remaining measured parameters (input variables) for aircraft engines with success. A coefficient of determination equal to 0.9034 was obtained when this hybrid PSO-RBF-SVM-based model was applied to experimental data. The agreement of this model with experimental data confirmed its good performance. One of the main advantages of this predictive model is that it does not require information about the previous operation states of the engine. Finally, the main conclusions of this study are exposed.},
   author = {P. J. García Nieto and E. García-Gonzalo and F. Sánchez Lasheras and F. J. De Cos Juez},
   doi = {10.1016/j.ress.2015.02.001},
   issn = {09518320},
   journal = {Reliability Engineering and System Safety},
   keywords = {Aircraft engine,Particle swarm optimization (PSO),Remaining useful life and reliability prediction,Support vector machines (SVMs)},
   pages = {219-231},
   publisher = {Elsevier Ltd},
   title = {Hybrid PSO-SVM-based method for forecasting of the remaining useful life for aircraft engines and evaluation of its reliability},
   volume = {138},
   year = {2015},
}
@book_section{Nielsen1993,
   author = {Jakob Nielsen},
   journal = {Usability Engineering},
   publisher = {Morgan Kaufmann},
   title = {Usability Heuristics},
   year = {1993},
}
@article{Ali2017,
   abstract = {Objective Manual evaluation of machine learning algorithms and selection of a suitable classifier from the list of available candidate classifiers, is highly time consuming and challenging task. If the selection is not carefully and accurately done, the resulting classification model will not be able to produce the expected performance results. In this study, we present an accurate multi-criteria decision making methodology (AMD) which empirically evaluates and ranks classifiers’ and allow end users or experts to choose the top ranked classifier for their applications to learn and build classification models for them. Methods and material Existing classifiers performance analysis and recommendation methodologies lack (a) appropriate method for suitable evaluation criteria selection, (b) relative consistent weighting mechanism, (c) fitness assessment of the classifiers’ performances, and (d) satisfaction of various constraints during the analysis process. To assist machine learning practitioners in the selection of suitable classifier(s), AMD methodology is proposed that presents an expert group-based criteria selection method, relative consistent weighting scheme, a new ranking method, called optimum performance ranking criteria, based on multiple evaluation metrics, statistical significance and fitness assessment functions, and implicit and explicit constraints satisfaction at the time of analysis. For ranking the classifiers performance, the proposed ranking method integrates Wgt.Avg.F-score, CPUTimeTesting, CPUTimeTraining, and Consistency measures using the technique for order performance by similarity to ideal solution (TOPSIS). The final relative closeness score produced by TOPSIS, is ranked and the practitioners select the best performance (top-ranked) classifier for their problems in-hand. Findings Based on the extensive experiments performed on 15 publically available UCI and OpenML datasets using 35 classification algorithms from heterogeneous families of classifiers, an average Spearman's rank correlation coefficient of 0.98 is observed. Similarly, the AMD method has showed improved performance of 0.98 average Spearman's rank correlation coefficient as compared to 0.83 and 0.045 correlation coefficient of the state-of-the-art ranking methods, performance of algorithms (PAlg) and adjusted ratio of ratio (ARR). Conclusion and implication The evaluation, empirical analysis of results and comparison with state-of-the-art methods demonstrate the feasibility of AMD methodology, especially the selection and weighting of right evaluation criteria, accurate ranking and selection of optimum performance classifier(s) for the user's application's data in hand. AMD reduces expert's time and efforts and improves system performance by designing suitable classifier recommended by AMD methodology.},
   author = {Rahman Ali and Sungyoung Lee and Tae Choong Chung},
   doi = {10.1016/j.eswa.2016.11.034},
   issn = {09574174},
   journal = {Expert Systems with Applications},
   keywords = {Algorithm recommendation,Algorithm selection,Classification algorithms,Classifiers recommendation,Multi-criteria decision making,Ranking classifiers,TOPSIS},
   pages = {257-278},
   publisher = {Elsevier Ltd},
   title = {Accurate multi-criteria decision making methodology for recommending machine learning algorithm},
   volume = {71},
   year = {2017},
}
@article{Lindauer2022,
   abstract = {Algorithm parameters, in particular hyperparameters of machine learning algorithms, can substantially impact their performance. To support users in determining well-performing hyperparameter configurations for their algorithms, datasets and applications at hand, SMAC3 offers a robust and flexible framework for Bayesian Optimization, which can improve performance within a few evaluations. It offers several facades and pre-sets for typical use cases, such as optimizing hyperparameters, solving low dimensional continuous (artificial) global optimization problems and configuring algorithms to perform well across multiple problem instances. The SMAC3 package is available under a permissive BSD-license at https://github.com/automl/SMAC3.},
   author = {Marius Lindauer and Katharina Eggensperger and Matthias Feurer and André Biedenkapp and Difan Deng and Carolin Benjamins and Tim Ruhkopf and René Sass and Frank Hutter},
   journal = {Journal of Machine Learning Research},
   keywords = {Algorithm Configuration,Automated Machine Learning,Bayesian Optimization,Hyperparameter Optimization,Multi-Fidelity Opti-mization},
   pages = {1-9},
   title = {{SMAC3}: A Versatile Bayesian Optimization Package for Hyperparameter Optimization},
   volume = {23},
   year = {2022},
}
@inproceedings{Paszke2019,
   abstract = {Deep learning frameworks have often focused on either usability or speed, but not both. PyTorch is a machine learning library that shows that these two goals are in fact compatible: it provides an imperative and Pythonic programming style that supports code as a model, makes debugging easy and is consistent with other popular scientific computing libraries, while remaining efficient and supporting hardware accelerators such as GPUs. In this paper, we detail the principles that drove the implementation of PyTorch and how they are reflected in its architecture. We emphasize that every aspect of PyTorch is a regular Python program under the full control of its user. We also explain how the careful and pragmatic implementation of the key components of its runtime enables them to work together to achieve compelling performance. We demonstrate the efficiency of individual subsystems, as well as the overall speed of PyTorch on several common benchmarks.},
   author = {Adam Paszke and Sam Gross and Francisco Massa and Adam Lerer and James Bradbury Google and Gregory Chanan and Trevor Killeen and Zeming Lin and Natalia Gimelshein and Luca Antiga and Alban Desmaison and Andreas Köpf Xamla and Edward Yang and Zach Devito and Martin Raison Nabla and Alykhan Tejani and Sasank Chilamkurthy and Qure Ai and Benoit Steiner and Lu Fang Facebook and Junjie Bai Facebook and Soumith Chintala},
   booktitle = {Advances in Neural Information Processing Systems 32},
   pages = {8024-8035},
   title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
   year = {2019},
}
@article{Holm1979,
   abstract = {JSTOR is a not-for-profit service that helps scholars, researchers, and students discover, use, and build upon a wide range of content in a trusted digital archive. We use information technology and tools to increase productivity and facilitate new forms of scholarship. For more information about JSTOR, please contact support@jstor.org.. Wiley and Board of the Foundation of the Scandinavian Journal of Statistics are collaborating with JSTOR to digitize, preserve and extend access to Scandinavian Journal of Statistics. ABSTRACT. This paper presents a simple and widely applicable multiple test procedure of the sequentially rejective type, i.e. hypotheses are rejected one at a tine until no further rejections can be done. It is shown that the test has a prescribed level of significance protection against error of the first kind for any combination of true hypotheses. The power properties of the test and a number of possible applications are also discussed.},
   author = {Sture Holm},
   isbn = {201308:15:53},
   issue = {2},
   journal = {Source: Scandinavian Journal of Statistics},
   keywords = {multiple test,simultaneous test},
   pages = {65-70},
   title = {A Simple Sequentially Rejective Multiple Test Procedure},
   volume = {6},
   year = {1979},
}
@inproceedings{Kancharla2022,
   abstract = {More and more businesses have taken to adopting Machine Learning (ML) and Deep Learning methods for solving problems in the application domain. One such area is Anomaly detection. While research in recent years has yielded better accuracies, the main hurdle for businesses remains managing the high cost of resources required for their implementation. Traditional ML/Deep Learning techniques require expert knowledge, and thus presently rely on human efficiency. Automated machine learning (AutoML) has emerged as a solution to the above scenario. In this paper, we evaluate the performances of traditional anomaly detection techniques used in time-series forecasting, namely, statistical and deep learning models, and compare their results in terms of efficiency and performance with AutoML. We use H2O driverless AI (H2o.ai automl documentation, http://docs.h2o.ai/h2o/latest-stable/h2o-docs/automl.html, accessed: 2020-06-10) as our platform for experiments on AutoML. All the experiments are performed on the Numenta Anomaly Benchmark's streaming time-series dataset (Lavin A and Subutai A in 2015 IEEE 14th international conference on machine learning and applications (ICMLA), pp 38–44).},
   author = {Ajanta Kancharla and N. Raghu Kishore},
   isbn = {9789811623769},
   issn = {23673389},
   booktitle = {Lecture Notes in Networks and Systems},
   keywords = {ARIMA,Anomaly detection,Convolutional LSTM,H2O AutoML,LSTM autoencoders,Real-time computing,Recurrent neural network,Time series,Univariate},
   pages = {937-947},
   publisher = {Springer Science and Business Media Deutschland GmbH},
   title = {Applicability of AutoML to Modeling of Time-Series Data},
   volume = {235},
   year = {2022},
}
@inproceedings{He2018,
   abstract = {Model compression is an effective technique to efficiently deploy neural network models on mobile devices which have limited computation resources and tight power budgets. Conventional model compression techniques rely on hand-crafted features and require domain experts to explore the large design space trading off among model size, speed, and accuracy, which is usually sub-optimal and time-consuming. In this paper, we propose AutoML for Model Compression (AMC) which leverages reinforcement learning to efficiently sample the design space and can improve the model compression quality. We achieved state-of-the-art model compression results in a fully automated way without any human efforts. Under 4× FLOPs reduction, we achieved 2.7% better accuracy than the hand-crafted model compression method for VGG-16 on ImageNet. We applied this automated, push-the-button compression pipeline to MobileNet-V1 and achieved a speedup of 1.53× on the GPU (Titan Xp) and 1.95× on an Android phone (Google Pixel 1), with negligible loss of accuracy.},
   author = {Yihui He and Ji Lin and Zhijian Liu and Hanrui Wang and Li-Jia Li and Song Han},
   journal = {Proceedings of the European Conference on Computer Vision (ECCV)},
   keywords = {AutoML ·,Mobile vision,Model compression · CNN acceleration ·,Reinforcement learning ·},
   pages = {784-800},
   title = {AMC: AutoML for Model Compression and Acceleration on Mobile Devices},
   year = {2018},
}
@inproceedings{VanRijn2018,
   abstract = {With the advent of automated machine learning, automated hyperparameter optimization methods are by now routinely used in data mining. However, this progress is not yet matched by equal progress on automatic analyses that yield information beyond performance-optimizing hyperparameter settings. In this work, we aim to answer the following two questions: Given an algorithm, what are generally its most important hyperparameters, and what are typically good values for these? We present methodology and a framework to answer these questions based on meta-learning across many datasets. We apply this methodology using the experimental meta-data available on OpenML to determine the most important hyperparameters of support vector machines, random forests and Adaboost, and to infer priors for all their hyperparameters. The results, obtained fully automatically, provide a quantitative basis to focus efforts in both manual algorithm design and in automated hyperparameter optimization. The conducted experiments confirm that the hyperparameters selected by the proposed method are indeed the most important ones and that the obtained priors also lead to statistically significant improvements in hyperparameter optimization.},
   author = {Jan N. Van Rijn and Frank Hutter},
   doi = {10.1145/3219819.3220058},
   isbn = {9781450355520},
   journal = {Proceedings of the ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
   keywords = {Hyperparameter Importance,Hyperparameter Optimization,Meta-learning},
   pages = {2367-2376},
   publisher = {Association for Computing Machinery},
   title = {Hyperparameter importance across datasets},
   year = {2018},
}
@inproceedings{Moosbauer2021,
   abstract = {Automated hyperparameter optimization (HPO) can support practitioners to obtain peak performance in machine learning models. However, there is often a lack of valuable insights into the effects of different hyperparameters on the final model performance. This lack of explainability makes it difficult to trust and understand the automated HPO process and its results. We suggest using interpretable machine learning (IML) to gain insights from the experimental data obtained during HPO with Bayesian optimization (BO). BO tends to focus on promising regions with potential high-performance configurations and thus induces a sampling bias. Hence, many IML techniques, such as the partial dependence plot (PDP), carry the risk of generating biased interpretations. By leveraging the posterior uncertainty of the BO surrogate model, we introduce a variant of the PDP with estimated confidence bands. We propose to partition the hyperparameter space to obtain more confident and reliable PDPs in relevant sub-regions. In an experimental study, we provide quantitative evidence for the increased quality of the PDPs within sub-regions.},
   author = {Julia Moosbauer and Julia Herbinger and Giuseppe Casalicchio and Marius Lindauer and Bernd Bischl},
   journal = {Advances in Neural Information Processing Systems },
   pages = {2280-2291},
   title = {Explaining Hyperparameter Optimization via Partial Dependence Plots},
   year = {2021},
}
@report{Bouthillier2020,
   abstract = {How do machine-learning researchers run their empirical validation? In the context of a push for improved reproducibility and benchmarking, this question is important to develop new tools for model comparison. This document summarizes a simple survey about experimental procedures, sent to authors of published papers at two leading conferences, NeurIPS 2019 and ICLR 2020. It gives a simple picture of how hyper-parameters are set, how many baselines and datasets are included, or how seeds are used.},
   author = {Xavier Bouthillier and Canada Gaël Varoquaux},
   title = {Survey of machine-learning experimental methods at NeurIPS2019 and ICLR2020},
   year = {2020},
}
@inproceedings{Halvari2021,
   abstract = {Sensor data collection in IoT networks is sensitive to malfunction of sensors and communications. Hence, it is important that models using the data work in a reasonable way even when there are some, potentially temporary, problems. In this paper, we investigate the robustness of AutoML systems for time series forecasting in sensor networks, using temperature data as example. We experiment with different AutoML systems and study how the resulting models tolerate faults in their input data. The analyzed AutoML systems are Microsoft's Azure AutoML, Intel's Analytics Zoo AutoML, and Facebook's Prophet. As a result, we rank AutoML systems based on their performance with respect to data faults and their severity. In addition, we show how the AutoML generated models differ given the data fault type.},
   author = {Tuomas Halvari and Jukka K. Nurminen and Tommi Mikkonen},
   doi = {10.23919/IFIPNetworking52078.2021.9472199},
   isbn = {9783903176393},
   journal = {IFIP Networking Conference},
   keywords = {AutoML,forecasting,robustness,time series},
   pages = {2021-2023},
   publisher = {IFIP},
   title = {Robustness of AutoML for Time Series Forecasting in Sensor Networks},
   year = {2021},
}
@article{Sergio2016,
   abstract = {Time series forecasting is an important research field in machine learning. Since the literature shows several techniques for the solution of this problem, combining outputs of different models is a simple and robust strategy. However, even when using combiners, the experimenter may face the following dilemma: which technique should one use to combine the individual predictors? Inspired by classification and pattern recognition algorithms, this work presents a dynamic selection method of forecast combiners. In the dynamic selection, each test pattern is submitted to a certain combiner according to a nearest neighbor rule. The proposed method was used to forecast eight time series with chaotic behavior in short and long term. In general, the dynamic selection presented satisfactory results for all datasets.},
   author = {Anderson T. Sergio and Tiago P.F. de Lima and Teresa B. Ludermir},
   journal = {Neurocomputing},
   keywords = {Chaotic time series,Dynamic selection,Time series forecasting,Time series forecasting ensemble},
   pages = {37-50},
   publisher = {Elsevier},
   title = {Dynamic selection of forecast combiners},
   volume = {218},
   year = {2016},
}
@inproceedings{Stuhler2023,
   abstract = {Price forecasting for used construction equipment is a challenging task due to spatial and temporal price fluctuations. It is thus of high interest to automate the forecasting process based on current market data. Even though applying machine learning (ML) to these data represents a promising approach to predict the residual value of certain tools, it is hard to implement for small and medium-sized enterprises due to their insufficient ML expertise. To this end, we demonstrate the possibility of substituting manually created ML pipelines with automated machine learning (AutoML) solutions, which automatically generate the underlying pipelines. We combine AutoML methods with the domain knowledge of the companies. Based on the CRISP-DM process, we split the manual ML pipeline into a machine learning and non-machine learning part. To take all complex industrial requirements into account and to demonstrate the applicability of our new approach, we designed a novel metric named method evaluation score, which incorporates the most important technical and non-technical metrics for quality and usability. Based on this metric, we show in a case study for the industrial use case of price forecasting, that domain knowledge combined with AutoML can weaken the dependence on ML experts for innovative small and medium-sized enterprises which are interested in conducting such solutions.},
   author = {Horst Stühler and Marc-André Zöller and Dennis Klau and Alexandre Beiderwellen-Bedrikow and Christian Tutschku},
   journal = {Proceedings of the 12th International Conference on Data Science, Technology and Applications},
   title = {Benchmarking Automated Machine Learning Methods for Price Forecasting Applications},
   url = {http://arxiv.org/abs/2304.14735},
   year = {2023},
}
@inproceedings{Zoller2023,
   abstract = {Being able to predict the remaining useful life (RUL) of an engineering system is an important task in prognostics and health management. Recently, data-driven approaches to RUL predictions are becoming prevalent over model-based approaches since no underlying physical knowledge of the engineering system is required. Yet, this just replaces required expertise of the underlying physics with machine learning (ML) expertise, which is often also not available. Automated machine learning (AutoML) promises to build end-to-end ML pipelines automatically enabling domain experts without ML expertise to create their own models. This paper introduces AUTORUL, an AutoML-driven end-to-end approach for automatic RUL predictions. AUTORUL combines fine-tuned standard regression methods to an ensemble with high predictive power. By evaluating the proposed method on eight real-world and synthetic datasets against state-of-the-art hand-crafted models, we show that AutoML provides a viable alternative to hand-crafted data-driven RUL predictions. Consequently , creating RUL predictions can be made more accessible for domain experts using AutoML by eliminating ML expertise from data-driven model construction.},
   author = {Marc-André Zöller and Fabian Mauthe and Peter Zeiler and Marius Lindauer and Marco F Huber},
   keywords = {AutoML,Automated Machine Learning,Index Terms-Remaining Useful Life,ML,PHM,RUL,data-driven},
   title = {Automated Machine Learning for Remaining Useful Life Predictions},
   booktitle = {IEEE SMC},
   year = {2023},
}
@article{Hyndman2008,
   abstract = {Automatic forecasts of large numbers of univariate time series are often needed in business and other contexts. We describe two automatic forecasting algorithms that have been implemented in the forecast package for R. The first is based on innovations state space models that underly exponential smoothing methods. The second is a step-wise algorithm for forecasting with ARIMA models. The algorithms are applicable to both seasonal and non-seasonal data, and are compared and illustrated using four real time series. We also briefly describe some of the other functionality available in the forecast package.},
   author = {Rob J. Hyndman and Yeasmin Khandakar},
   journal = {Journal of Statistical Software},
   keywords = {ARIMA models,R,automatic forecasting,exponential smoothing,prediction inter-vals,state space models,time series},
   pages = {1-22},
   title = {Automatic Time Series Forecasting: The forecast Package for R},
   volume = {27},
   year = {2008},
}
@book{Box2015,
   author = {George E.P. Box and Gwilym M. Jenkins and Gregory C. Reinsel and Greta M. Ljung},
   edition = {5},
   publisher = {Wiley},
   title = {Time Series Analysis: Forecasting and Control},
   year = {2015},
}
@book{Hyndman2008b,
   author = {Rob J. Hyndman and Anne B. Koehler and J. Keith Ord and Ralph D. Snyder},
   publisher = {Springer Science and Business Media},
   title = {Forecasting with Exponential Smoothing: The State Space Approach},
   year = {2008},
}
@article{Ahmed2010,
   abstract = {In this work we present a large scale comparison study for the major machine learning models for time series forecasting. Specifically, we apply the models on the monthly M3 time series competition data (around a thousand time series). There have been very few, if any, large scale comparison studies for machine learning models for the regression or the time series forecasting problems, so we hope this study would fill this gap. The models considered are multilayer per-ceptron, Bayesian neural networks, radial basis functions, generalized regression neural networks (also called kernel regression), K-nearest neighbor regression, CART regression trees, support vector regression, and Gaussian processes. The study reveals significant differences between the different methods. The best two methods turned out to be the multilayer perceptron and the Gaussian process regression. In addition to model comparisons, we have tested different preprocessing methods and have shown that they have different impacts on the performance.},
   author = {Nesreen K. Ahmed and Amir F. Atiya and Neamat El Gayar and Hisham El-Shishiny},
   issue = {5},
   journal = {Econometric Reviews},
   keywords = {()},
   pages = {594-621},
   title = {An Empirical Comparison of Machine Learning Models for Time Series Forecasting},
   volume = {29},
   year = {2010},
}
@book_section{Akaike1998,
   author = {Hirotogu Akaike},
   pages = {199-213},
   title = {Information Theory and an Extension of the Maximum Likelihood Principle},
   year = {1998},
}
@article{Hyndman2006,
   abstract = {We discuss and compare measures of accuracy of univariate time series forecasts. The methods used in the M-competition and the M3-competition, and many of the measures recommended by previous authors on this topic, are found to be degenerate in commonly occurring situations. Instead, we propose that the mean absolute scaled error become the standard measure for comparing forecast accuracy across multiple time series.},
   author = {Rob J Hyndman and Anne B Koehler},
   issue = {4},
   journal = {International Journal of Forecasting},
   keywords = {M-competition,forecast accuracy,forecast error measures,forecast evaluation,mean absolute scaled error 2},
   pages = {679-688},
   title = {Another look at measures of forecast accuracy},
   volume = {22},
   year = {2006},
}
@inproceedings{Ji2005,
   abstract = {This paper presents a comparison between direct and recursive prediction strategies. In order to perform the input selection, an approach based on mutual information is used. The mutual information is computed between all the possible input sets and the outputs. Least Squares Support Vector Machines are used as non-linear models to avoid local minima problems. Results are illustrated on the Poland electricity load benchmark and they show the superiority of the direct prediction strategy.},
   author = {Yongnan Ji and Jin Hao and Nima Reyhani and Amaury Lendasse},
   booktitle = {Computational Intelligence and Bioinspired Systems},
   keywords = {Direct Prediction,Least Squares Support Vector Machines and Prediction Strategy,Mutual Information,Re-cursive Prediction,Time Series Prediction},
   pages = {1010-1017},
   title = {Direct and Recursive Prediction of Time Series Using Mutual Information Selection},
   volume = {3512},
   year = {2005},
}
@article{Cortes1995,
   author = {Corinna Cortes and Vladimir Vapnik},
   issn = {0885-6125},
   issue = {3},
   journal = {Machine Learning},
   pages = {273-297},
   title = {Support-vector networks},
   volume = {20},
   year = {1995},
}
@book{Hyndman2021,
   author = {Rob J. Hyndman and Georg Athanasopoulos},
   publisher = {OTexts},
   title = {Forecasting: Principles and Practice},
   year = {2021},
}
@article{Cho2014a,
   abstract = {In this paper, we propose a novel neural network model called RNN Encoder-Decoder that consists of two recurrent neural networks (RNN). One RNN encodes a sequence of symbols into a fixed-length vector representation, and the other decodes the representation into another sequence of symbols. The encoder and decoder of the proposed model are jointly trained to maximize the conditional probability of a target sequence given a source sequence. The performance of a statistical machine translation system is empirically found to improve by using the conditional probabilities of phrase pairs computed by the RNN Encoder-Decoder as an additional feature in the existing log-linear model. Qualitatively, we show that the proposed model learns a semantically and syntactically meaningful representation of linguistic phrases.},
   author = {Kyunghyun Cho and Bart van Merrienboer and Caglar Gulcehre and Dzmitry Bahdanau and Fethi Bougares and Holger Schwenk and Yoshua Bengio},
   journal = {arXiv:1406.1078},
   title = {Learning Phrase Representations using RNN Encoder-Decoder for Statistical Machine Translation},
   year = {2014},
}
@article{Zhang1998,
   abstract = {Interest in using artificial neural networks (ANNs) for forecasting has led to a tremendous surge in research activities in the past decade. While ANNs provide a great deal of promise, they also embody much uncertainty. Researchers to date are still not certain about the effect of key factors on forecasting performance of ANNs. This paper presents a state-of-the-art survey of ANN applications in forecasting. Our purpose is to provide (1) a synthesis of published research in this area, (2) insights on ANN modeling issues, and (3) the future research directions.},
   author = {Guoqiang Zhang and B Eddy Patuwo and Michael Y Hu},
   journal = {International Journal of Forecasting},
   keywords = {Forecasting,Neural networks},
   pages = {35-62},
   title = {Forecasting with artificial neural networks: The state of the art},
   volume = {14},
   year = {1998},
}
@inproceedings{Yamak2020,
   abstract = {A critical area of machine learning is Time Series forecasting, as various forecasting problems contain a time component. A series of observations taken chronologically in time is known as a Time Series. In this research, however, we aim to compare three different machine learning models in making a time series forecast. We are going to use the Bitcoin's price dataset as our time series data set and make predictions accordingly. The results show that the ARIMA model gave better results than the deep learning-based regression models. ARIMA gives the best results at 2.76% and 302.53 for MAPE and RMSE respectively. The Gated Recurrent Unit (GRU) however performed better than the Long Short-term Memory (LSTM), with 3.97% and 381.34 of MAPE and RMSE respectively.},
   author = {Peter T. Yamak and Li Yujian and Pius K. Gadosey},
   isbn = {9781450372619},
   booktitle = {ACAI},
   keywords = {ARIMA,Bitcoin,GRU,LSTM,Time Series},
   pages = {49-55},
   title = {A comparison between ARIMA, LSTM, and GRU for time series forecasting},
   year = {2020},
}
@article{Bontempi2013,
   author = {Gianluca Bontempi and Souhaib Ben Taieb and Yann Aël Le Borgne},
   isbn = {9783642363177},
   issn = {18651348},
   issue = {January},
   journal = {LNBIP},
   pages = {62-77},
   title = {Machine Learning Strategies for Time Series Forecasting},
   volume = {138},
   year = {2013},
}
@web_page{Prophet2017,
   author = {Meta},
   title = {Prophet: Automatic Forecasting Procedure},
   year = {2017},
}
@misc{Catlin2020,
   author = {Colin Catlin},
   title = {AutoTS},
   year = {2020},
   howpublished = {\url{https://github.com/winedarksea/AutoTS}}
}
@misc{Zheng2022,
   author = {Xiaojing Zhang and Haifeng Wu and Jian Yang},
   title = {HyperTS: A Full-Pipeline Automated Time Series Analysis Toolkit},
   howpublished = {\url{https://github.com/DataCanvasIO/HyperTS}},
   year = {2022},
}
@article{Maciag2021,
   abstract = {Unsupervised anomaly discovery in stream data is a research topic with many practical applications. However, in many cases, it is not easy to collect enough training data with labeled anomalies for supervised learning of an anomaly detector in order to deploy it later for identification of real anomalies in streaming data. It is thus important to desigFn anomalies detectors that can correctly detect anomalies without access to labeled training data. Our idea is to adapt the Online evolving Spiking Neural Network (OeSNN) classifier to the anomaly detection task. As a result, we offer an Online evolving Spiking Neural Network for Unsupervised Anomaly Detection algorithm (OeSNN-UAD), which, unlike OeSNN, works in an unsupervised way and does not separate output neurons into disjoint decision classes. OeSNN-UAD uses our proposed new two-step anomaly detection method. Also, we derive new theoretical properties of neuronal model and input layer encoding of OeSNN, which enable more effective and efficient detection of anomalies in our OeSNN-UAD approach. The proposed OeSNN-UAD detector was experimentally compared with state-of-the-art unsupervised and semi-supervised detectors of anomalies in stream data from the Numenta Anomaly Benchmark and Yahoo Anomaly Datasets repositories. Our approach outperforms the other solutions provided in the literature in the case of data streams from the Numenta Anomaly Benchmark repository. Also, in the case of real data files of the Yahoo Anomaly Benchmark repository, OeSNN-UAD outperforms other selected algorithms, whereas in the case of Yahoo Anomaly Benchmark synthetic data files, it provides competitive results to the results recently reported in the literature.},
   author = {Piotr S. Maciag and Marzena Kryszkiewicz and Robert Bembenik and Jesus L. Lobo and Javier Del Ser},
   journal = {Neural Networks},
   pages = {118-139},
   title = {Unsupervised Anomaly Detection in Stream Data with Online Evolving Spiking Neural Networks},
   volume = {139},
   year = {2021},
}
@misc{Carme2023,
   author = {Antoine Carme},
   title = {Time Series Datasets},
   howpublished = {\url{https://github.com/antoinecarme/TimeSeriesData}},
   year = {2023},
}
@misc{Mulla2018,
   author = {Rob Mulla},
   title = {Time Series Datasets},
   howpublished = {\url{https://www.kaggle.com/datasets/robikscube/hourly-energy-consumption}},
   year = {2018},
}
@article{Feurer2022,
   author = {Matthias Feurer and Katharina Eggensperger and Stefan Falkner and Marius Lindauer and Frank Hutter},
   journal = {JMLR},
   pages = {11936-11996},
   title = {Auto-Sklearn 2.0: Hands-free AutoML via Meta-Learning},
   volume = {23},
   year = {2022},
}
@article{Vintsyuk1968,
  title={Speech discrimination by dynamic programming},
  author={Vintsyuk, Taras K},
  journal={Cybernetics},
  volume={4},
  number={1},
  pages={52--57},
  year={1968},
  publisher={Springer}
}
@article{Zimmer2021,
   abstract = {While early AutoML frameworks focused on optimizing traditional ML pipelines and their hyperparameters, a recent trend in AutoML is to focus on neural architecture search. In this paper, we introduce Auto-PyTorch, which brings the best of these two worlds together by jointly and robustly optimizing the architecture of networks and the training hyperparameters to enable fully automated deep learning (AutoDL). Auto-PyTorch achieves state-of-the-art performance on several tabular benchmarks by combining multi-fidelity optimization with portfolio construction for warmstarting and ensembling of deep neural networks (DNNs) and common baselines for tabular data. To thoroughly study our assumptions on how to design such an AutoDL system, we additionally introduce a new benchmark on learning curves for DNNs, dubbed LCBench, and run extensive ablation studies of the full Auto-PyTorch on typical AutoML benchmarks, eventually showing that Auto-PyTorch performs better than several state-of-the-art competitors on average.},
   author = {Lucas Zimmer and Marius Lindauer and Frank Hutter},
   journal = {IEEE TPAMI},
   pages = {3079-3090},
   title = {Auto-PyTorch Tabular: Multi-Fidelity MetaLearning for Efficient and Robust AutoDL},
   year = {2021},
}
@article{Chen2017,
   abstract = {This tutorial provides a gentle introduction to kernel density estimation (KDE) and recent advances regarding confidence bands and geometric/topological features. We begin with a discussion of basic properties of KDE: the convergence rate under various metrics, density derivative estimation, and bandwidth selection. Then, we introduce common approaches to the construction of confidence intervals/bands, and we discuss how to handle bias. Next, we talk about recent advances in the inference of geometric and topological features of a density function using KDE. Finally, we illustrate how one can use KDE to estimate a cumulative distribution function and a receiver operating characteristic curve. We provide R implementations related to this tutorial at the end.},
   author = {Yen-Chi Chen},
   issue = {1},
   journal = {Biostatistics \& Epidemiology},
   pages = {161-187},
   title = {A Tutorial on Kernel Density Estimation and Recent Advances},
   volume = {1},
   year = {2017},
}
@misc{Carme2016,
   author = {Antoine Carme},
   title = {PyAF Python Automatic Forecasting},
   howpublished = {\url{https://github.com/antoinecarme/pyaf}},
   year = {2016},
}
@inproceedings{Zhou2021,
   abstract = {Many real-world applications require the prediction of long sequence time-series, such as electricity consumption planning. Long sequence time-series forecasting (LSTF) demands a high prediction capacity of the model, which is the ability to capture precise long-range dependency coupling between output and input efficiently. Recent studies have shown the potential of Transformer to increase the prediction capacity. However, there are several severe issues with Transformer that prevent it from being directly applicable to LSTF, including quadratic time complexity, high memory usage, and inherent limitation of the encoder-decoder architecture. To address these issues, we design an efficient transformer-based model for LSTF, named Informer, with three distinctive characteristics: (i) a ProbSparse self-attention mechanism, which achieves O(L log L) in time complexity and memory usage, and has comparable performance on sequences' dependency alignment. (ii) the self-attention distilling highlights dominating attention by halving cascading layer input, and efficiently handles extreme long input sequences. (iii) the generative style decoder, while conceptually simple, predicts the long time-series sequences at one forward operation rather than a step-by-step way, which drastically improves the inference speed of long-sequence predictions. Extensive experiments on four large-scale datasets demonstrate that Informer significantly outperforms existing methods and provides a new solution to the LSTF problem.},
   author = {Haoyi Zhou and Shanghang Zhang and Jieqi Peng and Shuai Zhang and Jianxin Li and Hui Xiong and Wancai Zhang},
   booktitle = {AAAI Conference on Artificial Intelligence},
   keywords = {Application Domains: Energy & Environment & Sustainability,Machine Learning: (Deep) Neural Network Algorithms,Machine Learning: Time-Series/Data Streams},
   pages = {11106-11115},
   title = {Informer: Beyond Efficient Transformer for Long Sequence Time-Series Forecasting},
   year = {2021},
}
@article{Hajirahimi2023,
   abstract = {Achieving the desired accuracy in time series forecasting has become a binding domain, and developing a forecasting framework with a high degree of accuracy is one of the most challenging tasks in this area. Combining different forecasting methods to construct efficient hybrid models has been widely reported in the literature regarding this challenge. Various types of hybrid models have been developed and successfully employed to improve forecasting accuracy. The well-known hybrid models can be generally categorized into four classes: (1) preprocessing-based, (2) parameter optimization-based, (3) components combination-based, and (4) postprocessing-based hybrid models. Despite the significant successes of hybrid models, efforts to access more accurate results face continued growth. Hybridization of hybrid models is a novel idea proposed to obtain extreme accuracy in recent literature, in which two or more hybrid classes are combined instead of conjoining the conventional individual forecasting methods. Although, in many publications, the aforementioned classes of hybrid models have been reviewed and analyzed in a wide variety of forecasting fields; no study is conducted to review the hybridization of hybrid models. This paper’s main contribution is to fill this gap and provide classification and comprehensive review of the current endeavors done in the hybridization of hybrid models in time series forecasting areas. Our searches indicate that more than 250 papers have been published in recent years utilizing hybridization of hybrid models. In this paper, these published papers have been classified regarding their different used combination strategies into four main categories, including (1) Hybridization with preprocessing-based hybrid models (HPH), (2) Hybridization with parameter optimization-based hybrid models (HOH), (3) Hybridization with components combination-based hybrid models (HCH) and, (4) Hybridization with postprocessing-based hybrid models (HSH). Each hybridization of the hybrid class is evaluated regarding the usage frequency, specific merits, and limitations. It can be inferred from reviewing articles that the hybridization of the hybrid concept, as a recent advancement in time series forecasting, can significantly improve traditional hybrid models’ accuracy. Furthermore, each category’s research gaps and some future research directions are identified in this paper.},
   author = {Zahra Hajirahimi and Mehdi Khashei},
   issn = {15737462},
   issue = {2},
   journal = {Artificial Intelligence Review},
   keywords = {Artificial Neural Networks (ANNs),Hybrid models,Hybridization of hybrid structures,Improving forecasting accuracy,Time series forecasting},
   pages = {1201-1261},
   publisher = {Springer Nature},
   title = {Hybridization of hybrid structures for time series forecasting: a review},
   volume = {56},
   year = {2023},
}
@inproceedings{Oliveira2014,
   abstract = {This paper describes a new type of ensembles that aims at improving the predictive performance of these approaches in time series forecasting. Ensembles are recognised as one of the most successful approaches to prediction tasks. Previous theoretical studies of ensembles have shown that one of the key reasons for this performance is diversity among ensemble members. Several methods exist to generate diversity. The key idea of the work we are presenting here is to propose a new form of diversity generation that explores some specific properties of time series prediction tasks. Our hypothesis is that the resulting ensemble members will be better at addressing different dynamic regimes of time series data. Our large set of experiments confirms that the methods we have explored for generating diversity are able to improve the performance of the equivalent ensembles with standard diversity generation procedures.},
   author = {Mariana Oliveira and Dinh Phung and Hang Li},
   booktitle = {Asian Conference on Machine Learning},
   keywords = {bagging,ensemble methods,maximum embed,time series forecasting},
   pages = {360-370},
   title = {Ensembles for Time Series Forecasting},
   volume = {39},
   year = {2014},
}
@article{gijsbers2022amlb,
   abstract = {Comparing different AutoML frameworks is notoriously challenging and often done incorrectly. We introduce an open and extensible benchmark that follows best practices and avoids common mistakes when comparing AutoML frameworks. We conduct a thorough comparison of 9 well-known AutoML frameworks across 71 classification and 33 regression tasks. The differences between the AutoML frameworks are explored with a multi-faceted analysis, evaluating model accuracy, its trade-offs with inference time, and framework failures. We also use Bradley-Terry trees to discover subsets of tasks where the relative AutoML framework rankings differ. The benchmark comes with an open-source tool that integrates with many AutoML frameworks and automates the empirical evaluation process end-to-end: from framework installation and resource allocation to in-depth evaluation. The benchmark uses public data sets, can be easily extended with other AutoML frameworks and tasks, and has a website with up-to-date results.},
   author = {Pieter Gijsbers and Marcos L. P. Bueno and Stefan Coors and Erin LeDell and Sébastien Poirier and Janek Thomas and Bernd Bischl and Joaquin Vanschoren},
   journal = {arXiv:2207.12560},
   title = {AMLB: an AutoML Benchmark},
   year = {2022},
}
@article{Demsar2006,
   abstract = {While methods for comparing two learning algorithms on a single data set have been scrutinized for quite some time already, the issue of statistical tests for comparisons of more algorithms on multiple data sets, which is even more essential to typical machine learning studies, has been all but ignored. This article reviews the current practice and then theoretically and empirically examines several suitable tests. Based on that, we recommend a set of simple, yet safe and robust non-parametric tests for statistical comparisons of classifiers: the Wilcoxon signed ranks test for comparison of two classifiers and the Friedman test with the corresponding post-hoc tests for comparison of more classifiers over multiple data sets. Results of the latter can also be neatly presented with the newly introduced CD (critical difference) diagrams.},
   author = {Janez Demšar},
   journal = {Journal of Machine Learning Research},
   keywords = {Friedman test,Wilcoxon signed ranks test,comparative studies,multiple comparisons tests,statistical methods},
   pages = {1-30},
   title = {Statistical Comparisons of Classifiers over Multiple Data Sets},
   volume = {7},
   year = {2006},
}
@inproceedings{Shchur2023,
   abstract = {We introduce AutoGluon-TimeSeries - an open-source AutoML library for probabilistic time series forecasting. Focused on ease of use and robustness, AutoGluon-TimeSeries enables users to generate accurate point and quantile forecasts with just 3 lines of Python code. Built on the design philosophy of AutoGluon, AutoGluon-TimeSeries leverages ensembles of diverse forecasting models to deliver high accuracy within a short training time. AutoGluon-TimeSeries combines both conventional statistical models, machine-learning based forecasting approaches, and ensembling techniques. In our evaluation on 29 benchmark datasets, AutoGluon-TimeSeries demonstrates strong empirical performance, outperforming a range of forecasting methods in terms of both point and quantile forecast accuracy, and often even improving upon the best-in-hindsight combination of prior methods.},
   author = {Oleksandr Shchur and Caner Turkmen and Nick Erickson and Huibin Shen and Alexander Shirkov and Tony Hu and Yuyang Wang},
   booktitle = {International Conference on Automated Machine Learning},
   title = {AutoGluon-TimeSeries: AutoML for Probabilistic Time Series Forecasting},
   year = {2023},
}
@article{Lim2019,
   abstract = {Multi-horizon forecasting often contains a complex mix of inputs – including static (i.e. time-invariant) covariates, known future inputs, and other exogenous time series that are only observed in the past – without any prior information on how they interact with the target. Several deep learning methods have been proposed, but they are typically ‘black-box’ models that do not shed light on how they use the full range of inputs present in practical scenarios. In this paper, we introduce the Temporal Fusion Transformer (TFT) – a novel attention-based architecture that combines high-performance multi-horizon forecasting with interpretable insights into temporal dynamics. To learn temporal relationships at different scales, TFT uses recurrent layers for local processing and interpretable self-attention layers for long-term dependencies. TFT utilizes specialized components to select relevant features and a series of gating layers to suppress unnecessary components, enabling high performance in a wide range of scenarios. On a variety of real-world datasets, we demonstrate significant performance improvements over existing benchmarks, and highlight three practical interpretability use cases of TFT.},
   author = {Bryan Lim and Sercan Arık and Nicolas Loeff and Tomas Pfister},
   issue = {4},
   journal = {International Journal of Forecasting},
   keywords = {Attention mechanisms,Deep learning,Explainable AI,Interpretability,Multi-horizon forecasting,Time series},
   pages = {1748-1764},
   publisher = {Elsevier B.V.},
   title = {Temporal Fusion Transformers for interpretable multi-horizon time series forecasting},
   volume = {37},
   year = {2021},
}
@article{Li2023,
   abstract = {Bayesian optimization is a highly efficient approach to optimizing objective functions which are expensive to query. These objectives are typically represented by Gaussian process (GP) surrogate models which are easy to optimize and support exact inference. While standard GP surrogates have been well-established in Bayesian optimization, Bayesian neural networks (BNNs) have recently become practical function approximators, with many benefits over standard GPs such as the ability to naturally handle non-stationarity and learn representations for high-dimensional data. In this paper, we study BNNs as alternatives to standard GP surrogates for optimization. We consider a variety of approximate inference procedures for finite-width BNNs, including high-quality Hamiltonian Monte Carlo, low-cost stochastic MCMC, and heuristics such as deep ensembles. We also consider infinite-width BNNs and partially stochastic models such as deep kernel learning. We evaluate this collection of surrogate models on diverse problems with varying dimensionality, number of objectives, non-stationarity, and discrete and continuous inputs. We find: (i) the ranking of methods is highly problem dependent, suggesting the need for tailored inductive biases; (ii) HMC is the most successful approximate inference procedure for fully stochastic BNNs; (iii) full stochasticity may be unnecessary as deep kernel learning is relatively competitive; (iv) infinite-width BNNs are particularly promising, especially in high dimensions.},
   author = {Yucen Lily Li and Tim G. J. Rudner and Andrew Gordon Wilson},
   journal = {arXiv preprint arXiv:2305.20028},
   title = {A Study of Bayesian Neural Network Surrogates for Bayesian Optimization},
   year = {2023},
}
@article{Frazier2009,
   abstract = {We consider a Bayesian ranking and selection problem with independent normal rewards and a correlated multivariate normal belief on the mean values of these rewards. Because this formulation of the ranking and selection problem models dependence between alternatives' mean values, algorithms may use this dependence to perform efficiently even when the number of alternatives is very large. We propose a fully sequential sampling policy called the knowledge-gradient policy, which is provably optimal in some special cases and has bounded suboptimality in all others. We then demonstrate how this policy may be applied to efficiently maximize a continuous function on a continuous domain while constrained to a fixed number of noisy measurements. © 2009 Informs.},
   author = {Peter Frazier and Warren Powell and Savas Dayanik},
   doi = {10.1287/ijoc.1080.0314},
   issn = {10919856},
   issue = {4},
   journal = {INFORMS Journal on Computing},
   keywords = {Bayesian,Decision analysis: sequential,Simulation: design of experiments,Statistics},
   pages = {599-613},
   title = {The Knowledge-Gradient Policy for Correlated Normal Beliefs},
   volume = {21},
   year = {2009},
}
@article{Henning2012,
   abstract = {Contemporary global optimization algorithms are based on local measures of utility, rather than a probability measure over location and value of the optimum. They thus attempt to collect low function values, not to learn about the optimum. The reason for the absence of probabilistic global optimizers is that the corresponding inference problem is intractable in several ways. This paper develops desiderata for probabilistic optimization algorithms, then presents a concrete algorithm which addresses each of the computational intractabilities with a sequence of approximations and explicitly addresses the decision problem of maximizing information gain from each evaluation.},
   author = {Philipp Hennig and Christian J Schuler},
   journal = {Journal of Machine Learning Research},
   keywords = {Gaussian processes,expectation propagation,information,optimization,probability},
   pages = {1809-1837},
   title = {Entropy Search for Information-Efficient Global Optimization},
   volume = {13},
   year = {2012},
}
@article{Bischl23,
   abstract = {Most machine learning algorithms are configured by a set of hyperparameters whose values must be carefully chosen and which often considerably impact performance. To avoid a time-consuming and irreproducible manual process of trial-and-error to find well-performing hyperparameter configurations, various automatic hyperparameter optimization (HPO) methods—for example, based on resampling error estimation for supervised machine learning—can be employed. After introducing HPO from a general perspective, this paper reviews important HPO methods, from simple techniques such as grid or random search to more advanced methods like evolution strategies, Bayesian optimization, Hyperband, and racing. This work gives practical recommendations regarding important choices to be made when conducting HPO, including the HPO algorithms themselves, performance evaluation, how to combine HPO with machine learning pipelines, runtime improvements, and parallelization. This article is categorized under: Algorithmic Development > Statistics Technologies > Machine Learning Technologies > Prediction.},
   author = {Bernd Bischl and Martin Binder and Michel Lang and Tobias Pielok and Jakob Richter and Stefan Coors and Janek Thomas and Theresa Ullmann and Marc Becker and Anne Laure Boulesteix and Difan Deng and Marius Lindauer},
   issue = {2},
   journal = {WIRE: Data Mining and Knowledge Discovery},
   keywords = {automl,hyperparameter optimization,machine learning,model selection,tuning},
   publisher = {John Wiley and Sons Inc},
   title = {Hyperparameter optimization: Foundations, algorithms, best practices, and open challenges},
   volume = {13},
   year = {2023},
}
@article{Pushak2022,
   abstract = { As interest in machine learning and its applications becomes more widespread, how to choose the best models and hyper-parameter settings becomes more important. This problem is known to be challenging for human experts, and consequently, a growing number of methods have been proposed for solving it, giving rise to the area of automated machine learning (AutoML). Many of the most popular AutoML methods are based on Bayesian optimization, which makes only weak assumptions about how modifying hyper-parameters effects the loss of a model. This is a safe assumption that yields robust methods, as the AutoML loss landscapes that relate hyper-parameter settings to loss are poorly understood. We build on recent work on the study of one-dimensional slices of algorithm configuration landscapes by introducing new methods that test n -dimensional landscapes for statistical deviations from uni-modality and convexity, and we use them to show that a diverse set of AutoML loss landscapes are highly structured. We introduce a method for assessing the significance of hyper-parameter partial derivatives, which reveals that most (but not all) AutoML loss landscapes only have a small number of hyper-parameters that interact strongly. To further assess hyper-parameter interactions, we introduce a simplistic optimization procedure that assumes each hyper-parameter can be optimized independently, a single time in sequence, and we show that it obtains configurations that are statistically tied with optimal in all of the n -dimensional AutoML loss landscapes that we studied. Our results suggest many possible new directions for substantially improving the state of the art in AutoML. },
   author = {Yasha Pushak and Holger Hoos},
   doi = {10.1145/3558774},
   issn = {2688-299X},
   issue = {3},
   journal = {ACM Transactions on Evolutionary Learning and Optimization},
   pages = {1-30},
   publisher = {Association for Computing Machinery (ACM)},
   title = {AutoML Loss Landscapes},
   volume = {2},
   year = {2022},
}
@incollection{Brazdil2022,
   abstract = {This chapter describes various approaches for the hyperparameter optimization (HPO) and combined algorithm selection and hyperparameter optimization problems (CASH). It starts by presenting some basic hyperparameter optimization methods, including grid search, random search, racing strategies, successive halving and hyperband. Next, it discusses Bayesian optimization, a technique that learns from the observed performance of previously tried hyperparameter settings on the current task. This knowledge is used to build a meta-model (surrogate model) that can be used to predict which unseen configurations may work better on that task. This part includes the description sequential model-based optimization (SMBO). This chapter also covers metalearning techniques that extend the previously discussed optimization techniques with the ability to transfer knowledge across tasks. This includes techniques such as warm-starting the search, or transferring previously learned meta-models that were trained on prior (similar) tasks. A key question here is how to establish how similar prior tasks are to the new task. This can be done on the basis of past experiments, but can also exploit the information gained from recent experiments on the target task. This chapter presents an overview of some recent methods proposed in this area.},
   author = {Pavel Brazdil and Jan N. van Rijn and Carlos Soares and Joaquin Vanschoren},
   doi = {10.1007/978-3-030-67024-5_6},
   issn = {21976635},
   booktitle = {Cognitive Technologies},
   pages = {103-122},
   publisher = {Springer Science and Business Media Deutschland GmbH},
   title = {Metalearning for Hyperparameter Optimization},
   year = {2022},
}
@inproceedings{Jarrett2021,
   abstract = {Time-series learning is the bread and butter of data-driven clinical decision support, and the recent explosion in ML research has demonstrated great potential in various healthcare settings. At the same time, medical time-series problems in the wild are challenging due to their highly composite nature: They entail design choices and interactions among components that preprocess data, impute missing values, select features, issue predictions, estimate uncertainty, and interpret models. Despite exponential growth in electronic patient data, there is a remarkable gap between the potential and realized utilization of ML for clinical research and decision support. In particular, orchestrating a real-world project lifecycle poses challenges in engineering (i.e. hard to build), evaluation (i.e. hard to assess), and efficiency (i.e. hard to optimize). Designed to address these issues simultaneously, Clairvoyance proposes a unified, end-to-end, autoML-friendly pipeline that serves as a (i) software toolkit, (ii) empirical standard, and (iii) interface for optimization. Our ultimate goal lies in facilitating transparent and reproducible experimentation with complex inference workflows, providing integrated pathways for (1) personalized prediction, (2) treatment-effect estimation, and (3) information acquisition. Through illustrative examples on real-world data in outpatient, general wards, and intensive-care settings, we illustrate the applicability of the pipeline paradigm on core tasks in the health-care journey. To the best of our knowledge, Clairvoyance is the first to demonstrate viability of a comprehensive and automatable pipeline for clinical time-series ML.},
   author = {Daniel Jarrett and Ari Ercole and Jinsung Yoon and Zhaozhi Qian and Mihaela Van Der Schaar},
   booktitle = {International Conference on Learning Representations},
   title = {Clairvoyance: A pipeline toolkit for medical time series.},
   url = {https://github.com/vanderschaarlab/clairvoyance},
   year = {2021},
}

